BUDHIES V: The baryonic Tully-Fisher relation at z=0.2 based on direct HI detections

We present HI-based B- and R-band Tully-Fisher relations (TFRs) and the Baryonic TFR (BTFR) at z=0.2 using direct HI detections from the Blind Ultra-Deep HI Environmental Survey (BUDHIES). Deep photometry from the Isaac Newton Telescope was used for 36 out of 166 HI sources, matching the quality criteria required for a robust TFR analysis. Two velocity definitions at 20% and 50% of the peak flux were measured from the global HI profiles and adopted as proxies for the circular velocities. We compare our results with an identically constructed z=0 TFR from the Ursa Major (UMa) association of galaxies. To ensure an unbiased comparison of the TFR, all the samples were treated identically regarding sample selection and applied corrections. We provide catalogues and an atlas showcasing the properties of the galaxies. Our analysis is focused on the zero points of the TFR and BTFR with their slopes fixed to the z=0 relation. Our main results are: (1) The BUDHIES galaxies show more asymmetric HI profiles with shallower wings compared to the UMa galaxies, which is likely due to the environment in which they reside, (2) The luminosity-based z=0.2 TFRs are brighter and bluer than the z=0 TFRs, even when cluster galaxies are excluded from the BUDHIES sample, (3) The BTFR shows no evolution in its zero point over the past 2.5 billion years and does not significantly change on the inclusion of cluster galaxies, and (4) proper sample selection and consistent corrections are crucial for an unbiased analysis of the evolution of the TFR.

==> TF_tables.tex <==
\onecolumn

%\setcounter{table}{0}
\begin{landscape}
\LTcapwidth=\textwidth
\begin{longtable}{c  c  c  c  c  c  c  c  c  c  c  c  c}

\caption{\label{tab:A963_HI_table} HI properties of the TF galaxies in A963.} \\

\hline \hline

Sr. no. & Cat no. & HI ID  & R & SNR & z$_{HI}$ & D$_{lum}$ & w$_{20}^{obs}$ & w$_{50}^{obs}$ & w$_{20}^{R,t,i}$ & w$_{50}^{R,t,i}$ & log M$_{HI}$ &  \\
 &   &  & km s$^{-1}$ &  &  & Mpc & km s$^{-1}$ & km s$^{-1}$ & km s$^{-1}$ &km s$^{-1}$ & M$_{\odot}$ & \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)\\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline

Sr. no. & Cat no. & HI ID  & R & SNR & z$_{HI}$ & D$_{lum}$ & w$_{20}^{obs}$ & w$_{50}^{obs}$ & w$_{20}^{R,t,i}$ & w$_{50}^{R,t,i}$ & log M$_{HI}$ & \\
 &   &  & km s$^{-1}$ &  &  & Mpc & km s$^{-1}$ & km s$^{-1}$ & km s$^{-1}$ &km s$^{-1}$ & M$_{\odot}$ & \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)\\

\hline 
\endhead
\hline
\endfoot
1  & 96  & HIJ101752.16+385857.1 & 39.46 & 4.88 & 0.20169 & 988.2  & 468.7 $\pm$ 15.2 & 368.8 $\pm$ 56.7 & 432.5 $\pm$ 30.4  & 355.4 $\pm$ 113.4 & 18.8 $\pm$ 0.5 & A963\\
2  & 124 & HIJ101914.04+391132.9 & 39.55 & 3.57 & 0.2043  & 1002.5 & 434.3 $\pm$ 8.4  & 397.2 $\pm$ 11.4 & 420.3 $\pm$ 17.7  & 405.1 $\pm$ 24.1  & 17.7 $\pm$ 0.8  & A963\\
3  & 9   & HIJ101611.10+384921.7 & 39.63 & 4.07 & 0.20674 & 1016.0 & 407.5 $\pm$ 8.1  & 380.3 $\pm$ 10.4 & 485.4 $\pm$ 21.2  & 479.6 $\pm$ 27.2  & 13.3 $\pm$ 0.6  & A963\\
4  & 93  & HIJ101748.32+390548.9 & 40.05 & 3.2  & 0.21947 & 1086.6 & 404.6 $\pm$ 19.3 & 339.1 $\pm$ 14.4 & 411.9 $\pm$ 43.2  & 364.1 $\pm$ 32.2  & 5.8 $\pm$ 0.3   & A963\\
5  & 20  & HIJ101626.57+391900.1 & 39.98 & 3.67 & 0.21746 & 1075.2 & 375.2 $\pm$ 13.6 & 338.0 $\pm$ 15.1 & 369.1 $\pm$ 29.6  & 353.4 $\pm$ 32.9  & 18.5 $\pm$ 0.8  & A963\\
6  & 2   & HIJ101523.89+390949.7 & 39.09 & 3.47 & 0.1904  & 926.7  & 349.1 $\pm$ 9.8  & 323.3 $\pm$ 9.5  & 328.0 $\pm$ 20.5  & 324.7 $\pm$ 19.9  & 5.5 $\pm$ 0.3   & A963\\
7  & 40  & HIJ101702.64+385109.6 & 39.6  & 4.85 & 0.20587 & 1011.2 & 341.4 $\pm$ 6.9  & 298.8 $\pm$ 5.6  & 309.6 $\pm$ 14.0  & 289.5 $\pm$ 11.4  & 13.1 $\pm$ 0.5  & A963\\
8  & 15  & HIJ101621.10+391550.8 & 38.33 & 3.39 & 0.16722 & 802.7  & 260.7 $\pm$ 15.0 & 211.1 $\pm$ 33.4 & 224.9 $\pm$ 30.0  & 198.0 $\pm$ 66.8  & 4.5 $\pm$ 0.2   & A963\\
9  & 41  & HIJ101703.64+391014.5 & 40.04 & 3.46 & 0.21937 & 1085.9 & 258.2 $\pm$ 23.6 & 221.3 $\pm$ 13.1 & 255.1 $\pm$ 54.3  & 238.9 $\pm$ 30.1  & 2.8 $\pm$ 0.2   & A963\\
10 & 107 & HIJ101803.86+384125.1 & 39.59 & 3.51 & 0.20546 & 1009.1 & 507.2 $\pm$ 18.0 & 428.3 $\pm$ 45.2 & 511.8 $\pm$ 39.1  & 450.8 $\pm$ 98.2  & 16.6 $\pm$ 0.8  & A963\\
11 & 78  & HIJ101737.25+391003.1 & 40.0  & 4.23 & 0.21788 & 1077.5 & 457.1 $\pm$ 49.5 & 380.2 $\pm$ 17.2 & 448.1 $\pm$ 105.4 & 390.5 $\pm$ 36.6  & 16.6 $\pm$ 0.6  & A963\\
12 & 67  & HIJ101727.44+384632.2 & 39.44 & 3.0  & 0.20104 & 984.8  & 449.0 $\pm$ 21.5 & 363.1 $\pm$ 14.4 & 438.5 $\pm$ 45.7  & 371.5 $\pm$ 30.6  & 9.9 $\pm$ 0.5   & A963\\
13 & 45  & HIJ101705.51+384927.4 & 39.54 & 3.08 & 0.20401 & 1000.8 & 445.6 $\pm$ 18.5 & 393.6 $\pm$ 13.4 & 453.9 $\pm$ 41.0  & 421.5 $\pm$ 29.7  & 8.4 $\pm$ 0.4   & A963\\
14 & 80  & HIJ101738.96+384817.8 & 38.35 & 3.63 & 0.16788 & 806.3  & 414.5 $\pm$ 8.6  & 311.7 $\pm$ 24.1 & 400.0 $\pm$ 18.2  & 315.4 $\pm$ 50.9  & 7.1 $\pm$ 0.4   & A963\\
15 & 82  & HIJ101739.56+391549.4 & 40.0  & 4.04 & 0.21802 & 1078.2 & 410.2 $\pm$ 13.6 & 379.0 $\pm$ 8.7  & 373.8 $\pm$ 27.2  & 365.4 $\pm$ 17.4  & 13.9 $\pm$ 0.6  & A963\\
16 & 109 & HIJ101809.30+390718.2 & 39.65 & 4.33 & 0.20745 & 1019.9 & 391.7 $\pm$ 9.1  & 345.7 $\pm$ 28.7 & 486.6 $\pm$ 24.9  & 454.8 $\pm$ 78.6  & 8.8 $\pm$ 0.4   & A963\\
17 & 10  & HIJ101613.62+390438.4 & 39.06 & 3.86 & 0.18954 & 922.2  & 372.1 $\pm$ 15.3 & 315.0 $\pm$ 17.8 & 400.2 $\pm$ 36.4  & 359.3 $\pm$ 42.4  & 8.4 $\pm$ 0.3   & A963\\
18 & 101 & HIJ101759.95+390637.9 & 39.72 & 3.89 & 0.20966 & 1032.0 & 345.0 $\pm$ 11.2 & 260.0 $\pm$ 10.9 & 395.4 $\pm$ 28.7  & 315.7 $\pm$ 27.9  & 6.9 $\pm$ 0.3   & A963\\
19 & 117 & HIJ101833.23+390403.3 & 39.5  & 2.97 & 0.20288 & 994.8  & 343.1 $\pm$ 22.5 & 282.1 $\pm$ 9.6  & 404.0 $\pm$ 59.2  & 353.7 $\pm$ 25.3  & 7.6 $\pm$ 0.5   & A963\\
20 & 63  & HIJ101725.27+390320.1 & 39.68 & 4.32 & 0.20822 & 1024.0 & 338.3 $\pm$ 8.1  & 305.0 $\pm$ 17.5 & 396.2 $\pm$ 21.3  & 382.4 $\pm$ 45.9  & 10.4 $\pm$ 0.4  & A963\\
21 & 27  & HIJ101641.11+391025.1 & 39.75 & 4.65 & 0.21047 & 1036.3 & 334.6 $\pm$ 22.2 & 256.1 $\pm$ 10.4 & 363.4 $\pm$ 54.1  & 295.5 $\pm$ 25.3  & 11.2 $\pm$ 0.4  & A963\\
22 & 54  & HIJ101717.31+391335.5 & 39.76 & 3.75 & 0.21079 & 1038.1 & 300.2 $\pm$ 8.7  & 233.7 $\pm$ 58.4 & 266.7 $\pm$ 17.6  & 222.5 $\pm$ 118.0 & 5.5 $\pm$ 0.3   & A963\\
23 & 37  & HIJ101701.14+384258.2 & 39.51 & 2.75 & 0.20328 & 996.9  & 266.7 $\pm$ 21.5 & 219.9 $\pm$ 23.0 & 294.5 $\pm$ 54.9  & 263.8 $\pm$ 58.8  & 4.3 $\pm$ 0.3   & A963\\
24 & 48  & HIJ101709.40+391138.3 & 40.01 & 4.33 & 0.21842 & 1080.6 & 259.8 $\pm$ 11.0 & 227.5 $\pm$ 14.4 & 225.0 $\pm$ 22.2  & 215.4 $\pm$ 29.0  & 6.3 $\pm$ 0.3   & A963\\
25 & 31  & HIJ101644.55+390744.6 & 39.67 & 2.96 & 0.20788 & 1022.4 & 257.1 $\pm$ 21.4 & 205.4 $\pm$ 22.9 & 244.4 $\pm$ 47.4  & 212.4 $\pm$ 50.7  & 4.1 $\pm$ 0.3   & A963\\
26 & 11  & HIJ101614.58+385123.2 & 39.63 & 3.29 & 0.20679 & 1016.6 & 255.8 $\pm$ 21.3 & 211.6 $\pm$ 20.8 & 242.9 $\pm$ 47.1  & 219.2 $\pm$ 46.0  & 6.8 $\pm$ 0.4   & A963\\
27 & 98  & HIJ101756.24+383811.3 & 39.55 & 3.1  & 0.20424 & 1002.2 & 243.9 $\pm$ 14.4 & 211.7 $\pm$ 19.0 & 215.2 $\pm$ 29.9  & 205.5 $\pm$ 39.4  & 6.5 $\pm$ 0.4   & A963\\
28 & 110 & HIJ101809.30+390118.4 & 39.54 & 3.17 & 0.20419 & 1002.2 & 226.9 $\pm$ 10.6 & 174.1 $\pm$ 18.8 & 202.0 $\pm$ 22.5  & 170.2 $\pm$ 39.8  & 6.5 $\pm$ 0.4   & A963\\
29 & 60  & HIJ101723.55+392811.2 & 39.5  & 4.3  & 0.20279 & 994.4  & 206.1 $\pm$ 9.4  & 168.6 $\pm$ 10.4 & 200.4 $\pm$ 22.2  & 183.0 $\pm$ 24.5  & 12.9 $\pm$ 0.7   & A963\\
%  & filt_ind & filthiid              & R4    & snr  & filtz   & filtdlum & w20pluserr       & w250pluserr      & w20corrpluserr   & w50corrpluserr   & mhipluserr     \\
30 & 13 & HIJ162557.88+425320.7 & 38.38 & 3.08 & 0.16869 & 810.5 & 475.1 $\pm$ 8.6  & 452.9 $\pm$ 6.6  & 486.2 $\pm$ 19.0 & 486.7 $\pm$ 14.6 & 11.1 $\pm$ 0.6  & A2192 \\
31 & 24 & HIJ162618.03+423811.8 & 39.11 & 2.91 & 0.19084 & 929.2 & 381.3 $\pm$ 8.8  & 360.5 $\pm$ 9.3  & 403.5 $\pm$ 20.6 & 405.7 $\pm$ 21.8 & 5.0 $\pm$ 0.3  & A2192\\
32 & 4  & HIJ162510.48+424033.8 & 38.99 & 3.88 & 0.18727 & 909.9 & 262.7 $\pm$ 8.5  & 237.9 $\pm$ 12.5 & 257.3 $\pm$ 19.3 & 254.9 $\pm$ 28.4 & 5.8 $\pm$ 0.3  & A2192\\
33 & 21 & HIJ162614.39+424632.3 & 39.13 & 3.27 & 0.1917  & 933.7 & 237.3 $\pm$ 9.0  & 197.7 $\pm$ 38.4 & 224.1 $\pm$ 20.1 & 205.4 $\pm$ 85.6 & 4.9 $\pm$ 0.3  & A2192\\
34 & 17 & HIJ162607.60+424126.7 & 39.08 & 3.74 & 0.19014 & 925.4 & 375.6 $\pm$ 11.5 & 270.6 $\pm$ 20.0 & 478.9 $\pm$ 32.5 & 362.8 $\pm$ 56.4 & 7.2 $\pm$ 0.3  & A2192\\
35 & 16 & HIJ162602.94+425053.5 & 39.04 & 2.27 & 0.1888  & 918.1 & 328.1 $\pm$ 16.5 & 226.0 $\pm$ 21.5 & 313.0 $\pm$ 35.4 & 227.9 $\pm$ 46.1 & 4.2 $\pm$ 0.3  & A2192\\
36 & 30 & HIJ162651.87+422710.8 & 39.0  & 3.15 & 0.18759 & 911.6 & 278.7 $\pm$ 6.5  & 229.2 $\pm$ 17.0 & 316.0 $\pm$ 17.0 & 281.2 $\pm$ 44.3 & 4.0 $\pm$ 0.2  & A2192\\
37 & 27 & HIJ162644.27+423915.5 & 39.1  & 2.53 & 0.19056 & 927.7 & 278.4 $\pm$ 7.5  & 251.6 $\pm$ 16.0 & 297.4 $\pm$ 18.4 & 292.4 $\pm$ 39.3 & 3.9 $\pm$ 0.3  & A2192\\
38 & 39 & HIJ162844.33+422617.8 & 38.45 & 3.11 & 0.17095 & 822.5 & 212.2 $\pm$ 25.1 & 178.7 $\pm$ 17.7 & 194.6 $\pm$ 55.4 & 182.7 $\pm$ 39.1 & 7.5 $\pm$ 0.5 & A2192 \\



\end{longtable}


\LTcapwidth=\textwidth
\begin{longtable}{ c  c  c  c  c  c  c  c  c  c  c  c  c}

\caption{\label{tab:A963_opt_table} Optical properties of the TF galaxies in A963.} \\

\hline \hline

Sr. no. & SDSS ID  & b/a & incl &M$_B$ & M$_R$ & M$_B^{corr}$ & M$_R^{corr}$ &M$_B^{tfq}$ & M$_R^{tfq}$ & log L$_{R}$ & log M$_{\ast}$ & log M$_{bar}$\\
 &   &  & deg &  &  &  &  &  &  & L$_{\odot}$ & M$_{\odot}$ & M$_{\odot}$ \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline

Sr. no. & SDSS ID  & b/a & incl &M$_B$ & M$_R$ & M$_B^{corr}$ & M$_R^{corr}$ &M$_B^{tfq}$ & M$_R^{tfq}$ & log L$_{R}$ & log M$_{\ast}$ & log M$_{bar}$\\
 &   &  & deg &  &  &  &  &  &  & L$_{\odot}$ & M$_{\odot}$ & M$_{\odot}$ \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\

\hline 
\endhead
\hline
\endfoot

%   & filtsdssid           & axrpluserr        & incl  & M_B    & M_R    & M_B_tfq             & M_R_tfq             & logL_R & logM_star_R & logM_star_R2 & logM_bar & logM_bar2 \\
1  & SJ101752.21+385857.3 & 0.154 $\pm$ 0.002 & 90.0  & -21.43 & -22.14 & -20.44 & -21.31 & 10.7  & 10.42 & 10.25 & 10.72 & 10.64 \\
2  & SJ101913.95+391122.2 & 0.372 $\pm$ 0.001 & 71.29 & -21.9  & -22.66 & -21.56 & -22.32 & 10.9  & 10.69 & 10.51 & 10.87 & 10.76 \\
3  & SJ101611.13+384924.3 & 0.662 $\pm$ 0.002 & 49.89 & -22.14 & -23.16 & -22.12 & -23.07 & 11.1  & 11.09 & 10.98 & 11.15 & 11.06 \\
4  & SJ101748.10+390544.4 & 0.483 $\pm$ 0.015 & 63.37 & -20.4  & -21.34 & -20.24 & -21.14 & 10.38 & 10.31 & 10.18 & 10.46 & 10.37 \\
5  & SJ101626.35+391900.8 & 0.437 $\pm$ 0.004 & 66.64 & -20.78 & -21.76 & -20.61 & -21.54 & 10.54 & 10.51 & 10.39 & 10.76 & 10.7  \\
6  & SJ101523.65+390941.2 & 0.354 $\pm$ 0.002 & 72.65 & -21.3  & -22.04 & -21.06 & -21.77 & 10.66 & 10.42 & 10.25 & 10.53 & 10.4  \\
7  & SJ101702.77+385115.5 & 0.26 $\pm$ 0.004  & 80.27 & -20.46 & -21.19 & -20.1  & -20.81 & 10.32 & 10.07 & 9.89  & 10.48 & 10.42 \\
8  & SJ101620.90+391552.7 & 0.184 $\pm$ 0.003 & 90.0  & -19.34 & -19.97 & -19.08 & -19.64 & 9.83  & 9.46  & 9.3   & 9.96  & 9.92  \\
9  & SJ101703.62+391018.0 & 0.524 $\pm$ 0.01  & 60.38 & -20.12 & -20.94 & -20.17 & -20.89 & 10.22 & 10.06 & 9.89  & 10.19 & 10.07 \\
10 & SJ101803.65+384119.7 & 0.433 $\pm$ 0.003 & 66.94 & -22.31 & -23.07 & -21.99 & -22.74 & 11.07 & 10.85 & 10.67 & 10.97 & 10.85 \\
11 & SJ101737.03+391005.8 & 0.392 $\pm$ 0.004 & 69.86 & -21.46 & -22.24 & -21.12 & -21.9  & 10.74 & 10.54 & 10.37 & 10.77 & 10.67 \\
12 & SJ101727.72+384627.8 & 0.386 $\pm$ 0.002 & 70.27 & -21.52 & -22.26 & -21.19 & -21.93 & 10.74 & 10.51 & 10.33 & 10.67 & 10.55 \\
13 & SJ101705.49+384924.8 & 0.468 $\pm$ 0.002 & 64.41 & -21.48 & -22.34 & -21.26 & -22.09 & 10.78 & 10.65 & 10.49 & 10.75 & 10.63 \\
14 & SJ101738.32+384806.7 & 0.374 $\pm$ 0.006 & 71.2  & -19.8  & -20.47 & -19.49 & -20.15 & 10.03 & 9.72  & 9.54  & 10.18 & 10.13 \\
15 & SJ101739.82+391547.9 & 0.176 $\pm$ 0.005 & 90.0  & -21.28 & -22.05 & -20.53 & -21.4  & 10.66 & 10.47 & 10.29 & 10.69 & 10.59 \\
16 & SJ101809.25+390716.6 & 0.698 $\pm$ 0.011 & 46.93 & -20.74 & -21.56 & -20.75 & -21.5  & 10.47 & 10.31 & 10.14 & 10.51 & 10.42 \\
17 & SJ101613.68+390437.8 & 0.568 $\pm$ 0.003 & 57.1  & -20.62 & -21.53 & -20.56 & -21.4  & 10.45 & 10.36 & 10.22 & 10.54 & 10.45 \\
18 & SJ101759.72+390636.5 & 0.644 $\pm$ 0.003 & 51.33 & -20.89 & -21.65 & -20.9  & -21.58 & 10.5  & 10.29 & 10.12 & 10.47 & 10.36 \\
19 & SJ101833.28+390356.5 & 0.668 $\pm$ 0.004 & 49.43 & -21.86 & -22.69 & -21.88 & -22.63 & 10.92 & 10.77 & 10.61 & 10.84 & 10.71 \\
20 & SJ101725.11+390316.5 & 0.665 $\pm$ 0.002 & 49.67 & -20.79 & -21.66 & -20.81 & -21.6  & 10.5  & 10.39 & 10.23 & 10.59 & 10.5  \\
21 & SJ101641.08+391025.7 & 0.594 $\pm$ 0.007 & 55.16 & -21.01 & -21.67 & -21.01 & -21.58 & 10.51 & 10.18 & 10.01 & 10.49 & 10.41 \\
22 & SJ101717.55+391334.5 & 0.245 $\pm$ 0.006 & 81.65 & -21.04 & -21.5  & -20.75 & -21.17 & 10.44 & 9.76  & 9.74  & 10.13 & 10.12 \\
23 & SJ101701.11+384258.9 & 0.642 $\pm$ 0.006 & 51.5  & -20.26 & -21.04 & -20.34 & -21.02 & 10.26 & 10.06 & 9.89  & 10.25 & 10.14 \\
24 & SJ101709.09+391136.2 & 0.232 $\pm$ 0.003 & 83.13 & -20.47 & -21.11 & -20.28 & -20.85 & 10.28 & 9.94  & 9.77  & 10.24 & 10.16 \\
25 & SJ101644.46+390744.6 & 0.465 $\pm$ 0.003 & 64.64 & -20.18 & -20.99 & -20.21 & -20.91 & 10.24 & 10.07 & 9.9   & 10.24 & 10.13 \\
26 & SJ101613.95+385122.4 & 0.465 $\pm$ 0.008 & 64.65 & -20.06 & -20.84 & -20.09 & -20.76 & 10.18 & 9.98  & 9.8   & 10.28 & 10.2  \\
27 & SJ101756.25+383807.3 & 0.326 $\pm$ 0.004 & 74.74 & -21.07 & -21.61 & -21.04 & -21.47 & 10.49 & 9.98  & 9.86  & 10.27 & 10.22 \\
28 & SJ101809.12+390118.5 & 0.381 $\pm$ 0.022 & 70.69 & -18.28 & -18.94 & -18.33 & -18.87 & 9.42  & 9.09  & 8.92  & 10.02 & 10.0  \\
29 & SJ101723.76+392801.3 & 0.557 $\pm$ 0.016 & 57.99 & -18.88 & -19.52 & -19.03 & -19.53 & 9.65  & 9.29  & 9.12  & 10.3  & 10.29 \\

%  & filtsdssid           & axrpluserr        & incl  & M_B    & M_R    & M_B_tfq             & M_R_tfq             & logL_R & logM_star_R & logM_star_R2 & logM_bar & logM_bar2 \\
30 & SJ162558.03+425319.4 & 0.465 $\pm$ 0.002 & 64.63 & -21.86 & -22.66 & -21.61 & -22.39 & 10.9  & 10.73 & 10.56 & 10.84 & 10.71 \\
31 & SJ162618.09+423808.9 & 0.545 $\pm$ 0.001 & 58.83 & -20.32 & -21.15 & -20.24 & -21.01 & 10.3  & 10.15 & 9.99  & 10.33 & 10.22 \\
32 & SJ162510.56+424028.8 & 0.505 $\pm$ 0.001 & 61.76 & -20.32 & -20.99 & -20.35 & -20.92 & 10.23 & 9.92  & 9.74  & 10.21 & 10.13 \\
33 & SJ162614.11+424631.5 & 0.476 $\pm$ 0.001 & 63.86 & -19.9  & -20.72 & -19.96 & -20.66 & 10.13 & 9.97  & 9.8   & 10.21 & 10.12 \\
34 & SJ162607.85+424128.4 & 0.719 $\pm$ 0.002 & 45.16 & -21.32 & -22.12 & -21.35 & -22.07 & 10.69 & 10.51 & 10.34 & 10.63 & 10.5  \\
35 & SJ162602.68+425054.8 & 0.405 $\pm$ 0.002 & 68.93 & -20.41 & -21.26 & -20.26 & -21.06 & 10.35 & 10.22 & 10.06 & 10.35 & 10.24 \\
36 & SJ162651.30+422709.9 & 0.659 $\pm$ 0.003 & 50.16 & -19.15 & -19.8  & -19.22 & -19.77 & 9.76  & 9.42  & 9.25  & 9.92  & 9.87  \\
37 & SJ162644.36+423918.2 & 0.602 $\pm$ 0.006 & 54.56 & -19.53 & -20.24 & -19.58 & -20.2  & 9.94  & 9.68  & 9.5   & 10.01 & 9.93  \\
38 & SJ162843.80+422618.2 & 0.46 $\pm$ 0.002  & 65.0  & -19.35 & -19.96 & -19.47 & -19.94 & 9.82  & 9.42  & 9.27  & 10.12 & 10.09
\end{longtable}
\end{landscape}
\twocolumn

==> TF_tables_new.tex <==
\onecolumn

%\setcounter{table}{0}
\begin{landscape}
%\LTcapwidth=\textwidth
\setlength\LTcapwidth{22 cm}
\begin{longtable}{c  c  c  c  c  c  c  c  c  c  c  c  c}

\caption{\label{tab:A963_HI_table_tf} HI properties of the BUDHIES TF galaxies. The columns are described in detail in Sect. \ref{catalogue}\\ \\
\textit{Column} (1): The running identification number of the galaxies for easy cross-reference with entries in Table \ref{tab:A963_opt_table_tf};
\textit{Column} (2): The catalogue number assigned to these galaxies in Paper 1, for easy cross-reference to the atlas pages.;
\textit{Column} (3): The \H\ ID which contains the Right Ascension and Declination of the \H\ source [J2000].;
\textit{Column} (4): The rest-frame velocity resolution R at which the \H\ profile, total \H\ map and Position-Velocity diagrams were extracted from the data cubes. The velocity resolution is set at 4 $\times$ $\Delta$v (R4), where $\Delta$v is the redshift-dependent rest-frame width of the channel in \kms.;
\textit{Column} (5): The channel-average Signal-to-Noise Ratio (SNR) of the extracted \H\ profiles of each galaxy;
\textit{Column} (6): The galaxy redshift based on the \H\ profile;
\textit{Column} (7): The luminosity distance to the galaxy, calculated using its \H\ redshift and the adopted cosmology;
\textit{Columns} (8) \& (9): The observed (rest frame) $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$ line widths, including their errors;
\textit{Column} (10) \& (11): The \wct\ and \wcf\ line widths corrected for instrumental resolution, turbulent motions and inclination, following the methodology described in Sect. \ref{corr};
\textit{Column} (12): \H\ masses ($\times$ 10$^9$ \Msun) calculated from the integrated flux densities of the extracted \H\ profiles, including their uncertainties. For further details, see Paper 1;
\textit{Column} (13): The volume (A963 or A2192) and sample (\textit{TFS} or \textit{HQS}) that a galaxy belongs to.}. \\

\hline \hline

Sr. no. & Cat no. & HI ID  & R & SNR & z$_{HI}$ & D$_{lum}$ & w$_{20}^{obs}$ & w$_{50}^{obs}$ & w$_{20}^{R,t,i}$ & w$_{50}^{R,t,i}$ & M$_{HI}$ &  \\
 &   &  & km s$^{-1}$ &  &  & Mpc & km s$^{-1}$ & km s$^{-1}$ & km s$^{-1}$ &km s$^{-1}$ & $\times$ 10$^9$ M$_{\odot}$ & \multicolumn{1}{c}{Sample}\\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) &  \multicolumn{1}{c}{(13)}\\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline

Sr. no. & Cat no. & HI ID  & R & SNR & z$_{HI}$ & D$_{lum}$ & w$_{20}^{obs}$ & w$_{50}^{obs}$ & w$_{20}^{R,t,i}$ & w$_{50}^{R,t,i}$ & log M$_{HI}$ & \\
 &   &  & km s$^{-1}$ &  &  & Mpc & km s$^{-1}$ & km s$^{-1}$ & km s$^{-1}$ &km s$^{-1}$ & $\times$ 10$^9$ M$_{\odot}$ & \multicolumn{1}{c}{Sample}\\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & \multicolumn{1}{c}{(13)}\\

\hline 
\endhead
\hline
\endfoot




1  & 7   & HIJ101600.44+385211.7 & 39.7 & 2.6 & 0.20861 & 1026 & 126 $\pm$ 10 & 104 $\pm$ 12 & 115 $\pm$ 27  & 117 $\pm$ 31  & 3.7 $\pm$ 0.4  & TFS A963 \\
2  & 10  & HIJ101613.62+390438.4 & 39.1 & 3.8 & 0.18954 & 922  & 372 $\pm$ 15 & 315 $\pm$ 18 & 400 $\pm$ 37  & 359 $\pm$ 42  & 8.4 $\pm$ 0.3  & TFS A963 \\
3  & 27  & HIJ101641.11+391025.1 & 39.8 & 4.6 & 0.21047 & 1036 & 335 $\pm$ 22 & 256 $\pm$ 10 & 363 $\pm$ 54  & 296 $\pm$ 25  & 11.2 $\pm$ 0.4 & TFS A963 \\
4  & 37  & HIJ101701.14+384258.2 & 39.5 & 2.7 & 0.20328 & 996 & 268 $\pm$ 22 & 220 $\pm$ 23 & 295 $\pm$ 55  & 264 $\pm$ 59  & 4.3 $\pm$ 0.3  & TFS A963 \\
5  & 45  & HIJ101705.51+384927.4 & 39.5 & 3.1 & 0.20401 & 1000 & 446 $\pm$ 19 & 394 $\pm$ 13 & 454 $\pm$ 41  & 422 $\pm$ 30  & 8.4 $\pm$ 0.4  & TFS A963 \\
6 & 50  & HIJ101711.87+385419.0 & 39.9 & 3.1  & 0.21613 & 1067 & 308 $\pm$ 16 & 228 $\pm$ 41 & 279 $\pm$ 32  & 220 $\pm$ 84  & 8.4 $\pm$ 0.6  & TFS A963 \\
7 & 54  & HIJ101717.31+391335.5 & 39.8 & 3.8 & 0.21079 & 1038 & 300 $\pm$ 9  & 234 $\pm$ 58 & 267 $\pm$ 18  & 223 $\pm$ 118 & 5.5 $\pm$ 0.3  & TFS A963 \\
8 & 58  & HIJ101720.60+391054.4 & 39.3 & 2.6 & 0.19808 & 968  & 433 $\pm$ 28 & 292 $\pm$ 24 & 507 $\pm$ 72  & 356 $\pm$ 61  & 8.8 $\pm$ 0.5  & TFS A963 \\
9 & 67  & HIJ101727.44+384632.2 & 39.4 & 3.0    & 0.20104 & 985  & 449 $\pm$ 22 & 363 $\pm$ 14 & 439 $\pm$ 46  & 372 $\pm$ 31  & 9.9 $\pm$ 0.5  & TFS A963 \\
10 & 78  & HIJ101737.25+391003.1 & 40.0   & 4.2 & 0.21788 & 1078 & 457 $\pm$ 50 & 380 $\pm$ 17 & 448 $\pm$ 106 & 391 $\pm$ 37  & 16.6 $\pm$ 0.6 & TFS A963 \\
11 & 93  & HIJ101748.32+390548.9 & 40.1 & 3.2  & 0.21947 & 1087 & 405 $\pm$ 19 & 339 $\pm$ 14 & 412 $\pm$ 43  & 364 $\pm$ 32  & 5.8 $\pm$ 0.3  & TFS A963 \\
12 & 99  & HIJ101757.27+391032.7 & 39.4 & 3.1 & 0.19946 & 976  & 252 $\pm$ 45 & 192 $\pm$ 39 & 239 $\pm$ 100 & 198 $\pm$ 85  & 4.0 $\pm$ 0.3  & TFS A963 \\
13 & 101 & HIJ101759.95+390637.9 & 39.7 & 3.9 & 0.20966 & 1032   & 345 $\pm$ 11 & 260 $\pm$ 11 & 395 $\pm$ 29  & 316 $\pm$ 28  & 6.9 $\pm$ 0.3  & TFS A963 \\
14 & 102 & HIJ101800.01+391649.2 & 39.4 & 2.3 & 0.19884 & 973  & 340 $\pm$ 22 & 293 $\pm$ 62 & 303 $\pm$ 43  & 280 $\pm$ 124 & 7.9 $\pm$ 0.6  & TFS A963\\
15 & 110 & HIJ101809.30+390118.4 & 39.5 & 3.2 & 0.20419 & 1002 & 227 $\pm$ 11 & 174 $\pm$ 19 & 202 $\pm$ 23  & 170 $\pm$ 40  & 6.5 $\pm$ 0.4  & TFS A963 \\
16 & 117 & HIJ101833.23+390403.3 & 39.5  & 3.0 & 0.20288 & 995  & 343 $\pm$ 23 & 282 $\pm$ 10  & 404 $\pm$ 59  & 354 $\pm$ 25  & 7.6 $\pm$ 0.5  & TFS A963 \\
17 & 118 & HIJ101835.11+385816.3 & 38.3 & 4.1 & 0.16669 & 800  & 380 $\pm$ 18 & 310 $\pm$ 39 & 410 $\pm$ 43  & 353 $\pm$ 92  & 9.7 $\pm$ 0.5  & TFS A963 \\
18  & 2   & HIJ101523.89+390949.7 & 39.1 & 3.5 & 0.19040  & 927  & 349 $\pm$ 10  & 323 $\pm$ 10  & 328 $\pm$ 21  & 325 $\pm$ 20  & 5.5 $\pm$ 0.3  & TFS/HQS A963 \\
19  & 9   & HIJ101611.10+384921.7 & 39.6 & 4.1 & 0.20674 & 1016   & 408 $\pm$ 8  & 380 $\pm$ 10 & 485 $\pm$ 21  & 480 $\pm$ 27  & 13.3 $\pm$ 0.6 & TFS/HQS A963 \\
20  & 20  & HIJ101626.57+391900.1 & 40.0 & 3.7 & 0.21746 & 1075 & 375 $\pm$ 14 & 338 $\pm$ 15 & 369 $\pm$ 30  & 353 $\pm$ 33  & 18.5 $\pm$ 0.8 & TFS/HQS A963 \\
21  & 40  & HIJ101702.64+385109.6 & 39.6  & 4.9 & 0.20587 & 1011 & 341 $\pm$ 7  & 299 $\pm$ 6  & 310 $\pm$ 14  & 289 $\pm$ 11  & 13.1 $\pm$ 0.5 & TFS/HQS A963 \\
22 & 48  & HIJ101709.40+391138.3 & 40.0 & 4.3 & 0.21842 & 1081 & 260 $\pm$ 11 & 227 $\pm$ 14 & 225 $\pm$ 22  & 215 $\pm$ 29  & 6.3 $\pm$ 0.3  & TFS/HQS A963 \\
23 & 61  & HIJ101723.56+390255.5 & 38.4 & 3.0 & 0.16871 & 811  & 267 $\pm$ 12 & 247 $\pm$ 7  & 239 $\pm$ 25  & 241 $\pm$ 14  & 2.2 $\pm$ 0.2  & TFS/HQS A963 \\
24 & 63  & HIJ101725.27+390320.1 & 39.7 & 4.32 & 0.20822 & 1024   & 338 $\pm$ 8  & 305 $\pm$ 18 & 396 $\pm$ 21  & 382 $\pm$ 46  & 10.4 $\pm$ 0.4 & TFS/HQS A963 \\
25 & 71  & HIJ101729.58+385829.8 & 39.5 & 3.6 & 0.20381 & 1000  & 319 $\pm$ 11 & 285 $\pm$ 23 & 291 $\pm$ 22  & 281 $\pm$ 48  & 3.5 $\pm$ 0.2  & TFS/HQS A963 \\
26 & 82  & HIJ101739.56+391549.4 & 40.0    & 4.0 & 0.21802 & 1078 & 410 $\pm$ 14 & 379 $\pm$ 9  & 374 $\pm$ 27  & 365 $\pm$ 17  & 13.9 $\pm$ 0.6 & TFS/HQS A963 \\
27 & 86  & HIJ101742.36+390133.5 & 39.7 & 5.5 & 0.20761 & 1021 & 168 $\pm$ 8  & 145 $\pm$ 9  & 154 $\pm$ 19  & 155 $\pm$ 22  & 2.9 $\pm$ 0.2  & TFS/HQS A963 \\
28 & 88  & HIJ101742.65+390104.7 & 39.7 & 3.7 & 0.20793 & 1023 & 335 $\pm$ 12 & 307 $\pm$ 34 & 310 $\pm$ 25  & 305 $\pm$ 70  & 3.6 $\pm$ 0.2  & TFS/HQS A963 \\
29 & 109 & HIJ101809.30+390718.2 & 39.7 & 4.3 & 0.20745 & 1020 & 392 $\pm$ 9  & 346 $\pm$ 29 & 487 $\pm$ 25  & 455 $\pm$ 79  & 8.8 $\pm$ 0.4  & TFS/HQS A963 \\
30 & 4   & HIJ162510.48+424033.8 & 39.0 & 3.9 & 0.18727 & 910  & 263 $\pm$ 9  & 238 $\pm$ 13 & 257 $\pm$ 19  & 255 $\pm$ 28  & 5.8 $\pm$ 0.3  & TFS/HQS A963 \\
31 & 13  & HIJ162557.88+425320.7 & 38.4 & 3.1 & 0.16869 & 811  & 475 $\pm$ 9  & 453 $\pm$ 7  & 486 $\pm$ 19  & 487 $\pm$ 15  & 11.1 $\pm$ 0.6 & TFS/HQS A2192 \\
32 & 18  & HIJ162607.84+424218.2 & 39.1 & 3.3  & 0.18975 & 923 & 235 $\pm$ 8  & 210 $\pm$ 14 & 227 $\pm$ 19  & 225 $\pm$ 31  & 3.2 $\pm$ 0.2  & TFS/HQS A2192 \\
33 & 24  & HIJ162618.03+423811.8 & 39.1 & 2.9 & 0.19084 & 929 & 381 $\pm$ 9  & 361 $\pm$ 9  & 404 $\pm$ 21  & 406 $\pm$ 22  & 5.0 $\pm$ 0.3  & TFS/HQS A2192 \\
34 & 30  & HIJ162651.87+422710.8 & 39.0    & 3.2 & 0.18759 & 917  & 279 $\pm$ 7  & 229 $\pm$ 17 & 316 $\pm$ 17  & 281 $\pm$ 44  & 4.0 $\pm$ 0.2  & TFS/HQS A2192 \\
35 & 31  & HIJ162652.61+422839.4 & 40.1 & 2.5 & 0.22086 & 1094 & 280 $\pm$ 10  & 250 $\pm$ 13 & 282 $\pm$ 23  & 273 $\pm$ 29  & 6.1 $\pm$ 0.4  & TFS/HQS A2192 \\
36 & 39  & HIJ162844.33+422617.8 & 38.5 & 3.1 & 0.17095 & 823  & 212 $\pm$ 25 & 179 $\pm$ 18 & 195 $\pm$ 55  & 183 $\pm$ 39  & 7.5 $\pm$ 0.5  & TFS/HQS A2192 \\


\end{longtable}




%\LTcapwidth=\textwidth
\setlength\LTcapwidth{20 cm}
\begin{longtable}{ c  c  c  c  c  c  c  c  c  c  c  c  c  c}

\caption{\label{tab:A963_opt_table_tf} Optical properties of the BUDHIES galaxies. The columns are described in detail in Sect. \ref{catalogue}\\ \\
\textit{Column} (1): The running identification number of the galaxies for easy cross-reference with entries in Table \ref{tab:A963_HI_table_tf};
\textit{Column} (2): The SDSS ID of the adopted optical counterpart of the \H\ detection, indicating the optical coordinates of the galaxy;
\textit{Column} (3): The minor-to-major axis ratios (b/a) obtained from \textit{galfit};
\textit{Column} (4): The inclination as inferred from the optical axis ratio (b/a), following Eq. (1) and assuming an intrinsic disc thickness q$_0$ of 0.2;
\textit{Columns} (5) \& (6): Total apparent INT B- and R- band magnitudes, respectively, including a small aperture correction as described in Sect. 4.2;
\textit{Columns} (7) \& (8): The k-corrections applied to the Galactic extinction corrected, apparent B- and R- band magnitudes, as described in Sect. 3;
\textit{Columns} (9) \& (10): The internal extinction corrections applied to the Galactic extinction and k-corrected B- and R- band magnitudes, as described in Sect. 3;
\textit{Columns} (11) \& (12): The corrected, absolute B- and R- band magnitudes, respectively;
\textit{Column} (13): Log stellar mass (\Msun) calculated using Eq. \ref{eq:mstar1};
\textit{Column} (14): Log baryonic mass (\Msun) calculated from the \H\ masses in Col. (12) of Table \ref{tab:A963_HI_table_tf}, and the stellar masses in Col. (13) respectively.
} \\

\hline \hline

Sr. no. & SDSS ID  & b/a & incl & m$_B$ & m$_R$ & k$_B$ & k$_R$ & A$^i_B$ & A$^i_R$ & M$_B$ & M$_R$ & log M$_{\ast}$ & log M$_{bar}$\\
 &   &  & deg &  &  &  &  & &  &  &  & M$_{\odot}$ & M$_{\odot}$ \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)  & (14) \\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline

Sr. no. & SDSS ID  & b/a & incl & m$_B$ & m$_R$ & k$_B$ & k$_R$ & A$^i_B$ & A$^i_R$ M$_B$ & M$_R$ & log M$_{\ast}$ & log M$_{bar}$\\
 &   &  & deg &  &  &  &  & &  &  &  & M$_{\odot}$ & M$_{\odot}$ \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)  & (14) \\

\hline 
\endhead
\hline
\endfoot

1  & SJ101600.10+385205.5 & 0.646 $\pm$ 0.011 & 51.2  & 21.19 & 20.08 & 0.07 & 0.06 & 0.41 & 0.04 & -19.40  & -20.10  & 9.63          & 9.98      \\
2  & SJ101613.68+390437.8 & 0.568 $\pm$ 0.003 & 57.1  & 20.46 & 18.81 & 0.45 & 0.33 & 0.74 & 0.15 & -20.62 & -21.53 & 10.37         & 10.55     \\
3  & SJ101641.08+391025.7 & 0.594 $\pm$ 0.007 & 55.2 & 19.98 & 18.78 & 0.39 & 0.29 & 0.47 & 0.06 & -21.01 & -21.67 & 10.19         & 10.5      \\
4  & SJ101701.11+384258.9 & 0.642 $\pm$ 0.006 & 51.5  & 20.65 & 19.29 & 0.29 & 0.21 & 0.58 & 0.10  & -20.26 & -21.04 & 10.07         & 10.25     \\
5  & SJ101705.49+384924.8 & 0.468 $\pm$ 0.002 & 64.4 & 20.04 & 18.34 & 0.66 & 0.48 & 0.80  & 0.17 & -21.48 & -22.34 & 10.66         & 10.76     \\
6 & SJ101711.90+385421.6 & 0.294 $\pm$ 0.022 & 77.3 & 21.89 & 20.08 & 0.75 & 0.56 & 0.90  & 0.19 & -19.95 & -20.84 & 10.08         & 10.38     \\
7 & SJ101717.55+391334.5 & 0.245 $\pm$ 0.006 & 81.7 & 20.30  & 19.25 & 0.83 & 0.62 & 0.37 & 0.02 & -21.04 & -21.50  & 9.80           & 10.15     \\
8 & SJ101721.45+391052.0 & 0.643 $\pm$ 0.010  & 51.4 & 20.55 & 18.55 & 0.41 & 0.29 & 0.95 & 0.22 & -20.80  & -21.92 & 10.66         & 10.76     \\
9 & SJ101727.72+384627.8 & 0.386 $\pm$ 0.002 & 70.3 & 20.02 & 18.46 & 0.81 & 0.59 & 0.71 & 0.14 & -21.52 & -22.26 & 10.52         & 10.68     \\
10 & SJ101737.03+391005.8 & 0.392 $\pm$ 0.004 & 69.9 & 20.37 & 18.71 & 0.81 & 0.58 & 0.81 & 0.17 & -21.46 & -22.24 & 10.55         & 10.77     \\
11 & SJ101748.10+390544.4 & 0.483 $\pm$ 0.015 & 63.4 & 21.35 & 19.51 & 0.60  & 0.43 & 0.93 & 0.20  & -20.40  & -21.34 & 10.32         & 10.46     \\
12 & SJ101757.22+391039.6 & 0.465 $\pm$ 0.031 & 64.6 & 22.63 & 21.25 & 0.41 & 0.31 & 0.59 & 0.10  & -18.37 & -19.14 & 9.30           & 9.88      \\
13 & SJ101759.72+390636.5 & 0.644 $\pm$ 0.003 & 51.3 & 20.18 & 18.81 & 0.35 & 0.25 & 0.60  & 0.11 & -20.89 & -21.65 & 10.30          & 10.47     \\
14 & SJ101759.13+391658.1 & 0.111 $\pm$ 0.032 & 90.0  & 22.10  & 20.57 & 1.45 & 1.07 & 0.68 & 0.13 & -20.03 & -20.60  & 9.64          & 10.19     \\
15 & SJ101809.12+390118.5 & 0.381 $\pm$ 0.022 & 70.7 & 22.67 & 21.48 & 0.43 & 0.33 & 0.46 & 0.06 & -18.28 & -18.94 & 9.11          & 10.02     \\
16 & SJ101833.28+390356.5 & 0.668 $\pm$ 0.004 & 49.4 & 19.18 & 17.69 & 0.33 & 0.24 & 0.67 & 0.13 & -21.86 & -22.69 & 10.78         & 10.85     \\
17 & SJ101835.20+385816.9 & 0.567 $\pm$ 0.006 & 57.2 & 19.64 & 17.88 & 0.46 & 0.34 & 0.74 & 0.17 & -21.13 & -22.17 & 10.71         & 10.81 \\
18  & SJ101523.65+390941.2 & 0.354 $\pm$ 0.002 & 72.7 & 19.96 & 18.48 & 0.73 & 0.53 & 0.64 & 0.12 & -21.30  & -22.04 & 10.44         & 10.54     \\
19  & SJ101611.13+384924.3 & 0.662 $\pm$ 0.002 & 49.9 & 19.20  & 17.37 & 0.37 & 0.27 & 0.89 & 0.19 & -22.14 & -23.16 & 11.09         & 11.15     \\
20  & SJ101626.35+391900.8 & 0.437 $\pm$ 0.004 & 66.6 & 21.02 & 19.10  & 0.63 & 0.46 & 0.96 & 0.22 & -20.78 & -21.76 & 10.51         & 10.77     \\
21  & SJ101702.77+385115.5 & 0.260 $\pm$ 0.004  & 80.3 & 21.24 & 19.67 & 0.90  & 0.66 & 0.73 & 0.14 & -20.46 & -21.19 & 10.08         & 10.48     \\
22 & SJ101709.09+391136.2 & 0.232 $\pm$ 0.003 & 83.1 & 21.05 & 19.74 & 0.74 & 0.55 & 0.56 & 0.09 & -20.47 & -21.11 & 9.95          & 10.25     \\
23 & SJ101723.76+390253.9 & 0.314 $\pm$ 0.004 & 75.7 & 20.26 & 18.88 & 0.62 & 0.46 & 0.55 & 0.10  & -20.50  & -21.26 & 10.13         & 10.22     \\
24 & SJ101725.11+390316.5 & 0.665 $\pm$ 0.002 & 49.7 & 20.36 & 18.80  & 0.33 & 0.24 & 0.72 & 0.14 & -20.79 & -21.66 & 10.39         & 10.59     \\
25 & SJ101730.00+385830.6 & 0.315 $\pm$ 0.010  & 75.6 & 20.91 & 19.35 & 0.74 & 0.54 & 0.72 & 0.14 & -20.6  & -21.37 & 10.2          & 10.31     \\
26 & SJ101739.82+391547.9 & 0.176 $\pm$ 0.005 & 90.0  & 21.23 & 19.33 & 1.34 & 0.97 & 0.96 & 0.21 & -21.28 & -22.05 & 10.48         & 10.69     \\
27 & SJ101742.42+390135.8 & 0.554 $\pm$ 0.011 & 58.2 & 21.25 & 20.05 & 0.18 & 0.14 & 0.48 & 0.06 & -19.50  & -20.23 & 9.70           & 9.96      \\
28 & SJ101742.99+390105.4 & 0.330 $\pm$ 0.009  & 74.5  & 21.23 & 19.39 & 0.75 & 0.55 & 0.90  & 0.20  & -20.52 & -21.44 & 10.34         & 10.43     \\
29 & SJ101809.25+390716.6 & 0.698 $\pm$ 0.011 & 46.9 & 20.33 & 18.87 & 0.32 & 0.23 & 0.66 & 0.12 & -20.74 & -21.56 & 10.32         & 10.52     \\
30 & SJ162510.56+424028.8 & 0.505 $\pm$ 0.001 & 61.8 & 20.35 & 19.18 & 0.39 & 0.29 & 0.45 & 0.06 & -20.32 & -20.99 & 9.93          & 10.22     \\
31 & SJ162558.03+425319.4 & 0.465 $\pm$ 0.002 & 64.6 & 19.04 & 17.53 & 0.69 & 0.50  & 0.62 & 0.12 & -21.86 & -22.66 & 10.74         & 10.85     \\
32 & SJ162607.94+424215.9 & 0.510 $\pm$ 0.004  & 61.4 & 21.71 & 20.62 & 0.34 & 0.26 & 0.39 & 0.04 & -18.89 & -19.52 & 9.30           & 9.81      \\
33 & SJ162618.09+423808.9 & 0.545 $\pm$ 0.001 & 58.8 & 20.72 & 19.20  & 0.49 & 0.36 & 0.68 & 0.13 & -20.32 & -21.15 & 10.16         & 10.33     \\
34 & SJ162651.30+422709.9 & 0.659 $\pm$ 0.003 & 50.2 & 21.37 & 20.27 & 0.28 & 0.21 & 0.40  & 0.04 & -19.15 & -19.80  & 9.44          & 9.92      \\
35 & SJ162652.56+422836.6 & 0.533 $\pm$ 0.004 & 59.7 & 20.77 & 19.51 & 0.39 & 0.29 & 0.52 & 0.08 & -20.38 & -21.08 & 10.00          & 10.27     \\
36 & SJ162843.80+422618.2 & 0.460 $\pm$ 0.002  & 65.0  & 20.93 & 19.91 & 0.33 & 0.25 & 0.34 & 0.02 & -19.35 & -19.96 & 9.44          & 10.12    


\end{longtable}
\end{landscape}
\twocolumn






==> galf_A2192/extra.tex <==
\appendix

\onecolumn
\getpdfpages{A963_main_TF.pdf}
\begin{landscape}
\foreach \x in {1,...,\value{pdfpages}} {
  \begin{figure}
  \centering
  \includegraphics[page=\x,scale=1.3, trim={0.5cm 0cm 0.5cm 0cm},clip]{A963_main_TF.pdf}
  \caption{The main sample in A963}
  \end{figure}}
\end{landscape}


\getpdfpages{A963_flag_TF.pdf}
\begin{landscape}
\foreach \x in {1,...,\value{pdfpages}} {
  \begin{figure}
  \centering
  \includegraphics[page=\x,scale=1.2, trim={1cm 0cm 1cm 0cm},clip]{A963_flag_TF.pdf}
  \caption{The flagged sample in A963}
  \end{figure}}
\end{landscape}



\onecolumn
\getpdfpages{A2192_main_TF.pdf}
\begin{landscape}
\foreach \x in {1,...,\value{pdfpages}} {
  \begin{figure}
  \centering
  \includegraphics[page=\x,scale=1.3, trim={0.5cm 0cm 0.5cm 0cm},clip]{A2192_main_TF.pdf}
  \caption{The main sample in A2192}
  \end{figure}}
\end{landscape}


\getpdfpages{A2192_flag_TF.pdf}
\begin{landscape}
\foreach \x in {1,...,\value{pdfpages}} {
  \begin{figure}
  \centering
  \includegraphics[page=\x,scale=1.2, trim={1cm 0cm 1cm 0cm},clip]{A2192_flag_TF.pdf}
  \caption{The flagged sample in A2192}
  \end{figure}}
\end{landscape}

==> sigma_offset.tex <==
\textit{W20 R} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  -8.15  $\pm$ 0.24  &  -0.49  $\pm$  0.6  & 4.31  &  0.37  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -8.15  (fixed)  &  -0.49  $\pm$  0.04  & 4.31  &  0.37  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -8.15  (fixed)  &  -0.7  $\pm$  0.05  & 8.29  &  0.76  &  3.28  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -8.15  (fixed)  &  -1.08  $\pm$  0.08  & 2.44  &  0.32  &  6.6  &  4.03  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -8.15  (fixed)  &  -0.36  $\pm$  0.07  & 7.88  &  0.63  &  1.61  &  3.95  &  6.77  & $\times$  &  $\times$    \\ 
A2192 main  &  -8.15  (fixed)  &  -0.64  $\pm$  0.1  & 8.03  &  0.55  &  1.39  &  0.54  &  3.44  & 2.29  &  $\times$    \\ 
BUDHIES All  &  -8.15  (fixed)  &  -0.59  $\pm$  0.04  & 8.59  &  0.74  &  1.77  &  1.72  &  5.48  & 2.85  &  0.46    \\ 
\textit{W50 R} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  -8.61  $\pm$ 0.26  &  0.6  $\pm$  0.64  & 4.46  &  0.39  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -8.61  (fixed)  &  0.6  $\pm$  0.04  & 4.46  &  0.39  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -8.61  (fixed)  &  -0.03  $\pm$  0.07  & 1.62  &  0.43  &  7.81  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -8.61  (fixed)  &  -0.02  $\pm$  0.09  & 1.45  &  0.28  &  6.3  &  0.09  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -8.61  (fixed)  &  0.6  $\pm$  0.09  & 3.04  &  0.47  &  0.0  &  5.53  &  4.87  & $\times$  &  $\times$    \\ 
A2192 main  &  -8.61  (fixed)  &  0.62  $\pm$  0.1  & 4.62  &  0.41  &  0.19  &  5.33  &  4.76  & 0.15  &  $\times$    \\ 
BUDHIES All  &  -8.61  (fixed)  &  0.19  $\pm$  0.05  & 2.91  &  0.54  &  6.4  &  2.56  &  2.04  & 3.98  &  3.85    \\ 
\textit{W50 R TFq} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  -7.99  $\pm$ 0.25  &  -0.73  $\pm$  0.64  & 5.3  &  0.4  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -7.99  (fixed)  &  -0.73  $\pm$  0.04  & 5.3  &  0.4  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -7.99  (fixed)  &  -1.4  $\pm$  0.06  & 2.03  &  0.45  &  9.29  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -7.99  (fixed)  &  -1.33  $\pm$  0.08  & 2.04  &  0.31  &  6.71  &  0.7  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -7.99  (fixed)  &  -0.82  $\pm$  0.08  & 3.22  &  0.45  &  1.01  &  5.8  &  4.51  & $\times$  &  $\times$    \\ 
A2192 main  &  -7.99  (fixed)  &  -0.79  $\pm$  0.09  & 4.75  &  0.38  &  0.61  &  5.64  &  4.48  & 0.25  &  $\times$    \\ 
BUDHIES All  &  -7.99  (fixed)  &  -1.19  $\pm$  0.05  & 3.23  &  0.53  &  7.18  &  2.69  &  1.48  & 3.92  &  3.89    \\ 
\textit{W20 B} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  -7.79  $\pm$ 0.23  &  -0.34  $\pm$  0.59  & 8.04  &  0.48  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -7.79  (fixed)  &  -0.34  $\pm$  0.04  & 8.04  &  0.48  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -7.79  (fixed)  &  -0.87  $\pm$  0.05  & 9.11  &  0.76  &  8.28  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -7.79  (fixed)  &  -1.19  $\pm$  0.07  & 3.26  &  0.35  &  10.54  &  3.72  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -7.79  (fixed)  &  -0.54  $\pm$  0.07  & 7.99  &  0.6  &  2.48  &  3.84  &  6.57  & $\times$  &  $\times$    \\ 
A2192 main  &  -7.79  (fixed)  &  -0.8  $\pm$  0.09  & 9.13  &  0.56  &  4.67  &  0.68  &  3.42  & 2.28  &  $\times$    \\ 
BUDHIES All  &  -7.79  (fixed)  &  -0.76  $\pm$  0.04  & 9.23  &  0.73  &  7.42  &  1.72  &  5.33  & 2.73  &  0.41    \\ 
\textit{W50 B} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  -8.17  $\pm$ 0.26  &  0.59  $\pm$  0.63  & 7.56  &  0.49  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -8.17  (fixed)  &  0.59  $\pm$  0.04  & 7.56  &  0.49  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -8.17  (fixed)  &  -0.33  $\pm$  0.06  & 2.06  &  0.46  &  12.76  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -8.17  (fixed)  &  -0.29  $\pm$  0.08  & 2.26  &  0.33  &  9.84  &  0.4  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -8.17  (fixed)  &  0.25  $\pm$  0.09  & 3.46  &  0.48  &  3.45  &  5.36  &  4.48  & $\times$  &  $\times$    \\ 
A2192 main  &  -8.17  (fixed)  &  0.27  $\pm$  0.09  & 5.73  &  0.43  &  3.25  &  5.55  &  4.65  & 0.16  &  $\times$    \\ 
BUDHIES All  &  -8.17  (fixed)  &  -0.12  $\pm$  0.05  & 3.27  &  0.54  &  11.09  &  2.69  &  1.8  & 3.59  &  3.79    \\ 
\textit{W50 B TFq} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  -7.47  $\pm$ 0.25  &  -1.01  $\pm$  0.64  & 10.54  &  0.53  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  -7.47  (fixed)  &  -1.01  $\pm$  0.03  & 10.54  &  0.53  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  -7.47  (fixed)  &  -1.95  $\pm$  0.06  & 2.62  &  0.47  &  14.01  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  -7.47  (fixed)  &  -1.86  $\pm$  0.08  & 2.66  &  0.33  &  9.95  &  0.9  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  -7.47  (fixed)  &  -1.42  $\pm$  0.08  & 3.77  &  0.45  &  4.8  &  5.3  &  3.89  & $\times$  &  $\times$    \\ 
A2192 main  &  -7.47  (fixed)  &  -1.39  $\pm$  0.08  & 5.95  &  0.4  &  4.45  &  5.6  &  4.15  & 0.27  &  $\times$    \\ 
BUDHIES All  &  -7.47  (fixed)  &  -1.76  $\pm$  0.05  & 3.75  &  0.53  &  12.86  &  2.43  &  1.06  & 3.6  &  3.92    \\ 
\textit{STFr V20: U} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  3.77  $\pm$ 0.11  &  1.91  $\pm$  0.3  & 3.2  &  0.15  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.77  (fixed)  &  1.91  $\pm$  0.02  & 3.2  &  0.15  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.77  (fixed)  &  1.74  $\pm$  0.02  & 7.08  &  0.32  &  6.01  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.77  (fixed)  &  1.94  $\pm$  0.04  & 1.94  &  0.13  &  0.67  &  4.47  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.77  (fixed)  &  1.6  $\pm$  0.03  & 7.64  &  0.29  &  8.6  &  3.88  &  6.8  & $\times$  &  $\times$    \\ 
A2192 main  &  3.77  (fixed)  &  1.73  $\pm$  0.04  & 6.49  &  0.23  &  4.02  &  0.22  &  3.71  & 2.6  &  $\times$    \\ 
BUDHIES All  &  3.77  (fixed)  &  1.69  $\pm$  0.02  & 7.52  &  0.32  &  7.78  &  1.77  &  5.59  & 2.5  &  0.89    \\ 
\textit{STFr V50: U} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  4.01  $\pm$ 0.12  &  1.4  $\pm$  0.31  & 3.71  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  4.01  (fixed)  &  1.4  $\pm$  0.02  & 3.71  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  4.01  (fixed)  &  1.45  $\pm$  0.03  & 1.1  &  0.17  &  1.39  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  4.01  (fixed)  &  1.45  $\pm$  0.04  & 0.81  &  0.1  &  1.12  &  0.0  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  4.01  (fixed)  &  1.13  $\pm$  0.04  & 2.3  &  0.19  &  6.04  &  6.4  &  5.66  & $\times$  &  $\times$    \\ 
A2192 main  &  4.01  (fixed)  &  1.12  $\pm$  0.04  & 2.64  &  0.14  &  6.26  &  6.6  &  5.83  & 0.18  &  $\times$    \\ 
BUDHIES All  &  4.01  (fixed)  &  1.29  $\pm$  0.02  & 5.61  &  0.29  &  3.89  &  4.44  &  3.58  & 3.58  &  3.8    \\ 
\textit{STFr V50 TFq: U} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  4.14  $\pm$ 0.13  &  0.98  $\pm$  0.31  & 3.73  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  4.14  (fixed)  &  0.98  $\pm$  0.02  & 3.73  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  4.14  (fixed)  &  1.02  $\pm$  0.03  & 1.07  &  0.17  &  1.11  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  4.14  (fixed)  &  1.02  $\pm$  0.04  & 0.93  &  0.11  &  0.89  &  0.0  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  4.14  (fixed)  &  0.69  $\pm$  0.04  & 2.06  &  0.19  &  6.48  &  6.6  &  5.83  & $\times$  &  $\times$    \\ 
A2192 main  &  4.14  (fixed)  &  0.68  $\pm$  0.05  & 2.18  &  0.14  &  5.57  &  5.83  &  5.31  & 0.16  &  $\times$    \\ 
BUDHIES All  &  4.14  (fixed)  &  0.85  $\pm$  0.02  & 5.11  &  0.29  &  4.6  &  4.71  &  3.8  & 3.58  &  3.16    \\ 
\textit{STFr V20: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  4.18  $\pm$ 0.12  &  0.95  $\pm$  0.29  & 3.73  &  0.18  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  4.18  (fixed)  &  0.95  $\pm$  0.02  & 3.73  &  0.18  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  4.18  (fixed)  &  0.64  $\pm$  0.03  & 6.57  &  0.35  &  8.6  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  4.18  (fixed)  &  0.84  $\pm$  0.04  & 1.66  &  0.14  &  2.46  &  4.0  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  4.18  (fixed)  &  0.49  $\pm$  0.04  & 6.66  &  0.3  &  10.29  &  3.0  &  6.19  & $\times$  &  $\times$    \\ 
A2192 main  &  4.18  (fixed)  &  0.61  $\pm$  0.05  & 6.97  &  0.26  &  6.31  &  0.51  &  3.59  & 1.87  &  $\times$    \\ 
BUDHIES All  &  4.18  (fixed)  &  0.59  $\pm$  0.02  & 6.88  &  0.34  &  12.73  &  1.39  &  5.59  & 2.24  &  0.37    \\ 
\textit{STFr V50: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  4.47  $\pm$ 0.14  &  0.34  $\pm$  0.31  & 4.53  &  0.21  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  4.47  (fixed)  &  0.34  $\pm$  0.02  & 4.53  &  0.21  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  4.47  (fixed)  &  0.25  $\pm$  0.03  & 1.08  &  0.18  &  2.5  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  4.47  (fixed)  &  0.26  $\pm$  0.05  & 0.71  &  0.1  &  1.49  &  0.17  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  4.47  (fixed)  &  -0.12  $\pm$  0.05  & 2.26  &  0.21  &  8.54  &  6.35  &  5.37  & $\times$  &  $\times$    \\ 
A2192 main  &  4.47  (fixed)  &  -0.14  $\pm$  0.05  & 2.4  &  0.15  &  8.91  &  6.69  &  5.66  & 0.28  &  $\times$    \\ 
BUDHIES All  &  4.47  (fixed)  &  0.09  $\pm$  0.02  & 5.48  &  0.32  &  8.84  &  4.44  &  3.16  & 3.9  &  4.27    \\ 
\textit{STFr V50 TFq: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  4.52  $\pm$ 0.14  &  0.08  $\pm$  0.3  & 4.2  &  0.2  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  4.52  (fixed)  &  0.08  $\pm$  0.02  & 4.2  &  0.2  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  4.52  (fixed)  &  0.0  $\pm$  0.03  & 1.08  &  0.18  &  2.22  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  4.52  (fixed)  &  -0.0  $\pm$  0.05  & 0.79  &  0.11  &  1.49  &  0.0  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  4.52  (fixed)  &  -0.36  $\pm$  0.05  & 2.17  &  0.21  &  8.17  &  6.17  &  5.09  & $\times$  &  $\times$    \\ 
A2192 main  &  4.52  (fixed)  &  -0.39  $\pm$  0.05  & 2.29  &  0.15  &  8.73  &  6.69  &  5.52  & 0.42  &  $\times$    \\ 
BUDHIES All  &  4.52  (fixed)  &  -0.15  $\pm$  0.02  & 5.14  &  0.32  &  8.13  &  4.16  &  2.79  & 3.9  &  4.46    \\ 
\textit{BTFr V20: U} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  2.97  $\pm$ 0.09  &  3.8  $\pm$  0.32  & 4.46  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  2.97  (fixed)  &  3.8  $\pm$  0.01  & 4.46  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  2.97  (fixed)  &  3.81  $\pm$  0.02  & 6.84  &  0.25  &  0.45  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  2.97  (fixed)  &  3.96  $\pm$  0.03  & 1.56  &  0.09  &  5.06  &  4.16  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  2.97  (fixed)  &  3.64  $\pm$  0.03  & 6.37  &  0.21  &  5.06  &  4.71  &  7.54  & $\times$  &  $\times$    \\ 
A2192 main  &  2.97  (fixed)  &  3.72  $\pm$  0.04  & 7.79  &  0.2  &  1.94  &  2.01  &  4.8  & 1.6  &  $\times$    \\ 
BUDHIES All  &  2.97  (fixed)  &  3.75  $\pm$  0.02  & 7.46  &  0.25  &  2.24  &  2.12  &  5.82  & 3.05  &  0.67    \\ 
\textit{BTFr V50: U} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  3.17  $\pm$ 0.1  &  3.38  $\pm$  0.34  & 5.12  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.17  (fixed)  &  3.38  $\pm$  0.01  & 5.12  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.17  (fixed)  &  3.55  $\pm$  0.02  & 1.48  &  0.15  &  7.6  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.17  (fixed)  &  3.56  $\pm$  0.03  & 1.06  &  0.09  &  5.69  &  0.28  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.17  (fixed)  &  3.24  $\pm$  0.03  & 2.92  &  0.17  &  4.43  &  8.6  &  7.54  & $\times$  &  $\times$    \\ 
A2192 main  &  3.17  (fixed)  &  3.22  $\pm$  0.04  & 3.74  &  0.14  &  3.88  &  7.38  &  6.8  & 0.4  &  $\times$    \\ 
BUDHIES All  &  3.17  (fixed)  &  3.41  $\pm$  0.02  & 6.23  &  0.24  &  1.34  &  4.95  &  4.16  & 4.71  &  4.25    \\  \\
\textit{BTFr V50 TFq: U} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  3.09  $\pm$ 0.1  &  3.46  $\pm$  0.34  & 5.76  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.09  (fixed)  &  3.46  $\pm$  0.01  & 5.76  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.09  (fixed)  &  3.65  $\pm$  0.02  & 1.58  &  0.15  &  8.5  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.09  (fixed)  &  3.66  $\pm$  0.03  & 1.35  &  0.1  &  6.32  &  0.28  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.09  (fixed)  &  3.34  $\pm$  0.03  & 2.87  &  0.16  &  3.79  &  8.6  &  7.54  & $\times$  &  $\times$    \\ 
A2192 main  &  3.09  (fixed)  &  3.32  $\pm$  0.03  & 3.56  &  0.13  &  4.43  &  9.15  &  8.01  & 0.47  &  $\times$    \\ 
BUDHIES All  &  3.09  (fixed)  &  3.52  $\pm$  0.02  & 6.11  &  0.24  &  2.68  &  4.6  &  3.88  & 4.99  &  5.55    \\ 
\textit{BTFr V20: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  3.12  $\pm$ 0.09  &  3.46  $\pm$  0.31  & 4.45  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.12  (fixed)  &  3.46  $\pm$  0.01  & 4.45  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.12  (fixed)  &  3.4  $\pm$  0.02  & 6.67  &  0.26  &  2.68  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.12  (fixed)  &  3.54  $\pm$  0.03  & 1.59  &  0.1  &  2.53  &  3.88  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.12  (fixed)  &  3.21  $\pm$  0.03  & 5.75  &  0.21  &  7.91  &  5.27  &  7.78  & $\times$  &  $\times$    \\ 
A2192 main  &  3.12  (fixed)  &  3.28  $\pm$  0.04  & 8.45  &  0.21  &  4.37  &  2.68  &  5.2  & 1.4  &  $\times$    \\ 
BUDHIES All  &  3.12  (fixed)  &  3.34  $\pm$  0.02  & 7.22  &  0.26  &  5.37  &  2.12  &  5.55  & 3.61  &  1.34    \\ 
\textit{BTFr V50: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  3.35  $\pm$ 0.1  &  2.97  $\pm$  0.33  & 5.54  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.35  (fixed)  &  2.97  $\pm$  0.02  & 5.54  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.35  (fixed)  &  3.07  $\pm$  0.03  & 1.76  &  0.17  &  2.77  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.35  (fixed)  &  3.08  $\pm$  0.03  & 1.41  &  0.11  &  3.05  &  0.24  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.35  (fixed)  &  2.72  $\pm$  0.03  & 2.99  &  0.18  &  6.93  &  8.25  &  8.49  & $\times$  &  $\times$    \\ 
A2192 main  &  3.35  (fixed)  &  2.69  $\pm$  0.04  & 3.48  &  0.14  &  6.26  &  7.6  &  7.8  & 0.6  &  $\times$    \\ 
BUDHIES All  &  3.35  (fixed)  &  2.94  $\pm$  0.02  & 6.47  &  0.26  &  1.06  &  3.61  &  3.88  & 6.1  &  5.59    \\ 
\textit{BTFr V50 TFq: Z} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  3.23  $\pm$ 0.1  &  3.14  $\pm$  0.33  & 6.12  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  3.23  (fixed)  &  3.14  $\pm$  0.01  & 6.12  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
A963 All  &  3.23  (fixed)  &  3.27  $\pm$  0.02  & 1.97  &  0.18  &  5.81  &  $\times$  &  $\times$  & $\times$  &  $\times$    \\ 
A963 main  &  3.23  (fixed)  &  3.29  $\pm$  0.03  & 1.87  &  0.12  &  4.74  &  0.55  &  $\times$  & $\times$  &  $\times$    \\ 
A2192 All  &  3.23  (fixed)  &  2.93  $\pm$  0.03  & 3.08  &  0.18  &  6.64  &  9.43  &  8.49  & $\times$  &  $\times$    \\ 
A2192 main  &  3.23  (fixed)  &  2.9  $\pm$  0.04  & 3.58  &  0.13  &  5.82  &  8.27  &  7.8  & 0.6  &  $\times$    \\ 
BUDHIES All  &  3.23  (fixed)  &  3.15  $\pm$  0.02  & 6.54  &  0.25  &  0.45  &  4.24  &  3.88  & 6.1  &  5.59    \\ 

==> tab_old_param.tex <==
\begin{longtable}{c | c  c  c  c  c | c  c  c  c  c}

\caption{\label{fitparams} Parameters and offsets of the various TFrs.} \\

\hline \hline

& & & \textit{Parameters} & & & & & \textit{Offset comparisons}& & \\ \cline{2-11}
TFr & Count & a  & b  & $\chi^2_{\mathrm{red}}$ & Scatter & UMa & A963 All & A963 Main & A2192 All & A2192 Main \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10) & (11)\\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline


& &  & \textit{Parameters} & & & & & \textit{Offset comparisons}& & \\ \cline{2-11}
TFr & Count & a  & b  & $\chi^2_{\mathrm{red}}$ & Scatter & UMa & A963all & A963main & A2192all & A2192main \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8) & (9) & (10)  & (11)\\

\hline 
\endhead
\hline
\endfoot



\textit{\textbf{W20 R}} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  22  &  -8.15  $\pm$ 0.24  &  -0.49  $\pm$  0.6  & 4.31  &  0.37  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -8.15  (fixed)  &  -0.49  $\pm$  0.04  & 4.31  &  0.37  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -8.15  (fixed)  &  -0.63  $\pm$  0.04  & 8.18  &  0.72  &  0.14 $\pm$ 0.06  &  0.12 $\pm$ 0.06  &  \textbf{0.45} $\pm$ \textbf{0.08}  & 0.27 $\pm$ 0.08  &  0.01 $\pm$ 0.11    \\ 
BUDHIES main  &  38  &  -8.15  (fixed)  &  -0.92  $\pm$  0.06  & 5.06  &  0.47  &  \textbf{0.43} $\pm$ \textbf{0.07}  &  0.17 $\pm$ 0.08  &  0.16 $\pm$ 0.09  & \textbf{0.56} $\pm$ \textbf{0.09}  &  0.28 $\pm$ 0.12    \\ 
\textit{\textbf{W50 R}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  -8.61  $\pm$ 0.26  &  0.6  $\pm$  0.64  & 4.46  &  0.39  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -8.61  (fixed)  &  0.6  $\pm$  0.04  & 4.46  &  0.39  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -8.61  (fixed)  &  0.14  $\pm$  0.05  & 2.84  &  0.53  &  \textbf{0.46} $\pm$ \textbf{0.06}  &  0.21 $\pm$ 0.08  &  0.2 $\pm$ 0.1  & 0.46 $\pm$ 0.1  &  0.48 $\pm$ 0.11    \\ 
BUDHIES main  &  38  &  -8.61  (fixed)  &  0.25  $\pm$  0.06  & 4.39  &  0.49  &  0.35 $\pm$ 0.07  &  0.32 $\pm$ 0.08  &  0.31 $\pm$ 0.11  & 0.35 $\pm$ 0.11  &  0.37 $\pm$ 0.12    \\ 
\textit{\textbf{W50 R TFq}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  -7.99  $\pm$ 0.25  &  -0.73  $\pm$  0.64  & 5.3  &  0.4  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -7.99  (fixed)  &  -0.73  $\pm$  0.04  & 5.3  &  0.4  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -7.99  (fixed)  &  -1.2  $\pm$  0.05  & 3.2  &  0.52  &  \textbf{0.47} $\pm$ \textbf{0.06}  &  0.18 $\pm$ 0.08  &  0.18 $\pm$ 0.09  & 0.38 $\pm$ 0.09  &  0.41 $\pm$ 0.1    \\ 
BUDHIES main  &  38  &  -7.99  (fixed)  &  -1.11  $\pm$  0.06  & 4.42  &  0.45  &  \textbf{0.38} $\pm$ \textbf{0.07}  &  0.27 $\pm$ 0.08  &  0.27 $\pm$ 0.1  & 0.29 $\pm$ 0.1  &  0.32 $\pm$ 0.11    \\ 
\textit{\textbf{W20 B}} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  22  &  -7.79  $\pm$ 0.23  &  -0.34  $\pm$  0.59  & 8.04  &  0.48  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -7.79  (fixed)  &  -0.34  $\pm$  0.04  & 8.04  &  0.48  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -7.79  (fixed)  &  -0.8  $\pm$  0.04  & 8.8  &  0.72  &  \textbf{0.46} $\pm$ \textbf{0.06}  &  0.12 $\pm$ 0.06  &  \textbf{0.41} $\pm$ \textbf{0.08}  & 0.26 $\pm$ 0.08  &  0.0 $\pm$ 0.1    \\ 
BUDHIES main  &  38  &  -7.79  (fixed)  &  -1.06  $\pm$  0.06  & 5.65  &  0.48  &  \textbf{0.72} $\pm$ \textbf{0.07}  &  0.14 $\pm$ 0.08  &  0.15 $\pm$ 0.09  & \textbf{0.52} $\pm$ \textbf{0.09}  &  0.26 $\pm$ 0.11    \\ 
\textit{\textbf{W50 B}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  -8.17  $\pm$ 0.26  &  0.59  $\pm$  0.63  & 7.56  &  0.49  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -8.17  (fixed)  &  0.59  $\pm$  0.04  & 7.56  &  0.49  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -8.17  (fixed)  &  -0.17  $\pm$  0.05  & 3.18  &  0.53  &  \textbf{0.76} $\pm$ \textbf{0.06}  &  0.2 $\pm$ 0.08  &  0.17 $\pm$ 0.09  & 0.42 $\pm$ 0.1  &  0.44 $\pm$ 0.1    \\ 
BUDHIES main  &  38  &  -8.17  (fixed)  &  -0.06  $\pm$  0.06  & 4.91  &  0.49  &  \textbf{0.65} $\pm$ \textbf{0.07}  &  0.31 $\pm$ 0.08  &  0.28 $\pm$ 0.1  & 0.31 $\pm$ 0.11  &  0.33 $\pm$ 0.11    \\ 
\textit{\textbf{W50 B TFq}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  -7.47  $\pm$ 0.25  &  -1.01  $\pm$  0.64  & 10.54  &  0.53  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  -7.47  (fixed)  &  -1.01  $\pm$  0.03  & 10.54  &  0.53  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  -7.47  (fixed)  &  -1.76  $\pm$  0.04  & 3.77  &  0.53  &  \textbf{0.75} $\pm$ \textbf{0.05}  &  0.16 $\pm$ 0.06  &  0.14 $\pm$ 0.09  & 0.34 $\pm$ 0.09  &  0.37 $\pm$ 0.09    \\ 
BUDHIES main  &  38  &  -7.47  (fixed)  &  -1.67  $\pm$  0.06  & 4.87  &  0.44  &  \textbf{0.66} $\pm$ \textbf{0.07}  &  0.25 $\pm$ 0.08  &  0.23 $\pm$ 0.1  & 0.25 $\pm$ 0.1  &  0.28 $\pm$ 0.1    \\ 
\textit{\textbf{STFr V20: U}} & & & & & & & & & \\ \cline{1-1}  
UMa (free)  &  22  &  3.77  $\pm$ 0.11  &  1.91  $\pm$  0.3  & 3.2  &  0.15  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.77  (fixed)  &  1.91  $\pm$  0.02  & 3.2  &  0.15  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.77  (fixed)  &  1.71  $\pm$  0.02  & 7.15  &  0.31  &  \textbf{0.2} $\pm$ \textbf{0.03}  &  0.04 $\pm$ 0.03  &  \textbf{0.22} $\pm$ \textbf{0.04}  & 0.11 $\pm$ 0.04  &  0.02 $\pm$ 0.04    \\ 
BUDHIES main  &  38  &  3.77  (fixed)  &  1.86  $\pm$  0.03  & 4.6  &  0.21  &  0.05 $\pm$ 0.04  &  0.11 $\pm$ 0.04  &  0.07 $\pm$ 0.04  & \textbf{0.26} $\pm$ \textbf{0.04}  &  0.13 $\pm$ 0.05    \\ 
\textit{\textbf{STFr V50: U}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  4.01  $\pm$ 0.12  &  1.4  $\pm$  0.31  & 3.71  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  4.01  (fixed)  &  1.4  $\pm$  0.02  & 3.71  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  4.01  (fixed)  &  1.31  $\pm$  0.02  & 5.38  &  0.29  &  0.09 $\pm$ 0.03  &  0.15 $\pm$ 0.04  &  0.16 $\pm$ 0.04  & 0.18 $\pm$ 0.04  &  0.19 $\pm$ 0.04    \\ 
BUDHIES main  &  38  &  4.01  (fixed)  &  1.31  $\pm$  0.03  & 3.9  &  0.21  &  0.09 $\pm$ 0.04  &  0.15 $\pm$ 0.04  &  0.16 $\pm$ 0.05  & 0.18 $\pm$ 0.05  &  0.19 $\pm$ 0.05    \\ 
\textit{\textbf{STFr V50 TFq: U}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  4.14  $\pm$ 0.13  &  0.98  $\pm$  0.31  & 3.73  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  4.14  (fixed)  &  0.98  $\pm$  0.02  & 3.73  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  4.14  (fixed)  &  0.87  $\pm$  0.02  & 4.86  &  0.28  &  0.11 $\pm$ 0.03  &  0.15 $\pm$ 0.04  &  0.16 $\pm$ 0.04  & 0.18 $\pm$ 0.04  &  0.19 $\pm$ 0.05    \\ 
BUDHIES main  &  38  &  4.14  (fixed)  &  0.87  $\pm$  0.03  & 3.7  &  0.21  &  0.11 $\pm$ 0.04  &  0.15 $\pm$ 0.04  &  0.16 $\pm$ 0.05  & 0.18 $\pm$ 0.05  &  0.19 $\pm$ 0.06    \\ 
\textit{\textbf{STFr V20: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  4.18  $\pm$ 0.12  &  0.95  $\pm$  0.29  & 3.73  &  0.18  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  4.18  (fixed)  &  0.95  $\pm$  0.02  & 3.73  &  0.18  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  4.18  (fixed)  &  0.61  $\pm$  0.02  & 6.55  &  0.33  &  \textbf{0.34} $\pm$ \textbf{0.03}  &  0.05 $\pm$ 0.04  &  0.22 $\pm$ 0.04  & 0.12 $\pm$ 0.04  &  0.0 $\pm$ 0.05    \\ 
BUDHIES main  &  38  &  4.18  (fixed)  &  0.75  $\pm$  0.03  & 4.55  &  0.23  &  \textbf{0.2} $\pm$ \textbf{0.04}  &  0.09 $\pm$ 0.04  &  0.08 $\pm$ 0.05  & \textbf{0.26} $\pm$ \textbf{0.05}  &  0.14 $\pm$ 0.06    \\ 
\textit{\textbf{STFr V50: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  4.47  $\pm$ 0.14  &  0.34  $\pm$  0.31  & 4.53  &  0.21  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  4.47  (fixed)  &  0.34  $\pm$  0.02  & 4.53  &  0.21  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  4.47  (fixed)  &  0.11  $\pm$  0.02  & 5.24  &  0.32  &  \textbf{0.23} $\pm$ \textbf{0.03}  &  0.15 $\pm$ 0.04  &  0.17 $\pm$ 0.05  & 0.23 $\pm$ 0.05  &  0.25 $\pm$ 0.05    \\ 
BUDHIES main  &  38  &  4.47  (fixed)  &  0.08  $\pm$  0.03  & 4.13  &  0.24  &  \textbf{0.26} $\pm$ \textbf{0.04}  &  0.18 $\pm$ 0.04  &  0.2 $\pm$ 0.06  & 0.2 $\pm$ 0.06  &  0.22 $\pm$ 0.06    \\ 
\textit{\textbf{STFr V50 TFq: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  4.52  $\pm$ 0.14  &  0.08  $\pm$  0.3  & 4.2  &  0.2  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  4.52  (fixed)  &  0.08  $\pm$  0.02  & 4.2  &  0.2  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  4.52  (fixed)  &  -0.14  $\pm$  0.02  & 4.89  &  0.31  &  \textbf{0.22} $\pm$ \textbf{0.03}  &  0.15 $\pm$ 0.04  &  0.16 $\pm$ 0.05  & 0.22 $\pm$ 0.05  &  0.25 $\pm$ 0.05    \\ 
BUDHIES main  &  38  &  4.52  (fixed)  &  -0.17  $\pm$  0.03  & 3.91  &  0.24  &  \textbf{0.25} $\pm$ \textbf{0.04}  &  0.18 $\pm$ 0.04  &  0.19 $\pm$ 0.06  & 0.19 $\pm$ 0.06  &  0.22 $\pm$ 0.06    \\ 
\textit{\textbf{BTFr V20: U}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  2.97  $\pm$ 0.09  &  3.8  $\pm$  0.32  & 4.46  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  2.97  (fixed)  &  3.8  $\pm$  0.01  & 4.46  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  2.97  (fixed)  &  3.76  $\pm$  0.01  & 7.16  &  0.25  &  0.04 $\pm$ 0.01  &  0.06 $\pm$ 0.02  &  \textbf{0.19} $\pm$ \textbf{0.03}  & 0.12 $\pm$ 0.03  &  0.04 $\pm$ 0.04    \\ 
BUDHIES main  &  38  &  2.97  (fixed)  &  3.87  $\pm$  0.02  & 5.7  &  0.18  &  0.07 $\pm$ 0.02  &  0.05 $\pm$ 0.03  &  0.08 $\pm$ 0.04  & \textbf{0.23} $\pm$ \textbf{0.04}  &  0.15 $\pm$ 0.04    \\ 
\textit{\textbf{BTFr V50: U}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  3.17  $\pm$ 0.1  &  3.38  $\pm$  0.34  & 5.12  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.17  (fixed)  &  3.38  $\pm$  0.01  & 5.12  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.17  (fixed)  &  3.43  $\pm$  0.02  & 6.04  &  0.24  &  0.05 $\pm$ 0.02  &  0.12 $\pm$ 0.03  &  0.14 $\pm$ 0.04  & \textbf{0.19} $\pm$ \textbf{0.04}  &  0.21 $\pm$ 0.04    \\ 
BUDHIES main  &  38  &  3.17  (fixed)  &  3.41  $\pm$  0.02  & 5.88  &  0.21  &  0.03 $\pm$ 0.02  &  0.14 $\pm$ 0.03  &  0.16 $\pm$ 0.04  & 0.17 $\pm$ 0.04  &  0.19 $\pm$ 0.04    \\ 
\textit{\textbf{BTFr V50 TFq: U}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  3.09  $\pm$ 0.1  &  3.46  $\pm$  0.34  & 5.76  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.09  (fixed)  &  3.46  $\pm$  0.01  & 5.76  &  0.16  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.09  (fixed)  &  3.53  $\pm$  0.02  & 5.9  &  0.23  &  0.07 $\pm$ 0.02  &  0.12 $\pm$ 0.03  &  0.14 $\pm$ 0.04  & \textbf{0.19} $\pm$ \textbf{0.04}  &  \textbf{0.21} $\pm$ \textbf{0.04}    \\ 
BUDHIES main  &  38  &  3.09  (fixed)  &  3.51  $\pm$  0.02  & 6.27  &  0.21  &  0.05 $\pm$ 0.02  &  0.14 $\pm$ 0.03  &  0.16 $\pm$ 0.04  & 0.17 $\pm$ 0.04  &  \textbf{0.19} $\pm$ \textbf{0.04}    \\ 
\textit{\textbf{BTFr V20: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  3.12  $\pm$ 0.09  &  3.46  $\pm$  0.31  & 4.45  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.12  (fixed)  &  3.46  $\pm$  0.01  & 4.45  &  0.14  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.12  (fixed)  &  3.35  $\pm$  0.02  & 6.91  &  0.25  &  0.11 $\pm$ 0.02  &  0.06 $\pm$ 0.03  &  \textbf{0.19} $\pm$ \textbf{0.04}  & 0.14 $\pm$ 0.04  &  0.07 $\pm$ 0.04    \\ 
BUDHIES main  &  38  &  3.12  (fixed)  &  3.44  $\pm$  0.02  & 6.03  &  0.2  &  0.02 $\pm$ 0.02  &  0.03 $\pm$ 0.03  &  0.1 $\pm$ 0.04  & \textbf{0.23} $\pm$ \textbf{0.04}  &  0.16 $\pm$ 0.04    \\ 
\textit{\textbf{BTFr V50: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  3.35  $\pm$ 0.1  &  2.97  $\pm$  0.33  & 5.54  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.35  (fixed)  &  2.97  $\pm$  0.02  & 5.54  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.35  (fixed)  &  2.95  $\pm$  0.02  & 6.25  &  0.26  &  0.02 $\pm$ 0.03  &  0.12 $\pm$ 0.03  &  0.14 $\pm$ 0.04  & \textbf{0.23} $\pm$ \textbf{0.04}  &  \textbf{0.26} $\pm$ \textbf{0.04}    \\ 
BUDHIES main  &  38  &  3.35  (fixed)  &  2.91  $\pm$  0.03  & 6.73  &  0.23  &  0.06 $\pm$ 0.04  &  0.16 $\pm$ 0.04  &  0.18 $\pm$ 0.04  & 0.19 $\pm$ 0.04  &  0.22 $\pm$ 0.05    \\ 
\textit{\textbf{BTFr V50 TFq: Z}} & & & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  3.23  $\pm$ 0.1  &  3.14  $\pm$  0.33  & 6.12  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
UMa  &  22  &  3.23  (fixed)  &  3.14  $\pm$  0.01  & 6.12  &  0.17  &  -  &  -  &  -  & -  &  -    \\ 
BUDHIES All  &  38  &  3.23  (fixed)  &  3.16  $\pm$  0.02  & 6.31  &  0.25  &  0.02 $\pm$ 0.02  &  0.12 $\pm$ 0.03  &  0.14 $\pm$ 0.04  & \textbf{0.23} $\pm$ \textbf{0.04}  &  \textbf{0.26} $\pm$ \textbf{0.04}    \\ 
BUDHIES main  &  38  &  3.23  (fixed)  &  3.12  $\pm$  0.02  & 7.25  &  0.23  &  0.02 $\pm$ 0.02  &  \textbf{0.16} $\pm$ \textbf{0.03}  &  0.18 $\pm$ 0.04  & \textbf{0.19} $\pm$ \textbf{0.04}  &  0.22 $\pm$ 0.04    \\ 


\end{longtable}

==> thesischap.tex <==

\chapter{\b\ V: The Baryonic Tully-Fisher relation 2.5 Gyrs ago based on direct \H\ detections}

\label{ch:tfr}
\addthumb{\b\ V: The Baryonic Tully-Fisher relation 2.5 Gyrs ago based on direct \H\ detections}{\Large \bf \thechapter}{ch_voidsde_fg}{ch3}

% \addcontentsline{toc}{chapter}{Dark energy and cosmic voids}
\chapterauthors{
Avanti Gogate\footnote{Kapteyn Astronomical Institute, University of Groningen, PO box 800, 9700AV, Groningen},
Marc Verheijen$^a$,
Thijs van der Hulst$^a$
Yara Jaff\'e\footnote{Instituto de F\'isica y Astronom\'ia, Universidad de Valpara\'iso, Avda. Gran Breta\~na 1111, Casilla 5030, Valpara\'iso, Chile},
}

\chapterpublish{
Submitted, under review.
}


\newpage

\hspace{0pt}
\vfill

\section*{Abstract}

We present \H-based B- and R-band Tully-Fisher relations (TFrs) and the Baryonic TFr (BTFr) at z$\sim$0.2 using direct \H\ detections from the Blind Ultra-Deep \H\ Environmental Survey (\b). Deep photometry from the Isaac Newton Telescope was used for 36 out of 166 \H\ sources, matching the quality criteria required for a robust TFr analysis. Two velocity definitions at 20\% and 50\% of the peak flux were measured from the global \H\ profiles and adopted as proxies for the rotational velocities. We compare our results with an identically constructed z=0 TFr from the Ursa Major association of galaxies. All the samples were treated identically regarding sample selection and corrections applied to ensure an unbiased comparison of the TFr. We provide an atlas and catalogues showcasing the properties of the galaxies. Our analysis is focused on the zero points of the TFr and BTFr with their slopes fixed to the z=0 relation. Our main results are: (1) The \b\ sample consists of shallower and more asymmetric \H\ profiles than UMa, which is likely due to the environment in which the galaxies reside, (2) The luminosity-based z$\sim$0.2 TFrs are brighter and bluer than the z=0 TFrs, even when cluster galaxies are excluded from the \b\ sample, (3) The BTFr shows no evolution in its zero point over the past 2.5 billion years and does not significantly change on inclusion of cluster galaxies, and (4) Proper sample selection and consistent corrections are crucial for an unbiased analysis of the evolution of the TFr.

\vfill
\hspace{0pt}

\newpage

\section{Introduction}

In the past few decades, several efforts have been made to improve our understanding of fundamental scaling relations between various properties of galaxies. For rotationally supported systems, i.e. for regular, late-type disc galaxies, the Tully-Fisher relation \citep[TFr,][]{Tully_Fisher77} is one such scaling relation, correlating two observed quantities of galaxies: the intrinsic luminosity, which is a proxy for the stellar mass of the galaxy, and the width of an emission line from the interstellar medium (ISM), which is directly linked to the galaxy's rotational velocity. It is now also general practice to study other manifestations of the TFr, such as the Stellar-mass TFr (STFr) and the Baryonic TFr (BTFr), by converting the luminosity and gas content of a galaxy into derived quantities such as stellar and baryonic masses. Rotational velocities can be inferred from various distance independent, kinematic measures such as the width of a global profile and the amplitude of a rotation curve \citep[see][]{Verheijen01, Ponomareva17,Lelli19}. While the TFr is standardly studied using galaxies with regular, disc-like morphologies, it is found that early-type and S0 galaxies in the Local Universe also follow a similar relation \citep[see][]{Trujillo-Gomez11,Cortese14}. In theory, however, an offset in the zero-point of the TFr for early-types can be expected due to the higher stellar Mass-to-Light ratios (M/L) of their older stellar populations. This has also been confirmed by a number of studies \citep{Bedregal06, Aragon-Salamanca06, Williams10, Davis11, denHeijer15}. Furthermore, massive, compact galaxies tend to have declining rotation curves, resulting in the measured global profile width to over-estimate the circular velocity of the dark matter halo \citep{Casertano91, Noordermeer07}, which also results in an offset of the zero point.


The TFr has been used extensively for distance measurements, wherein the distance modulus to disc galaxies can be recovered from the TFr if their distance independent rotational velocities are measured properly. The observed and intrinsic scatter in the TFr, however, leads to uncertainties in the inferred distances and several studies have tried to quantify and reduce this scatter to thereby attain the tightest TFr. Using distances derived from the TFr, the Hubble constant \citep[see][]{Schombert20} as well as local cosmic flows have been studied \citep{Kashibadze08,Tully13,Boruah20,Kourkchi20}. %for this part: Lelli 2019).
Additionally, the TFr is a useful tool to provide constraints for numerical simulations of galaxy formation \citep{Navarro00,Dutton07, Vogelsberger14, Schaye15, Maccio16}, wherein the slope, scatter and zero point of the TFr need to be accurately reproduced at various cosmic epochs in order to verify the plausibility of galaxy formation scenarios. The TFr may also provide insights into internal galaxy structure and kinematics, such as the prevalence of warps and non-circular motions \citep{Franx92}.


In the Local Universe, it is general practice to use the 21-cm atomic hydrogen (\H) emission line for TFr studies. \H\ proves to be an excellent tracer of galaxy dynamics due to several factors; firstly, \H\ discs generally extend much farther out than stellar discs and in most cases, probe the outer, flat part of the rotation curve, which provides the ideal velocity measurement for a TFr study. Secondly, atomic gas has a lower velocity dispersion compared to ionised gas and hence is more directly associated with circular velocities. Thirdly, it also has a relatively constant surface density and a high area-covering factor. Notably, several \H-based TFr studies using spatially resolved rotation curves have been carried out in the recent past \citep[e.g.,][]{Verheijen01,Ponomareva16,Noordermeer07,deblok14}, providing more accurate measures of the circular velocity compared to the corrected width of the global profile.


One drawback of using \H\ measurements, however, is that \H\ emission is intrinsically weak and, therefore, its detectability is restricted to the Local Universe. At higher redshifts, \H\ becomes increasingly difficult to detect with the current generation of radio telescopes, thus requiring extremely long integration times. Consequently, \H\ surveys carried out beyond the Local Universe are limited in number \citep{Fernandez13,Hoppmann15,Gogate20,Catinella15}. So far, \citep{Catinella15} have presented the only other study of the BTFr at an intermediate redshift (z$\sim$0.3) using targeted \H\ observations. Their sample of extremely massive and luminous galaxies, optically selected from the Sloan Digital Sky Survey (SDSS, \citealp{York00}) seems to follow the z=0 BTFr from \citet{Catinella12} and \citet{McGaugh00}. However, no fits were made to this sample or offsets quantified, and this study is hence considered arbitrary. 


With an increase in the amount of observational data sets over the past decade, several TFr studies of galaxy samples have been carried out using other emission line tracers of a galaxy's kinematics, such as  H\textsc{$\alpha$}, H\textsc{$\beta$},  O\textsc{ii} and O\textsc{iii} and CO \citep{Dickey92, Schoniger94,Tutui97, Lavezzi98, Tutui01, Ho07, Davis11, Tiley16}. All these tracers are usually confined to the inner, star forming regions of galaxies and typically do not accurately probe the circular velocity of the Dark Matter halo. While several TFr studies have been carried out beyond the Local Universe using optical emission lines \citep{Conselice05, Flores06, Kassin07, Puech08, Jaffe11a}, only one CO-based TFr study \citep{Topal18} exists to date. At intermediate redshifts, CO is a preferred kinematic tracer as compared to ionised gas due to its lower intrinsic velocity dispersion, while its emission line is relatively brighter compared to \H.
% and stronger correlation with the stellar component of galaxies, given that the CO emission extends beyond the peak of the rotation curve.  (I don't know what you mean here).


Despite the plethora of information on the TFr at intermediate and high redshifts, there is no convergence yet on the results for the redshift evolution of the TFr (see discussion in Sect. \ref{redshiftevol}). Inconsistencies in the TFr parameters are often encountered in the literature, due to factors such as the choice of tracer and differences in photometric bands, sample selection and size, methodology adopted for the measurement of galaxy properties, corrections applied to the data etc., %The choice of kinematic tracer can lead to systematic differences in the statistical properties of the TFr,
making it particularly difficult to consistently compare and study the evolution of the TFr slope, scatter and zero point over cosmic time. Consequently, these observational and selection biases often tend to introduce systematic offsets, which could be mistaken for an intrinsic evolution in the parameters of the TFr. For instance, \citet{Verheijen&Sancisi01} found that a galaxy with an uncertainty of just 1 degree on the measured inclination alone could lead to a scatter of 0.04 magnitudes (assuming a slope of -10). Another study by \citet{Bedregal06} indicates a downward shift of the Local TFr \citep[adopted in their case, from ][]{Tully00} by about 1.2 mags for a sample of lenticular galaxies, emphasising the importance of selecting proper comparison samples. For an unbiased TFr comparison, one has to ensure that the methodology adopted for measuring and correcting the observed galaxy properties used in the TFr is consistent, since it is the relative offsets between these properties that are of significance \citep{Ponomareva17}. While the observed scatter in the TFr can be minimised when using a carefully selected sample of regular, disc-like systems with extended, flat rotation curves or clear double-horned global profiles, the same cannot be expected for studies of galaxy samples at higher redshifts due to, for example, the use of a kinematically hot tracer with limited radial extent, survey limitations such as poor spatial and velocity resolution or smaller sample sizes and uncertainties in the measurement of inclinations. % Sorce16 talks about sample size using Eagle


In this chapter, we aim to provide, for the first time, a meaningful and detailed comparison of the \H-based TFr and BTFr at z=0 and z=0.2 in a careful and consistent manner using a blind \H\ sample, namely the Blind Ultra-Deep \H\ Environmental Survey \citep[\b,][referred to as Paper 1 hereafter]{Gogate20}. \b\ was undertaken using the Westerbork Synthesis Radio Telescope (WSRT) and is one of the first blind \H\ imaging surveys at z > 0.1. The surveyed volume includes a range of cosmic environments, effectively encompassing a total volume of 73,400 Mpc$^3$ with a depth of 328 Mpc and covering a redshift range of 0.164 < z < 0.224. From the 166 direct \H\ detections, a subset of suitable galaxies was chosen to represent the \b\ TF sample. With this study, we present the first thorough analysis of an \H-based TFr by comparing our results to the z=0 \H-based TFr from a previous study of the Ursa Major association of galaxies \citep{Verheijen01}. The data reduction procedures and extraction of galaxy properties were carried out in an identical manner for both samples, which is crucial for a proper analysis. Our goal is to also present the effect on the observed statistical properties of the TFr due to the choice of corrections and prescriptions applied to the observables. It is our objective to provide this study as a reference for the next-generation \H\ surveys that will be able to study the \H-based TFr out to higher redshifts. 


Sect. \ref{data} describes the \b\ sample and the TFr sample down-selection process. The rigorous sample selection process is given in Sect. \ref{sampsel}. In Sect. \ref{corr}, we describe the corrections applied to the data. The \H\ and optical catalogues as well as an atlas containing the various observed properties of the \b\ TF galaxies, are presented in Sect. \ref{atlas_tf}. Sect. \ref{results_tf} provides the main results from this study. Finally, we discuss our findings in Sect. \ref{discussion} and summarise our work in Sect. \ref{summary}. Throughout this chapter, we assume a $\Lambda$CDM cosmology, with $\mathrm{\Omega_{M}}$ = 0.3, $\Omega_{\Lambda}$ = 0.7 and a Hubble constant H$_0$ = 70 km s$^{-1}$ Mpc$^{-1}$. All magnitudes used in this chapter are Vega magnitudes.

%\textcolor{cyan}{ I would like to insert the following points but I am not sure where to do so without breaking the flow of the intro.\\
%1. \\}% pt1 ref:Christensen2017,topal2018

\newpage
\section{The Data}\label{data}

\subsection{The \b\ data}


\b\ is a blind \H\ imaging survey undertaken with the primary aim of providing an \H\ perspective on the so-called Butcher-Oemler (BO) effect \citep{BO84} at an intermediate redshift of z $\simeq$ 0.2, corresponding to a look-back time of $\sim 2.5$ Gyr. To this effect, the survey was centred on two galaxy clusters: Abell 963 at z $= 0.206$, which is a massive, virialised, lensing BO cluster with a large fraction (19\%) of blue galaxies in its core and strong in X-ray emission from the Intra-Cluster Medium (ICM), and Abell 2192 at z $= 0.188$, which is a much smaller, non-BO cluster still in the process of forming and weak in X-rays. The two surveyed volumes also include the large-scale structure in which the clusters are embedded. The volumes within the Abell radii of these clusters occupy as little as 4 percent of the total surveyed volume, which is 73,400 Mpc$^3$ within the Full Width at Quarter Maximum (FWQM) of the primary beam. The average angular resolution of \b\ is \ang{;;23}$\times$\ang{;;38} (corresponding to 65 $\times$ 107 kpc$^2$ at z$\sim$0.164) while the rest-frame velocity resolution is 19 \kms. The achieved \H\ mass limits at the redshifts of the clusters and in the field centres is 2 $\times$ 10$^9$ \msun\ at the redshift of the two clusters, for an emission line width of 150 \kms. A total of 127 galaxies with confirmed optical counterparts were detected in \H\ in the cube containing Abell 963 (A963 hereafter), while 39 \H-detected galaxies were identified in the cube containing Abell 2192 (A2192 hereafter).


Apart from the \H\ data, a deep B- and R-band imaging survey of the two fields was carried out with the Isaac Newton Telescope (INT), which was utilised for counterpart identification, photometry, assessing optical morphologies as well as estimating inclinations. Additionally, u, g, r, i, z photometry as well as optical spectroscopy from the SDSS is available for the two fields. Other supporting data include deep GALEX NUV and FUV imaging, spectroscopic redshifts from the William Herschel Telescope \citep[WHT,][]{Yara1_13} and CO observations using the Large Millimeter Telescope \citep[LMT,][]{Cybulski16}. These data, however, have not been used in this chapter. Details on the \b\ data processing, source finding and stellar counterpart identification can be found in Paper 1. 


\subsection{Reference studies from the literature}\label{litsamp}

For comparison with the Local Universe TFr, we adopt \citet{Verheijen01}'s study of the Ursa Major association of galaxies (UMa, hereafter). In particular, we adopt the global \H\ profiles of the 22 UMa galaxies for which the amplitude of the outer flat part of the \H\ rotation curve could be measured from spatially resolved \H\ synthesis imaging data obtained with the WSRT \citep{Verheijen&Sancisi01}, and for which photometric imaging data is available in the B, R, I and K'-band \citep{Tully96}. These UMa galaxies are nearly equidistant at 18.6 Mpc \citep{Tully00}, consistent with the average of the Cosmicflows-3 distances \citep{Tully16} to the 22 individual galaxies as provided by the Extragalactic Distance Database\footnote[1]{available at https://edd.ifa.hawaii.edu} \citep{Tully09}. The radio and photometric data reduction and analysis procedures used for the \b\ sample and those employed by \citet{Verheijen01} are essentially identical. Note that the UMa BRIK' and the INT B- and R-band images for the two \b\ fields are significantly deeper than the SDSS images. From his analysis, \citet{Verheijen01} found that the K'-band TFr using rotational velocities derived from the outer flat part of the rotation curves has the tightest correlation; however, for an unresolved \H\ study, the R-band TFr using corrected global \H\ line widths as proxies for rotational velocities is the preferred choice. While other, more recent \H-based z=0 TFr studies exist \citep[e.g.,][]{Ponomareva16,Lelli19}, we chose the UMa sample because of its many observational similarities with \b\ such as similar \H\ data sets, both obtained with the WSRT, and the availability of B- and R-band photometric images. Moreover, the UMa sample is volume-limited and complete to a limiting magnitude of m$_{zw}$=15.2 for late-type galaxies, while the data reduction procedures are identical to ours.


For a cursory high-redshift comparison we use the HIGHz sample by \citet{Catinella15}, which is a targeted \H\ survey with Arecibo and consists of 39 isolated galaxies optically selected from the SDSS, covering a redshift range of 0.17 $<$ z $<$ 0.25. These galaxies were selected to represent a sample of extremely massive, luminous, and star-forming galaxies at z > 0.16. From a preliminary analysis they found that these rare galaxies lie on the local BTFr adopted from \citet{Catinella12}, suggesting that they are scaled-up versions of local disc galaxies. To make this sample available for our comparative study, the SDSS photometry of these 39 galaxies was re-extracted from the DR7 database and transformed to Johnson-B and Cousins-R bands using the transformation equations by \citet{Cook14}. While the \H\ and photometric data acquisitions by \citet{Catinella15} differ from those for the \b\ and UMa samples, we consistently applied identical corrections to the line widths and photometry (see Sect. \ref{corr}) for all three samples. It is to be noted that the comparisons with the HIGHz sample is limited in scope, firstly due to the absence of direct B- and R- band photometry, which is required for a consistent analysis, and secondly because $\mathrm{W_{20}}$ line widths are unavailable for the HIGHz sample, which is also a key aspect of this chapter. Lastly, a reliable quantification of the offset from the z=0 TFr for the HIGHz sample is impossible due to the limited ranges in the luminosities and $\mathrm{W_{50}}$ line widths. Thus, the HIGHz sample is used for illustrative purposes only in the various figures that follow.




\section{Sample selection} \label{sampsel}

For a robust TFr study, one of the fundamental requirements is to be able to accurately measure the rotational velocities of the Dark Matter halos of galaxies.  In the Local Universe, this is best achieved with resolved \H\ studies, which can provide rotational velocities from the \H\ rotation curves of galaxies.  Flat, extended rotation curves are generally exhibited by late-type, rotationally supported disc galaxies, whereas smaller, irregular systems usually exhibit rising rotation curves up to the outermost measured radius, and are unsuitable for a TFr analysis.  A galaxy with a flat rotation curve is typified by a classic "double-horned" \H\ profile, with steep profile edges.  However, for blind \H\ imaging at intermediate redshifts, such as \b, galaxies are only marginally resolved at best, making rotation curve measurements unattainable.  For this study, therefore, rotational velocities were inferred from \H\ global profile measurements.  The corrected \H\ profile line widths at 20\% and 50\% of the peak flux are often used as proxies for the rotational velocities at the flat part of the rotation curve (see Sect.  \ref{velmeasure} for a further discussion).  This makes it necessary to carefully select galaxies with larger inclinations and suitable \H\ profiles.  We constructed two sub-samples from the parent sample of 166 galaxies, as described below. A full break-down of the galaxies rejected at every stage of the sample selection is provided as supplementary material online.


\subsection{The Tully-Fisher Sample (\textit{TFS})} \label{TFSsample}

This \b\ sub-sample was constructed based on a qualitative inspection of the optical images and an objective assessment of the \H\ profile shapes. Galaxies were rejected up-front due to the following observational and qualitative constraints:\\





\noindent
\textbf{A. Qualitative observational rejection criteria:} 
\begin{itemize}[align=left,
   leftmargin=2.4em,
   itemindent=0pt,
   labelsep=2pt,
   labelwidth=2em]
    \item[A1.] Galaxies with global \H\ profiles that are cut-off at the edges of the observed WSRT bandpass
    \item[A2.] Galaxies that lie outside the field-of-view of the INT mosaic
    \item[A3.] Galaxies with corrupted or uncertain INT photometry due to imaging artefacts from nearby bright stars, with stars superimposed on the optical image of the galaxy, or with nearby, overlapping companion(s). 
\end{itemize}

\noindent
\textbf{B. Rejection criteria based on optical morphologies or potential confusion of the stellar counterpart:}
\begin{itemize}[align=left,
   leftmargin=2.4em,
   itemindent=0pt,
   labelsep=2pt,
   labelwidth=2em]
    \item[B1.] \H\ detections with multiple nearby, UV-bright companions within the WSRT synthesized beam that lack an optical redshift.  Such cases do not allow for an unambiguous identification of the stellar counterpart of an \H\ detection. 
    \item[B2.] Galaxies with obvious disturbed optical morphologies such as tidal features or strong asymmetries.  The \H\ gas in these galaxies is likely not on circular orbits while the optical morphologies preclude an accurate measurement of the inclination.
\end{itemize}

\noindent
\textbf{C. \H\ profile shapes:}\\
Galaxies with Gaussian or strongly asymmetric \H\ profiles were rejected. An automated profile classifier was constructed which compared the maximum fluxes in three equally-spaced velocity bins of the \H\ profiles and classified them into five categories: Double-Horned (type 1), Single-Gaussian (type 2), Boxy (type 3), Skewed Boxy (type 4) and Asymmetric (type 5). We retained types 1, 3 and 4, in an effort to ensure the inclusion of only galaxies with steep \H\ profile edges.\\

\noindent
\textbf{D. Inclinations:} \\
Finally, the inclinations of the galaxies that were not rejected by the criteria mentioned above were computed. Since inclinations based on our SExtractor photometry were not very robust, the galaxies were modelled with \textit{galfit} \citep{Peng10}.  Parameters computed by SExtractor were used as the initial estimates required by \textit{galfit}. We fit S\'ersic models to all our galaxies. From the axis ratios (b/a) returned by \textit{galfit}, inclinations were calculated following:

\begin{equation}
     \mathrm{cos \: i = \sqrt{\frac{(\textit{b}/\textit{a})^2 - q_0^2}{1- q_0^2}}}
\end{equation}
 
\noindent
where \textit{a} and \textit{b} are the semi-major and semi-minor axes of the model ellipse and the disc thickness (q$_0$) was chosen to be 0.2. For consistency with other comparison samples, galaxies with an inclination more face-on than 45$^\circ$ were rejected.

This resulted in a sample of 36 galaxies, largely based on criteria aimed at avoiding missing or corrupt measurements, preventing the confusion or blending of possible stellar counterparts, rejecting kinematically disturbed gas discs, and ensuring that the width of the global \H\ profile is a good proxy for the flat part of the rotation curve. Of these 36 galaxies, 29 belong to A963 and 7 belong to A2192 (note that A963 and A2192 refer to the entire survey volume, not the Abell clusters themselves) 


\subsection{ The High-Quality Sample (\textit{HQS})}

 From the 36 galaxies in the \textit{TFS}, we constructed a high-quality sub-sample by applying three additional quantitative criteria to the global \H\ profile shapes. This was done to ensure the best possible comparison with the high-quality data of the UMa sample. These criteria concern the signal-to-noise, symmetry and shape of the \H\ profiles and are described below. \\%For the 36 galaxies in the \textit{TFS}, we further assessed the quality and shapes of the global \H\ profiles. This was done in order to minimize the involvement of a subjective selection method and ensure the inclusion of good quality, steep and symmetric profiles by imposing the following quantitative criteria.}\\


\noindent    
\textbf{E. Quantitative rejection criteria:} \\

\noindent
Galaxies were rejected based on their \H\ properties subject to pre-defined quantitative thresholds:

\begin{itemize}[align=left,
   leftmargin=2.4em,
   itemindent=0pt,
   labelsep=2pt,
   labelwidth=2em]
    \item[E1.] \textit{Signal-to-noise of the \H\ profiles}: To ensure an accurate measurement of the widths of the global \H\ profiles, we imposed a threshold on the \H\ profile line width uncertainties and rejected galaxies with uncertainties in excess of 10\% of the respective line widths.\\
 
    \item[E2.] \textit{Symmetry of the \H\ profiles}: Galaxies with asymmetric \H\ profiles do not provide robust line width measurements. One method of assessing an asymmetric profile is to assess the systemic velocities (V$_{\mathrm{sys}}$) derived from the \wot\ and \wof\ line widths. If this difference $\delta$V$_{\mathrm{sys}}$ is large, then the profile is most likely asymmetric. Based on our assessment, galaxies with absolute fractional differences in V$_{\mathrm{sys}}$ following |\;$\delta$V$_{\mathrm{sys}}$/\wot\;| > 0.05 were rejected. \\
 
    \item[E3.] \textit{Steepness of the \H\ profile edges}: To assess the steepness of the \H\ profile edges, the differences in \wot\ and \wof\ were considered. Based on our assessment, galaxies with (\wot\ - \wof)\;>\; 50 \kms\ were rejected.
\end{itemize}

\noindent
These stricter, objective criteria on the quality of the global profiles resulted in the rejection of 17 more galaxies and yielded a sample of 19 galaxies, of which 12 galaxies are from the A963 volume and 7 galaxies are from the A2192 volume. 


    
%\noindent    
%\textbf{C. Quantitative criteria:} \\
%Galaxies were rejected based on their HI properties subject to pre-defined quantitative thresholds:
%\begin{itemize}[align=left,
   %leftmargin=2em,
   %itemindent=0pt,
   %labelsep=2pt,
   %labelwidth=1em]
    %\item[1.] \textit{Signal-to-noise in HI profiles}: To ensure the exclusion of low SNR galaxies, those with errors on the line widths (both \wot and \wof) > 10 \% were rejected. \\
 
    %\item[2.] \textit{Symmetry in HI profiles}: Galaxies with asymmetric HI profiles are do not provide robust line widths measurements. One measure of an asymmetric profile is to assess the systemic velocities (V$_{\mathrm{sys}}$) derived from the \wot and \wof line widths. If the differences are large, the profile is most likely asymmetric. Based on our assessment, galaxies with absolute fractional differences in V$_{\mathrm{sys}}$ i.e. |$\delta$V$_{\mathrm{sys}}$/\wot| > 0.05 were rejected. \\
 
    %\item[3.] \textit{Steepness in HI profiles}: To inspect the steepness of the HI profile, the differences in \wot and \wof were taken into account. Based on our assessment, we applied a cut of 50 \kms\ on  \wot - \wof, and galaxies above this cut were rejected. \\
 
    %\item[4.] \textit{Inclinations}: Finally, the inclinations of the galaxies that made it past the first three criteria were computed. Since inclinations based on our SExtractor photometry were not very robust, the galaxies were modelled with \textit{galfit} \citep{Peng10}.  Parameters computed from SExtractor formed the basis of the initial estimates required by \textit{galfit}. We fit S\'ersic models for all our galaxies. From the axis ratios (b/a) returned by \textit{galfit}, inclinations were calculated following:
    
    %\begin{equation}
     %\mathrm{cos \: i = \sqrt{\frac{(b/a)^2 - q_0^2}{1- q_0^2}}}
    %\end{equation}
 
    %Where \textit{a} and \textit{b} are the semi-major and semi-minor axes of the model ellipse and the disc thickness (q$_0$) was chosen to be 0.2. For consistency with other comparative samples, an inclination cut of 45$^\circ$ was set. Galaxies with i < 45$^\circ$ were rejected.
    %\end{itemize}

%\noindent
%This selection exercise resulted in 22 galaxies in \textit{MS}, with 14 galaxies from A963 and 8 galaxies from A2192.  The galaxies are numbered based on the original catalogues presented from Paper 1. The properties of the galaxies in the \textit{MS} are provided in Sect \ref{atlas}. 

%\subsection{The "Qualitative Sample" or "QS"}
%The selection criteria that made the \textit{MS} were meticulously set up to minimise subjective selection bias. However, as expected with small samples \citep[see][]{Sorce16}, questions could arise about the plausibility of the offsets (or the lack of) observed from the fiducial TFr. To investigate this further, we appended the MS by qualitatively reviewing some of the galaxies rejected at stages C.1, C.2 and C.3 of the selection criteria in Sect. \ref{ms}. At stage C.1, the criterion was relaxed to include galaxies with errors on both \wot and \wof < 15 \%. Stages C.2 and C.3 were eliminated, while C.4. was maintained. The HI profiles of these galaxies were re-assessed visually. This relaxation of the selection criteria resulted in 12 extra galaxies that, along with the MS, made up the \textit{"Qualitative Sample"} or \textit{"QS"}. The \textit{QS} consists of 34 galaxies, which are highlighted in Table A1. The properties of these galaxies are also provided in Sect. \ref{atlas}.



\subsection{Literature samples}

For the UMa sample we used the "RC/FD" sample of 22 galaxies from \citet{Verheijen01} for which spatially resolved \H\ rotation curves confirm that the corrected widths of the corresponding global \H\ profiles properly represent their rotational velocities. These UMa galaxies abide by the same qualitative selection criteria as the \b\ \textit{HQS} galaxies. Due to some limitations of the HIGHz sample (see Sect. \ref{litsamp}), it was not used for a quantitative assessment of the TFr. All the galaxies in the HIGHz sample with inclinations above 45$^\circ$, however, are included in the illustrations of the $\mathrm{W_{50}}$ TFrs in this chapter. 


\section{Corrections to the data}\label{corr}

Before Tully-Fisher relations can be constructed, the observed \H\ line widths W$\mathrm{^{obs}_{\%}}$ and total apparent magnitudes m$\mathrm{^{obs}_{B,R}}$ need to be corrected for various instrumental, astrophysical and geometric effects such as finite spectral resolution, turbulent motions of the gas, Galactic and internal extinction, k-corrections and inclination. We ensure that these corrections are applied consistently to all galaxies in the \b, UMa and HIGHz samples. In this section we describe these corrections in some detail.


\subsection{Correction to the observed \H\ linewidths}\label{widthcorr}

\subsubsection{Conversion to rest-frame line widths}

For the \b\ galaxies, the observed widths of the redshifted global \H\ profiles were measured in MHz at 20\% and 50\% of the peak flux ($\Delta \nu_{\%}^{obs}$) and converted to observed, uncorrected rest-frame line widths (W$\mathrm{_{\%}^{obs}}$) in \kms\ using the following equation.


%\begin{figure}
%\includegraphics[trim={1.2cm 5.5cm 2.3cm 7cm},clip, width=0.65\linewidth]{chapter3/img_update/linewidth_frac_diff.pdf}
%\caption{Fractional differences in the HI line widths, defined as ($\mathrm{W_{20}}$-$\mathrm{W_{50}}$)/$\mathrm{W_{20}}$ for the various comparison samples.  The colours and markers used to represent the samples are identical to Figure \ref{fig:cmd} and are also provided in the legend. Additionally, an HI sample from VLA observations of the Perseus-Pisces filament (grey diamonds) is also included in the figure (Bilimogga et al., in prep). From top to bottom: (a) fractional differences in observed line widths, (b) after correcting for instrumental broadening, (c) for turbulent motion, (d) for inclination. Panel (e) illustrates the fractional differences in the corrected line widths as a function of the average Signal-to-Noise Ratio (SNR) derived from the HI profiles for the BUDHIES volumes.}
%\label{fig:fracdiff1}
%\end{figure}









\begin{equation}
    \mathrm{W_{\%}^{obs}=\frac{\Delta \nu_{\%}^{obs}}{\nu_{rest}} (1+z) c}
\end{equation}

\noindent
where $\mathrm{\nu_{rest}}$ is the rest frequency of the Hydrogen emission line (1420.4057517667 MHz).

For the HIGHz galaxies, \citet{Catinella15} provide observed line widths at 50\% of the peak flux, expressed as W$_{\rm 50} = \Delta$cz in \kms\ (column 6 in their Table 2), which we divide by (1+z) to obtain the observed rest-frame line widths in \kms\ such that we can consistently apply our correction for instrumental broadening as explained in the next subsection. For the galaxies in the UMa sample, we do not apply any correction for this relativistic effect and adopt the measured line widths as the rest-frame values.

% Note that the global profile widths were measured after spectrally smoothing the BUDHIES data to a Gaussian line spread function with a FWHM of four channels or 0.15625 MHz.


%\begin{figure*}
%\begin{center}
%\includegraphics[width=1\textwidth]{lupton_cook_comp.pdf}
%\caption{Comparison of instrumental INT magnitudes calculated from AUTO fluxes and SDSS model magnitudes %transformed to Johnson B and Cousins R magnitudes using Cook et al (top-left) and Lupton et al (top-right).}
%\label{fig:lup_cook}
%\end{center}
%end{figure*}

% VLA blind survey, average dist =65.5 Mpc, limiting mass = 10^8.4. Mock: 80Vmax<200, Randomly selected 

\subsubsection{Correction for instrumental broadening}

The effect of instrumental broadening on the observed line widths, caused by a finite spectral resolution R of the radio spectrometers, was corrected using the following equations, adopted from Paper 1, in which the authors studied this effect at different velocity resolutions:

\begin{equation}
    \mathrm{W_{20}^R} = \mathrm{W_{20}^{obs} - 0.36R}
\label{eq:w20corr_tf}
\end{equation}

\begin{equation}
     \mathrm{W_{50}^{R}} = \mathrm{W_{50}^{obs} - 0.29R} 
\label{eq:w50corr_tf}
\end{equation}

\noindent
For the \b\ galaxies, we measured the line widths after the data were spectrally smoothed to a Gaussian line spread function with a FWHM of four channels or 0.15625 MHz (R4, hereafter), corresponding to a rest-frame velocity resolution of R=33.0$\times$(1+z) \kms. For the UMa galaxies, the spectral resolution varied in the range R$=5.0-33.2$ \kms\ \citep{Verheijen&Sancisi01} while we adopted the rest-frame velocity resolutions for the HIGHz galaxies presented in Table 2 in \citet{Catinella15}.




\subsubsection{Correction for turbulent motion}

After correcting for instrumental velocity resolution effects, corrections for broadening due to turbulent motions of the \H\ gas were then made to the data. Following \citet{Verheijen&Sancisi01} we adopt the prescription by \citet{Tully85}, which corresponds to a linear subtraction by $w_{\rm t,\%}$ for \H\ profiles with W$_{\%}^{\rm R}$$>$$w_{\rm c,\%}$ and a quadratic subtraction if W$_{\%}^{\rm R}$$<$$w_{\rm c,\%}$ where $w_{\rm c,20}$=120 \kms\ and $w_{\rm c,50}$=100 \kms. Since all the \b\ and HIGHz galaxies in our samples have W$_{\%}^{\rm R}$$>$$w_{\rm c,\%}$, and assuming that they have monotonically rising rotation curves that properly sample the outer flat parts of the rotation curve, we adopt the values for $w_{\rm t,\%}$ from \citet{Verheijen&Sancisi01} as \\

\noindent
$w_{\rm t,20}^{\rm flat}=32$ \kms\ \;\; and \;\; $w_{\rm t,50}^{\rm flat}=15$ \kms, \\

\noindent
and thus our corrected line widths become:

\begin{equation}
     {\rm W}_{\%}^{\rm R,t} = {\rm W}_{\%}^{\rm R} - w_{\rm t,\%}^{\rm flat}
\label{eq:wturb}
\end{equation}

\noindent
Although \citet{Verheijen&Sancisi01} did not provide uncertainties related to the turbulent motion corrections, it can be noted that the values of $w_{\rm t,\%}^{\rm flat}$ in comparable studies \citep{Broeils92,Rhee96} are quite similar and hence we adopt the corresponding errors of 5 and 4 \kms\ for $w_{\rm t,20}^{\rm flat}$ and $w_{\rm t,50}^{\rm flat}$ by \citet{Broeils92} respectively.


\subsubsection{Correction for inclination}

Uncertainties in corrections involving the inclination contribute significantly to the scatter in the TFr. Hence, it is crucial, to calculate the inclinations as accurately as possible, and to propagate the corresponding uncertainties through the relevant correction formulas. Sect. \ref{TFSsample} describes our method for inferring inclinations based on the observed ellipticity $\epsilon = 1-(b/a)$ of the optical images. For completeness, we note here that \textit{galfit} takes the smoothing of the \b\ INT images due to the seeing into account while the value of $(b/a)$ as returned by \textit{galfit} pertains to the effective radius instead of a specified isophotal contour of the outer stellar disc. In case a significant spherical bulge is present in a galaxy, this approach may result in a slight overestimate of $(b/a)$ and, consequently, an underestimate of the inclination of the disc component and thereby an overestimate of the circular velocity. Table 2 lists the $(b/a)$ values for the \b\ galaxies as returned by \textit{galfit}, along with the formal errors.

For the UMa galaxies, \citet{Tully96} measured the $(b/a)$ ratio as a function of radius and selected the value that is representative of the outer disc, taking the optical morphology of the galaxy into account, including the presence of a bar, bulge and spiral arms. 
They converted this representative $(b/a)$ into an inclination using the same equation (1) and q$_0$=0.2. They assigned an uncertainty of 3 degrees to the inferred inclinations.

For the HIGHz galaxies, \citet{Catinella15} adopted the $(b/a)$ values from an exponential fit to the r-band SDSS images ($expAB_r$) in the SDSS database) and q$_0$=0.2 while employing the same equation (1) to infer an inclination. This axis ratio is representative at the effective radius of a galaxy. They do not provide an error estimate for either the $(b/a)$ values or the inferred inclinations.

Although the measurements of the optical minor-to-major axis ratio $(b/a)$ may have been slightly different for the galaxies in the three samples, the same formula and value of the intrinsic thickness q$_0$ was used in all studies. With the inferred inclinations, we corrected the already partially corrected line width according to:

\begin{equation}
    \mathrm{W^{R,t,i}_{\%}} = \frac{\mathrm{W^{R,t}_{\%}}}{\mathrm{ sin}\: i}
    \label{eq:wcorr}
\end{equation}

\noindent
where W$_{\%}^{\mathrm{R,t}}$ is the \H\ line width corrected for instrumental broadening and turbulent motion and $i$ is the inclination of the galaxy. Hereafter, we refer to $\mathrm{W^{R,t,i}_{\%}}$ as $\mathrm{W^{corr}_{\%}}$ for the sake of simplicity.


\subsection{Photometric corrections}\label{photcor}

For the \b\ sample, deep Harris B- and R-band imaging was carried out with the INT on La Palma. Photometric calibration of these images was carried out using the photometry of selected stars from the SDSS DR7 catalogue, transformed to Johnson B and Cousins R bands using the transformation equations provided by Lupton 2005\footnote[1]{http://classic.sdss.org/dr4/algorithms/sdssUBVRITransform.html} (see Paper 1). Subsequently, instrumental aperture B- and R-band magnitudes were derived with SExtractor by summing all the background subtracted pixels within adaptive Kron elliptical apertures defined by the R-band images and also applied to the B-band images. For our analysis, the resulting AUTO magnitudes from SExtractor needed to be converted to the equivalent of total model magnitudes for a consistent comparison with the other literature data sets, which consist of total extrapolated magnitudes for the UMa galaxies \citep{Tully96} or SDSS model magnitudes for the HIGHz galaxies. For this purpose, we extracted and analysed the luminosity profiles of several galaxies in the \textit{HQS}, measured the sky levels, identified the radial range where the exponential disc dominates the light, fitted an exponential profile to this radial range and calculated the total extrapolated magnitudes following \citet{Tully96}. From this exercise, we found that the differences between the SExtractor aperture (AUTO) magnitudes and our extrapolated total magnitudes were quite small: 0.038 for A963 and -0.014 for A2192. The INT aperture magnitudes were corrected accordingly to make up for these differences. Note that this statistical correction does not alter the results of our study.

To obtain intrinsic absolute magnitudes in the B- and R-bands, the total, extrapolated model magnitudes of the galaxies require further corrections for Galactic extinction, cosmological reddening and internal extinction as described below. These corrections were applied consistently to all galaxies in the three samples under consideration.

\subsubsection{Galactic extinction}

The total apparent magnitudes were corrected for Galactic extinction (A$\mathrm{^g_{B,R}}$) following \citet{Schlegel98}. The \b\ galaxies within a WSRT pointing are all close together on the sky and received the same correction according to\\

\noindent
\begin{tabular}{ l c c c}
A963  &:\; $\mathrm{A^g_{B}}$ = 0.052 & ; & $\mathrm{A^g_{R}}$ = 0.031 \\
      &                      &   &                   \\
A2192 &:\; $\mathrm{A^g_{B}}$ = 0.039 & ; & $\mathrm{A^g_{R}}$ = 0.023 \\
\end{tabular}\\

\noindent
Galactic extinction corrections for UMa galaxies were also adopted from \citet{Schlegel98} and are provided in Table 1 of \citet{Verheijen&Sancisi01}. In the case of the HIGHz sample, de-reddened SDSS magnitudes (dered\_u, dered\_g, dered\_r, dered\_i, dered\_z) were used, since they also follow \citet{Schlegel98}.

\subsubsection{K-corrections}

Corrections for cosmological reddening, known as K-corrections ($\mathrm{\kappa_{B,R}}$), were carried out with the help of the K-correction calculator by \citet{Chilingarian10}\footnote[1]{the online K-corrections calculator can be found at http://kcor.sai.msu.ru/}. This was done for both the high redshift samples. As expected, we find that the K-corrections are larger in the B-band (average $\mathrm{\kappa_B}$ = 0.65 mags) than the R-band (average $\mathrm{\kappa_{R}}$ = 0.12 mags). 


\subsubsection{Internal extinction}

Finally, the apparent magnitudes were corrected for internal extinction following \citet{Tully98}. Based on their prescription, the internal extinction correction is dependent on both the inclination and the corrected \H\ line widths of the galaxies, and is given by 

\begin{equation}
    \mathrm{A^{i}_{\mathrm{B,R}} = \gamma_{\mathrm{B,R}} \:} \mathrm{log} (a/b)
    \label{eq:intext_tully98}
\end{equation}

\noindent
were \textit{a/b} is the major-to-minor axis ratio. The $ \gamma_{\mathrm{B,R}}$ coefficient is line width dependent and calculated as

\begin{equation}
    \mathrm{\gamma_B =  1.57 + 2.75\: (log(W^{corr}_{\%}) - 2.5)} 
\end{equation} 

\begin{equation}
    \mathrm{\gamma_R = 1.15 + 1.88 \: (log(W^{corr}_{\%}) - 2.5)}
\end{equation}

\noindent
where W$^{\mathrm{corr}}_{\%}$ is the corrected \H\ line width as derived in Eq. \ref{eq:wcorr}. The final corrected magnitudes were calculated as

\begin{equation}
    \mathrm{m^{g,k,i}_{\mathrm{B,R}} = m^{obs}_{\mathrm{B,R}} - A^g_{\mathrm{B,R}} - {\kappa_\mathrm{B,R}} - A_{\mathrm{B,R}}^i}
\end{equation}

\noindent
where m$^{\mathrm{obs}}_\mathrm{{B,R}}$ is the uncorrected, total apparent magnitude. The subscripts signify the choice of filter, namely B or R. Note that this internal extinction correction method depends on both the inclination and the \H\ line width, recognising that galaxies of lower mass are usually less dusty. 


\subsubsection{Absolute magnitudes and luminosities}

Absolute B- and R-magnitudes, corrected for Galactic extinction, cosmological reddening and internal extinction, were calculated from the distance modulus equation, which takes into account the luminosity distance to each galaxy based on the adopted cosmology.

\begin{equation}
    \mathrm{M_\mathrm{B,R} = m^{g,k,i}_{\mathrm{B,R}} - 5 \:log (D_{lum}/10)}
\end{equation}

\noindent
where m$\mathrm{^{g,k,i}_{B,R}}$ is the corrected apparent magnitude, and the luminosity distance, D$_{\mathrm{lum}}$, is in parsecs. As mentioned before, a common distance of 18.6 Mpc was assumed for all galaxies in the UMa sample. Luminosities were computed from the corrected absolute magnitudes following the standard prescription, with adopted solar absolute magnitudes of M$_{\odot,B}$ = 5.31 and M$_{\odot,R}$ = 4.60.


\begin{figure*}
    \includegraphics[width=\textwidth]{chapter3/img_update/allhist.pdf}
    \caption{Histograms showing the various properties of the samples used for the TFr analysis. The \b\ samples are shown on the left. For A963, the grey histograms show the \textit{\textit{TFS}}, and the hatched cyan histograms show the \textit{HQS}. Note that the \textit{HQS} is a subset of the \textit{TFS}. For A2192, the \textit{TFS} and \textit{HQS} are identical, hence shown by the hatched magenta histograms. On the right, the histograms show the UMa and HIGHz samples, in orange and green (hatched) respectively. (a) and (b) illustrate the redshift distribution of the samples. The UMa sample is not a part of these histograms, since we assume an average distance of 18.6 Mpc, corresponding to z $\simeq$ 0. The \H\ mass distributions are shown in panels (c) and (d), while (e) and (f) illustrate the distribution of the \H\ line widths measured at 50\% of the peak flux. Lastly, panels (g) and (h) show the distribution of the cosine of the inclinations of galaxies in the various samples.}
    \label{fig:all_hist}
\end{figure*}



\subsection{Comparison of sample properties}\label{compprop}

As mentioned previously, all galaxies in the \b\ sample are selected to be isolated, \H\ rich, rotationally supported and geometrically inclined systems. In this section, some properties of the galaxy populations in the three comparison samples will be discussed. %\textcolor{red}{missing units near HI mass and luminosity/colour intervals, respectively.}

\subsubsection{Distribution of observables}

Figure \ref{fig:all_hist} presents the distributions of the various parameters for the \b\ galaxies on the left, distinguishing the \textit{HQS} galaxies in the A963 and A2192 volumes, and the reference samples of UMa and HIGHz on the right. The full \b\ \textit{TFS} (29+7 galaxies) is shown by the light-grey histogram while the \textit{HQS} galaxies are indicted with the hatched histograms for A963 (12 galaxies: teal) and A2192 (7 galaxies: magenta) separately. Note that all 7 galaxies in the \textit{TFS} of A2192 are in its \textit{HQS} as well.

The top panels ($a$) and ($b$) of Fig. \ref{fig:all_hist} show the redshift distributions of the \b\ and HIGHz galaxies. Compared to the \b\ sample, the HIGHz sample reaches slightly further in redshift, out to z=0.245, but only 2 of the 28 galaxies are beyond the maximum redshift of the \b\ sample (z=0.224). The majority of the \textit{TFS} galaxies in the \b\ sample (29 out of 36) are located in the volume containing A963, with a significant fraction of galaxies (11 out of 29) in the redshift bin that contains the large-scale structure in which A963 is embedded. The UMa sample is not shown in panel ($b$) as it is located at z=0, with an assumption that all galaxies in this sample are at a common distance of 18.6 Mpc. The HIGHz sample contains galaxies selected over a large area on the sky and, therefore, does not target a specific cosmic over-density.

Panels ($c$) and ($d$) of Fig. \ref{fig:all_hist} show the distribution of \H\ gas masses of the sample galaxies, and there are some striking differences between the samples. The \b\ galaxies have \H\ masses in the range $9.3<{\rm log(M}_{HI})<10.2$ while the UMa galaxies can have notably smaller \H\ masses, covering the range $8.7<{\rm log(M}_{HI})<9.9$. The HIGHz galaxies, however, have significantly higher \H\ masses, covering the range $10.4<{\rm log(M}_{HI})<10.9$. None of the \b\ or UMa galaxies have an \H\ mass as high as the lowest \H\ mass of any HIGHz galaxy. This is not surprising as the HIGHz galaxies were selected as the most extreme, massive \H-rich galaxies at z$>$0.16 while the global \H\ profiles of the 'code 1' galaxies from \citet{Catinella15}, that constitute the HIGHz subsample considered here, have the highest signal-to-noise and thereby a relatively high \H\ gas content.


Figure \ref{fig:all_hist}  ($e$) and ($f$) show histograms of the \H\ line width measured at 50\% of the peak flux. The fastest rotators belong to the HIGHz sample ($\langle$W$_{\rm {50}}^{\rm {corr}}\rangle=$477 \kms), which is expected since this sample is selected to contain massive and luminous galaxies. On the other hand, the distributions of the \b\ (\textit{TFS}) and UMa samples are quite similar ($\langle$W$_{\rm {50}}^{\rm {corr}}\rangle=$ 313.5 and 313.8 \kms\ respectively.) The two UMa galaxies with larger line widths are NGC 3953 and NGC 3992.

Lastly, panels ($g$) and ($h$) in Fig. \ref{fig:all_hist} illustrate the distribution of the inclinations of all our sample galaxies. Based on our sample selection criteria (see Sect. \ref{sampsel}), only galaxies with inclinations $>45^\circ$ were retained for this analysis. From the histograms, it is evident that the \b\ and UMa samples have flat distributions as expected for randomly oriented discs in a volume limited sample, whereas the HIGHz sample is biased towards more face-on systems with lower inclinations. This is an expected observational bias as galaxies with lower inclinations tend to have narrower \H\ emission lines that are easier to detect and measure.

\begin{figure}
\includegraphics[trim={0.2cm 0cm 0.5cm 1cm },clip,width=0.8\linewidth]{chapter3/img_update/CMD_w50_tully.pdf}
\caption{%\textcolor{red}{missing lable units here and other figs.}
The R-band colour-magnitude diagram of the various samples after photometric corrections have been applied. Cyan triangles represent galaxies belonging to the cluster Abell 963. Circles indicate galaxies from the foreground (FG) and background (BG) of the volume A963 (cyan) and all of the volume A2192 (magenta) which together make up the \b\ \textit{TFS} (open symbols), of which the \textit{HQS} is shown by the solid symbols.  The UMa sample is indicated by the orange stars. The HIGHz u, g, r, i magnitudes were transformed to Cousins R magnitudes using \citet{Cook14} and are shown by the green diamonds. Magnitudes were corrected using the inclination and line width dependent corrections by \citet{Tully98}. }
\label{fig:cmd}
\end{figure}



\subsubsection{The colour$-$magnitude diagram}

The rest-frame B$-$R versus M$_{\rm R}$ colour-magnitude diagram (CMD) of the three samples is shown in Fig. \ref{fig:cmd}. The magnitudes were corrected for galactic extinction, cosmological reddening and internal extinction as described in Sect. \ref{photcor}. The three samples occupy different areas in the CMD. The \b\ and UMa samples cover a similar range in absolute magnitude ($-23<{\rm M}_{\rm R}<-19$) but the \b\ galaxies ($\langle$B$-$R$\rangle=0.79$) are on average 0.26 magnitudes bluer than the UMa galaxies ($\langle$B$-$R$\rangle=1.05$) although there is considerable overlap in colour. The HIGHz galaxies ($\langle$B$-$R$\rangle=1.20$) have similar colours as the UMa galaxies but are significantly brighter ($-24<{\rm M}_{\rm R}<-23$) than the galaxies in both the \b\ and UMa samples. Only one \b\ galaxy falls in the magnitude range of the HIGHz sample. It should be recalled here that the applied correction for internal extinction not only depends on inclination but also on the corrected line width, which correlates with absolute luminosity through the TFr. This is discussed in more detail in Sect. \ref{corrdisc} as this correction for internal extinction will eventually have some impact on the slope of the TFr. The fact that the HIGHz sample is so 'disjoint' from the \b\ and UMa samples in the CMD is another motivation to consider the HIGHz sample for illustrative purposes only and exclude it from a quantitative assessment of the cosmic evolution of the TFr zero point.

\subsubsection{\H\ and stellar mass-to-light ratios}

The left panel of Fig. \ref{fig:mhil} shows the \H\ mass-to-light (\mhi/L$_{\rm R}$) ratios of the galaxies in the various samples. As expected, the \b\ and UMa galaxies show a general increasing trend in the \H\ mass-to-light ratio with decreasing luminosity. For a given magnitude, however, the \b\ galaxies tend to have a slightly higher \mhi/L$_{\rm R}$ ratio. The sample averages are $\langle{\rm log}($\mhi/L$_{\rm R)}\rangle=-0.52$ for the \b\ galaxies and $\langle{\rm log}($\mhi/L$_{\rm R})\rangle=-0.75$ for the UMa galaxies. The HIGHz galaxies do not follow the extrapolated trend to brighter magnitudes as they are overly gas rich with a sample average of $\langle{\rm log}($\mhi/L$_{\rm R})\rangle=-0.65$.

\begin{figure*}
\includegraphics[trim={2.2cm 0cm 2.5cm 0cm },clip,width=\linewidth]{chapter3/img_update/MHI_L_comps.pdf}
\caption{Comparison of R-band mass-to-light ratios for the various samples; left: \mhi/L ratios, right: \mstel/L ratios. The colours and markers used to represent the samples are identical to Figure \ref{fig:cmd} and are also provided in the legend. Stellar masses shown here are based on Eq. \ref{eq:mstar1}.}
\label{fig:mhil}
\end{figure*}



The right panel of Fig. \ref{fig:mhil} shows the maximum-disc inferred stellar mass-to-light ratio in the R-band (M$^{\rm mxd}_{\star}$/L$_{\rm R}$) according to equation \ref{eq:mstar1} as motivated in section \ref{btfr}. Since there is a rather strong dependence on the B$-$R colour, the distribution of points is similar to that in the CMD, with 0.4$<$(M$_{\star}$/L$_{\rm R}$)$<$1.6. The HIGHz galaxies have similar stellar mass-to-light ratios compared to most of the UMa galaxies. The \b\ galaxies have a notably lower stellar mass-to-light ratio with a clear trend of lower M$_{\star}$/L$_{\rm R}$ values toward fainter galaxies. The sample average values $\langle$M$_{\star}$/L$_{\rm R}\rangle$ are 0.63 for the \b\ galaxies, 0.98 for the UMa galaxies and 1.2 for the HIGHz galaxies.

\subsubsection{\H\ mass fractions}

The \H\ mass to stellar mass ratios (\mhi/\mstel) as a function of stellar mass is shown in panel (a) of Fig. \ref{fig:mratios}. Not surprisingly, we see the same trend as in the left panel of Fig. \ref{fig:mhil} where we used the R-band luminosity instead of stellar mass. We confirm the well-known trend that lower mass galaxies tend to have a larger ratio of \H-to-stellar mass while the HIGHz galaxies seem to lie above the trend defined by the \b\ and UMa galaxies, as expected given the selection criteria for the HIGH z sample. In panel(b) of Fig. \ref{fig:mratios} we plot \mhi/\mstel\ as a function of \mhi\ and note that the correlation seen in panel (a) has disappeared. The \mhi/\mstel\ ratios for the \b\ galaxies tend to be higher than for the UMa and HIGHz galaxies with sample averages of $\langle{\rm log}($\mhi/\mstel$)\rangle=-0.74$ and $-0.73$ for the UMa and HIGHz samples respectively, while $\langle{\rm log}($\mhi/\mstel$)\rangle=-0.31$ for the \b\ sample.

In panels (c) and (d) of Fig. \ref{fig:mratios} we plot the \mhi/\mbar\ fractions as a function of \mbar\ and \mhi. We observe in panel (c) that, compared to panel (a), the trend of \mhi/\mbar\ versus \mbar\ has become shallower as the \H\ mass is a larger fraction of \mbar\ for galaxies with a lower \mbar. Interestingly, in panel (d), plotting \mhi/\mbar\ versus \mhi\ instead of plotting \mhi/\mstel\ versus \mhi\ shows a significantly smaller scatter, while the HIGHz galaxies do not stand out significantly.

In panels (c) and (d) it is evident that the sample of \b\ galaxies tends to have a higher \mhi/\mstel\ ratio than the UMa and HIGHz galaxies. The sample averages for the UMa and HIGHz galaxies are $\langle{\rm log}($\mhi/\mbar$)\rangle=-0.89$ and $-0.83$ respectively, while $\langle{\rm log}($\mhi/\mbar$)\rangle=-0.58$. From Fig. \ref{fig:mratios} we conclude that the \b\ galaxies at z=0.2 are relatively more gas-rich than the UMa galaxies at z=0, even though they have similar stellar and baryonic masses.

Finally, we remark that the larger vertical spread of the UMa sample in Figs. \ref{fig:mhil} and \ref{fig:mratios} is due to the fact that the UMa sample has a better \H\ mass sensitivity than both \b\ and HIGHz, and hence includes galaxies with lower \H\ masses.

\begin{figure*}
\includegraphics[trim={2.2cm 1.5cm 2.5cm 1cm },clip,width=0.95\linewidth]{chapter3/img_update/MHI_Mstar_ratio.pdf}
\caption{Gas fractions of the galaxies in the various samples. Panels (a) and (b) show the \mhi/\mstel\ ratios as a function of \mstel\ and \mhi\ respectively, while panels (c) and (d) show the \mhi/\mbar\ ratios as a function of \mbar\ and \mhi\ respectively. The colours and markers are identical to Fig. \ref{fig:cmd}. Stellar and baryonic masses shown here are based on Eq. \ref{eq:mstar1}.}
\label{fig:mratios}
\end{figure*}



\subsubsection{\H\ profile shapes}

Ideally, the \H\ profiles of isolated spiral galaxies with suitable inclinations should have steep edges, allowing the two line width measures $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$, once properly corrected for instrumental spectral resolution, turbulent motion and inclination, to yield the same circular velocity. To inspect this notion is some detail, we compared the $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$ width of the galaxies in the various TFr samples, as illustrated in Fig \ref{fig:fracdiff1}. The figure shows the fractional differences between the observed $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$ line widths (a), and the same after accumulative corrections for instrumental resolution (b), turbulent motion (c) and inclination (d). For details on the applied corrections, see Sect. \ref{widthcorr}. Along with the \b\ \textit{TFS} and \textit{HQS} samples, we also included the UMa sample, as well as an \H\ sample from a blind VLA \H\ imaging survey of part of the Perseus-Pisces (PP) filament at a distance of 66 Mpc (Bilimogga et al., in prep). In panel (a), all samples deviate from the zero line, which is expected since the \H\ profile edges are not infinitely steep ($\mathrm{W_{20}}$$>$$\mathrm{W_{50}}$ always).

In the case of the UMa and PP samples, this offset is corrected as we move downwards to panel (c), in which the line widths are corrected for both, instrumental spectral resolution and turbulent motion. It is also immediately evident that in panel (c) there still exists an offset and a larger scatter in the \b\ samples that could not be eliminated by applying the same corrections. The offset, however, is smaller for the \textit{HQS} (solid symbols) than for the \textit{TFS} (open symbols) by merit of the more stringent, quantitative criteria applied to the profiles of the \textit{HQS} galaxies. The average fractional difference between the \wct\ and \wcf\ line widths is 0.16 for the \b\ \textit{TFS} galaxies, compared to 0.08 for the UMa galaxies. Naturally, correcting for inclination, as shown in panel (d), does not further reduce the fractional difference for any of the samples. It is important to point out in panel (e) that no trend is observed in the fractional differences as a function of the average Signal-to-Noise Ratio (SNR) of the \H\ profiles. In Sect. \ref{discussion} we address the possible reasons for this offset of the \b\ galaxies.

\begin{figure}
\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,center},capbesidewidth=6cm}}]{figure}[\FBwidth]
{\caption{%\textcolor{red}{x axes units missing, symbols too small}
Fractional differences in the \H\ line widths, defined as ($\mathrm{W_{20}}$-$\mathrm{W_{50}}$)/$\mathrm{W_{20}}$ for the various comparison samples.  The colours and markers used to represent the samples are identical to Figure \ref{fig:cmd} and are also provided in the legend. Additionally, an \H\ sample from VLA observations of the Perseus-Pisces filament (grey diamonds) is also included in the figure (Bilimogga et al., in prep). From top to bottom: (a) fractional differences in observed line widths, (b) after correcting for instrumental broadening, (c) for turbulent motion, (d) for inclination. Panel (e) illustrates the fractional differences in the corrected line widths as a function of the average Signal-to-Noise Ratio (SNR) derived from the \H\ profiles for the \b\ volumes.}\label{fig:fracdiff1}}
{\includegraphics[trim={1.2cm 5.5cm 1.5cm 7cm},clip, width=1.05\linewidth]{chapter3/img_update/linewidth_frac_diff.pdf}}
\end{figure}


Figure \ref{fig:steep} shows the histograms of the asymmetries and the shallowness of the \H\ profile edges of the \b\ and UMa galaxies. The red dashed lines indicate the applied cuts in the asymmetry and shallowness of the profiles given in Sect. \ref{sampsel} E2 and E3 respectively. It can be noted that while these thresholds do exclude \b\ galaxies with the most asymmetric profiles or shallow profile edges from the \textit{TFS}), the profiles of the \textit{HQS} galaxies are still more asymmetric and with shallower edges than the profiles of the UMa galaxies. The origin of such profiles is discussed in Sect. \ref{velmeasure}. From the UMa sample, we note that the profile of NGC 3729 is more asymmetric than the imposed threshold while NGC 4138 has a profile with shallower edges compared to the threshold applied for the selection of the \b\ \textit{HQS} galaxies.







%We refer to Fig. \ref{fig:cmd} which shows the combined CMD  This correction depends on both the inclinations as well as the corrected HI line widths of the individual galaxies. All galaxies in the CMD lie within the "blue cloud". However, in the figure, it is evident that the HIGHz galaxies, chosen to be extremely gas rich and luminous so as to be detectable out to z $\sim$ 0.3, are significantly redder than the BUDHIES sample at z $\sim$ 0.2. The cluster Abell 963 is a massive BO cluster hosting a large fraction of blue galaxies in its core, and thus we could speculate that the BUDHIES sample is unusually blue. Yet, in contrast, we could also speculate that a large number galaxies in the BUDHIES sample belong to cluster environments and thus are expected to be redder than the isolated, extremely gas-rich galaxies optically selected by \citet{Catinella15}. However, if we turn our attention to the bottom row of Fig. \ref{fig:cmd}, we can see B and R band CMDs with similar internal extinction corrections following \citet{Tully85}, which is dependent on inclination alone. Following these corrections, the difference in colour between BUDHIES and HIGHz significantly reduces, while the BUDHIES and UMa magnitudes remain relatively unchanged using either of the correction methods. We speculate that this is likely caused by a larger number of galaxies with larger inclinations (See Fig \ref{fig:all_hist} \textit{d}) in the HIGHz sample as compared to the other two. This implies that the effect of reddening is higher for such systems (cite?)




\section{The \b\ TF catalogue and atlas}\label{atlas_tf}

We present here the tables as well as an atlas containing the \H\ and optical properties of the galaxies chosen to represent the TF sample from \b. The tables include observed, corrected and inferred properties following the methodology as described in Sect. \ref{corr}. 


\begin{figure*}

    \includegraphics[trim={1cm 0cm 2cm 1cm },clip,width=0.45\linewidth]{chapter3/img_update/asymmetry.pdf} 
    \includegraphics[trim={1cm 0cm 2cm 1cm },clip,width=0.45\linewidth]{chapter3/img_update/steepness.pdf} 
    
    \caption{%\textcolor{red}{(Fig 6, right panel: the quantity on the x-axis must be the absolute value of W20-W50, since this difference is negative for a few galaxies (Fig 5).)}
    Histograms comparing the \H\ properties of the comparison samples; the open histogram shows the \textit{TFS} while the hatched histogram shows the \textit{HQS} (which is a subset of the \textit{TFS}). The UMa sample is shown in orange. The red dashed lines indicate the thresholds applied during the sample selection process for creating the \textit{HQS}. Right: Histograms showing the difference in the observed line widths which is a quantification of the shallowness of the \H\ profiles; Left: histograms showing asymmetries in the form of the absolute fractional differences in the systemic velocities derived from W$\mathrm{_{20,R,obs}}$ and W$\mathrm{_{50,R,obs}}$ respectively. }
    \label{fig:steep}
\end{figure*}



\subsection{The catalogues}\label{catalogue}

The \H\ and optical catalogues for the \b\ TF sample are provided in Tables \ref{tab:A963_HI_table_tf} and \ref{tab:A963_opt_table_tf} respectively. The contents of the \H\ catalogue as presented in Table \ref{tab:A963_HI_table_tf} are as follows: \\
\textit{Column} (1): The running identification number of the galaxies for easy cross-reference with entries in Table \ref{tab:A963_opt_table_tf}.\\
\textit{Column} (2): The catalogue number assigned to these galaxies in Paper 1, for easy cross-reference to the atlas pages.\\
\textit{Column} (3): The \H\ ID which contains the Right Ascension and Declination of the \H\ source [J2000].\\
\textit{Column} (4): The rest-frame velocity resolution R at which the \H\ profile, total \H\ map and Position-Velocity diagrams were extracted from the data cubes. The velocity resolution is set at 4 $\times$ $\Delta$v (R4), where $\Delta$v is the redshift-dependent rest-frame width of the channel in \kms.\\
\textit{Column} (5): The channel-average Signal-to-Noise Ratio (SNR) of the extracted \H\ profiles of each galaxy.\\
\textit{Column} (6): The galaxy redshift based on the \H\ profile.\\
\textit{Column} (7): The luminosity distance to the galaxy, calculated using its \H\ redshift and the adopted cosmology.\\
\textit{Columns} (8) \& (9): The observed (rest frame) $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$ line widths, including their errors.\\
\textit{Column} (10) \& (11): The \wct\ and \wcf\ line widths corrected for instrumental resolution, turbulent motions and inclination, following the methodology described in Sect. \ref{corr}.\\
\textit{Column} (12): \H\ masses ($\times$ 10$^9$ \Msun) calculated from the integrated flux densities of the extracted \H\ profiles, including their uncertainties. For further details, see Paper 1.\\
\textit{Column} (13): The volume (A963 or A2192) and sample (\textit{TFS} or \textit{HQS}) that a galaxy belongs to. \\

\noindent
The contents of the optical catalogue as presented in Table \ref{tab:A963_opt_table_tf} are as follows: \\
\textit{Column} (1): The running identification number of the galaxies for easy cross-reference with entries in Table \ref{tab:A963_HI_table_tf}.\\
\textit{Column} (2): The SDSS ID of the adopted optical counterpart of the \H\ detection, indicating the optical coordinates of the galaxy.\\
\textit{Column} (3): The minor-to-major axis ratios (b/a) obtained from \textit{galfit}.\\
\textit{Column} (4): The inclination as inferred from the optical axis ratio (b/a), following Eq. (1) and assuming an intrinsic disc thickness q$_0$ of 0.2.\\
\textit{Columns} (5) \& (6): Total apparent INT B- and R- band magnitudes, respectively, including a small aperture correction as described in Sect. 4.2.\\
\textit{Columns} (7) \& (8): The k-corrections applied to the Galactic extinction corrected, apparent B- and R- band magnitudes, as described in Sect. 3.\\
\textit{Columns} (9) \& (10): The internal extinction corrections applied to the Galactic extinction and k-corrected B- and R- band magnitudes, as described in Sect. 3.\\
\textit{Columns} (11) \& (12): The corrected, absolute B- and R- band magnitudes, respectively.\\
\textit{Column} (13): Log stellar mass (\Msun) calculated using Eq. \ref{eq:mstar1}.\\
\textit{Column} (14): Log baryonic mass (\Msun) calculated from the \H\ masses in Col. (12) of Table \ref{tab:A963_HI_table_tf}, and the stellar masses in Col. (13) respectively.\\


\begin{figure*}
   \includegraphics[trim={4.5cm 1cm 3.5cm 0cm},clip,width=\textwidth]{chapter3/img/galf_A963/galfit_78_atlas.pdf}
   \includegraphics[angle =270,trim={6cm 1.5cm 10cm 3.5cm},clip,width=1\textwidth]{chapter3/img/HI_A963/HIatlas78.pdf}
\caption{An example of the layout of the atlas, showing a galaxy from the \textit{TFS}. The top row shows the optical properties and \textit{galfit} outputs, whereas the bottom panel mostly shows the \H\ properties. The atlas layout has been described in detail in Sect. \ref{atlas_tf}. The full atlas is available online.}
\label{fig:atlaslayout}
\end{figure*}


\subsection{The atlas}

The catalogue presented in Tables \ref{tab:A963_HI_table_tf} and \ref{tab:A963_opt_table_tf} is accompanied by an atlas page for each galaxy. The full atlas is available online as supplementary material. Figure \ref{fig:atlaslayout} illustrates an example of the atlas layout, consisting of two rows. The top row consists of 5 panels highlighting the optical morphology and the results from the \textit{galfit} modelling. The bottom row consists of 4 panels highlighting the \H\ data, similar to the atlas pages in Paper 1. Each panel is briefly described below. \\

\noindent From left to right, the top row displays the following:\\
\textit{Panels} (1) and (2): INT colour composite images with a hard and soft contrast, respectively. The top-left corner of panel (1) shows the catalogue number as listed in Col. (2) of Table \ref{tab:A963_HI_table_tf}.\\
\textit{Panel} (3): The optical R-band image of the galaxy. The red dashed ellipse depicts the fitting result returned by \textit{galfit} as derived at the effective radius and deconvolved for the seeing. For clarity, it is enlarged by an arbitrary factor and therefore not representative for the radius at which it is drawn.\\
\textit{Panel} (4): The resulting model as returned by \textit{galfit}.\\
\textit{Panel} (5): The residual image as returned by \textit{galfit}. \\

\noindent From left to right, the bottom row of each atlas page displays the following:\\
\textit{Panel} (1): INT R-band image (30$\times$30 arcsec$^2$) of the optical counterpart. The SDSS ID is given in the top-left corner. The optical redshift is printed in the bottom-right corner of the image for those sources with optical spectroscopy. \\
\textit{Panel} (2): A zoomed-out INT R-band image with \H\ contours from the total \H\ map overlaid in red. The \H\ ID is provided in the top-left corner. The optical centre is indicated by the orange cross while the \H\ centre is given by the red cross. The contours are set at \H\ column density levels of 1, 2, 4, 8, 16, and 32 $\times$10$^{19}$ cm$^{-2}$.  \\
\textit{Panel} (3): The Position–velocity diagram along the optical major axis, extracted from the R4 ($\sim$38 \kms) cube. The contour levels correspond to –2 (dashed), 2, 4, 6, 9, 12, 15, 20, and 25 times the local rms noise level. The mask within which the \H\ flux was determined is outlined in red. The position angle is given in the bottom-left corner of the diagram. The central frequency and the \H\ centre are given by the vertical and horizontal dashed lines, respectively. \\
\textit{Panel} (4): The global \H\ profile as extracted from the R4 cube within the mask indicated in panel (3). The frequencies corresponding to the \H\ and optical redshifts are indicated by the grey and orange arrows respectively. Further details about the data processing can be found in Paper 1.\\


\begin{figure*}
\includegraphics[trim={0.7cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/W20_B_TFr_fin.pdf}
\includegraphics[trim={0.7cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/W50_B_TFr_fin.pdf}
\includegraphics[trim={0.7cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/W20_R_TFr_fin.pdf}
\includegraphics[trim={0.7cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/W50_R_TFr_fin.pdf}
\caption{The \H-based TFrs in the two photometric bands, B (left) and R
(right). Top panel: The \H-TFrs using \wct\ and \wcf\ line widths as velocity tracers in the B-band. Bottom panel: Similar to the top panel but in the R-band. In comparison, the Local TFr \citep{Verheijen01} is shown by the orange markers and a corresponding orange best-fit line, while the orange band framing the UMa TFr represents the total observed rms scatter in the UMa data points. Overlays of the HIGHz galaxies are shown in the \wcf\ TFrs for illustrative purposes. The colours and symbols used are identical to Fig. \ref{fig:cmd}. Open (pink and cyan) symbols indicate the \textit{TFS}, while the coloured symbols represent the \textit{HQS} (which is a subset of the \textit{TFS}). The respective best fit TFrs with slopes fixed to UMa are shown by the grey and red lines. The best-fit parameters of the \textit{TFS} and \textit{HQS} TFrs are printed to the bottom-right of the sub-figures. }
\label{fig:tfr}
\end{figure*}

\begin{figure}
\includegraphics[trim={0 1 0 1.5cm},clip,width=0.9\linewidth]{chapter3/img_update/M_by_L_vs_B_R.pdf}
\caption{M$_\star$/L$_R$ vs B-R for the UMa HSB galaxies using maximum-disc fits, assuming an isothermal halo. The line of best fit is given to the top-left.}
\label{fig:umastar}
\end{figure}

\section{The Tully-Fisher Relations}\label{results_tf}

Presented in this section are the TFrs obtained using the corrected \H\ line widths as tracers of the rotational velocities, and different photometric bands as well as derived quantities such as baryonic masses. We begin with explaining the fitting methods applied to the various samples, followed by a presentation of the luminosity-based, the stellar and the baryonic TF relations using rotational velocities derived from the corrected $\mathrm{W_{20}}$ and $\mathrm{W_{50}}$ \H\ line widths.


%\begin{figure}
%    \centering
%    \includegraphics[trim={2 2 2 1.8cm},clip, width=\linewidth]{TFr_allfree.pdf}
    
%    \includegraphics[trim={2 2 2 1.8cm},clip, width=\linewidth]{BTFr_allfree50.pdf}
%    \caption{With \wcf as the velocity measure, the HI-based R-band TFr (top) and BTFr (bottom) with both the parameters of the linear regression left free. Stellar mass estimates used in the BTFr are based on Eq. \ref{eq:mstar1}. All colours and symbols are identical to Fig. \ref{fig:tfr}. The best fit parameters are printed at the bottom-right of the figures.}
%    \label{fig:allfree}
%\end{figure}




\subsection{Fitting method}

The fitting method adopted in this chapter closely resembles that of \citet{Verheijen01} and for this study, our choice of the fiducial TFr in the Local Universe is from that study as well. 

%The TFr, generally expressed by the corrected HI linewidth (W) or rotational velocity (V) on the X-axis and absolute magnitude or mass (stellar or baryonic) on the Y axis, is rotated for the purpose of line fitting such that the fit minimizes the errors on W or V in the Y-direction since these errors are more significant than the errors on the magnitudes or masses. Thus, a straight line with slope $a$ and intercept $b$ through the data, generally expressed in the form




%\begin{equation}
%    \mathrm{M = a(log W) + b}
%\end{equation}

%\noindent
%where M is the absolute magnitude or mass and log W is the velocity measure, is now expressed as 

%\begin{equation}
%    \mathrm{log W = a'M + b'}
%\end{equation}

%\noindent
%Where $a'$ and $b'$ are the slope and intercept of the inverse line respectively. 


In order to minimise the Malmquist bias, inverse, weighted-least-square fits were made to the data, identical to the procedure followed by \citet{Verheijen01}. A custom-made fitting algorithm using the python package \textit{scipy.optimize.curve\_fit} was implemented for the fitting. Uncertainties in the corrected line widths were estimated using standard error propagation of the errors on the observed line widths. Uncertainties in the model parameters featuring in the various correction formulas were not considered. Only errors in the corrected line widths were taken into account during the fitting, and the small inclination related co-variance between the errors in the corrected luminosities and in the line widths were ignored.

\subsection{The Luminosity-based TFr}\label{tfr}

The best-fit TFrs for the full \textit{TFS} with both the slope and the zero point left free and using both velocity measures \wct\ and \wcf, combined with the two photometric bands B and R are given by Eqs. \ref{eq:tfr20Bfree}, \ref{eq:tfr50Bfree}, \ref{eq:tfr20Rfree} and \ref{eq:tfr50Rfree}. 

\begin{equation}
     \mathrm{M_B = (-10.6 \pm 0.73) log (W_{20}^{R,t,i}) + (6.35 \pm 1.49)}
     \label{eq:tfr20Bfree}
\end{equation}


\begin{equation}
     \mathrm{M_B = (-8.2 \pm 0.54) log (W_{50}^{R,t,i}) + (0.14 \pm 1.39)}
     \label{eq:tfr50Bfree}
\end{equation}



\begin{equation}
    \mathrm{M_R = (-10.9 \pm 0.71) log (W_{20}^{R,t,i}) + (6.27 \pm 1.47)}
    \label{eq:tfr20Rfree}
\end{equation}


\begin{equation}
    \mathrm{M_R = (-8.4 \pm 0.54) log (W_{50}^{R,t,i})+ (-0.33 \pm 1.41)}
    \label{eq:tfr50Rfree}
\end{equation}


\medskip

\noindent
We note that the TFrs based  on the smaller \textit{HQS} are indistinguishable from the TFrs to the larger \textit{TFS} (see Sect. \ref{sampseldiscussion}) and hence are not considered here.

%\textcolor{pink}{(expand on discussion of weights given in Verheijen2001)}. The slope $a$ and zero point $b$ of the UMa line of best fit were recovered with $a = -1/a'$ and $b = -b'/a'$.

Due to the rather limited range (2.25 < log W < 2.75) and relatively larger errors on the \H\ line widths for the \b\ galaxies, however, we limit our analysis to fitting and comparing the TFr zero points only. For this purpose, fits to the \textit{TFS} and \textit{HQS} were made with the slopes fixed to the corresponding TFR of the UMa sample, which displays a significantly smaller scatter.  The parameters of the inverse TFr fits are provided in Tables \ref{tab:fitparams} and \ref{tab:fitparamsbo} (see Sect. \ref{bo}). The corresponding figures are not provided in the chapter, since our main focus is on the evolution in the TFr zero points. Note that we did not make fits to the HIGHz sample because of the very limited range in luminosity of its constituent galaxies and the lack of available W${_\mathrm{20}}$ line widths. They are instead plotted for illustrative purposes only, by including them in the various \wcf\ TFr plots. In all the figures displaying the TFrs (except Fig. \ref{fig:bo}), the TFrs for the \textit{TFS} and \textit{HQS} are shown by the \textit{grey} and \textit{red} lines respectively. All symbols and colours are kept consistent throughout the chapter except, again, for Fig. \ref{fig:bo}.

Fig. \ref{fig:tfr} presents the luminosity-based TFr fits based on the two velocity measures \wct\ (left) and \wcf\ (right), and the absolute B-band (top) and R-band (bottom) magnitudes. The slope was fit to the UMa sample and then kept fixed for the fits to the \b\ samples. In all cases we find an offset of the \b\ TFr zero point towards brighter luminosities. These offsets are smallest when using the \wct\ line widths (right panels) with 0.47$\pm$0.06 in the B-band and 0.19$\pm$0.06 R-band. The offsets in the zero point are significantly larger when using \wcf\ (left panels) with 0.72$\pm$0.06 and 0.44$\pm$0.06 in the B and R bands respectively. In all four cases, the vertical scatters are comparable, between 0.56 and 0.69 magnitudes (see Table \ref{tab:fitparams}). The numbers quoted are for the \textit{TFS}, but there are no significant differences in the zero point offsets when fitting to the \textit{TFS} or the more restrictive \textit{HQS} (again, see Table \ref{tab:fitparams}).

\begin{figure*}
\includegraphics[trim={0.5cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/BTFr20_uma_fin.pdf}
\includegraphics[trim={0.5cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/BTFr50_uma_fin}
\includegraphics[trim={0.5cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/BTFr20_zib_fin}
\includegraphics[trim={0.5cm 0 1cm 1.5cm},clip, width=0.45\linewidth]{chapter3/img_update/BTFr50_zib_fin}
\caption{BTFrs based on the two velocity measures,\wct/2 (left) and \wcf/2 (right). Baryonic masses (1.4\mhi + \mstel) were computed from two different stellar mass prescriptions, Eq. \ref{eq:mstar1} (top) and Eq. \ref{eq:mstar2} (bottom). The layout, colours and symbols are identical to Fig. \ref{fig:tfr}.}
\label{fig:btfr}
\end{figure*}


\subsection{The Baryonic TFr}\label{btfr}

For the purpose of constructing baryonic TFrs, stellar masses were calculated by converting the corrected, absolute B$-$ and R$-$band magnitudes using two different prescriptions that both involve a (B$-$R) colour term but with a different degree of dependency. With the first prescription, stellar masses (M$_\star$) were determined empirically from maximum-disc rotation curve mass decompositions \citep[][ Chapter 6]{Verheijen97} of the UMa galaxies, using K$-$band luminosity profiles  and assuming a maximum-disc fit with an isothermal dark matter halo model. The stellar masses following from these rotation curve decompositions are tabulated in \citet[][ Chapter 6]{Verheijen97} and were used to calculate R$-$band stellar mass-to-light ratios \mstel/$\mathrm{L_R}$, which are plotted versus the (B$-$R) colour of the galaxies in Fig. \ref{fig:umastar}. A mild but significant correlation is observed and represented by a linear fit, which can be expressed as

\begin{equation}
    \mathrm{M_{\star}^{mxd}\: [M_\odot]= L_R \times (1.35(B - R) - 0.399 })
     \label{eq:mstar1}
\end{equation}

\noindent
Maximum-disc-based stellar masses computed in this way for all galaxies in the comparison samples are provided in Col. (12) of Table \ref{tab:A963_opt_table_tf}.

For comparison, we also adopted an alternative stellar mass estimator, following \citet{Zibetti09}. This prescription was also adopted by \citet{Cybulski16} who calculated stellar masses for 23 \b\ galaxies using the INT B$-$ and R$-$band photometry following:

\begin{equation}
    \mathrm{M_{\star}^{zib}\: [M_\odot]= L_R \times 10^{-1.2 + 1.066 (B-R)} + 10^{0.04}}
    \label{eq:mstar2}
\end{equation}

\noindent
where the term 10$^{0.04}$ accommodates a conversion to the Kroupa IMF. Stellar masses computed using this prescription are not tabulated.



\noindent
From the estimated stellar and \H\ masses, the baryonic masses were calculated for all galaxies following:

\begin{equation}
    \mathrm{M_{bar} = M_\star + 1.4 M_{HI}}
    \label{eq:mbar}
\end{equation}

\noindent
where the factor 1.4 accounts for the contribution by Helium and metals. The velocity measures for the BTFrs are given in the form of log(2V$\mathrm{_{rot,\%}}$) for which log(W$\mathrm{^{corr}_\%}$) is an approximation. \\

\noindent
The best fit inverse BTFrs with both the slope and the zero point left free are described by:

\begin{align}
    \begin{split}\label{eq:btfrfree20}
        \mathrm{log(M_{bar}/M_\odot) = (3.7 \pm 0.23) log (\mathrm{2V_{rot,20}}) + (1.1\pm0.65)}
    \end{split}\\
    \begin{split}\label{eq:btfrfree50}
            \mathrm{log(M_{bar}/M_\odot) = (3.4 \pm 0.20) log (\mathrm{2V_{rot,50}}) + (1.89\pm0.61)}
    \end{split}
\end{align}
\medskip

\noindent
These are based on the stellar masses computed using Eq. \ref{eq:mstar1}. Again, the corresponding figures for these BTFrs are not shown, since our focus is on the zero point of the BTFrs with their slopes fixed to the BTFr of UMa. Instead, we show in Fig. \ref{fig:btfr} the BTFrs based on the two stellar mass prescriptions given by Eqs. \ref{eq:mstar1} and \ref{eq:mstar2}. The zero points of the BTFrs based on the maximum disc approach (top panels) are indistinguishable from the zero points of the UMa BTFrs, with a maximum zero point offset of 0.08 dex when using \wcf. Similar statistically insignificant differential offsets in the zero point are observed for the BTFrs using Eq. \ref{eq:mstar2} (bottom panels). These results will be discussed in detail in Sect. \ref{discussion}.


%Finally, in Fig. \ref{fig:allfree} we show, for illustrative purposes, the R-band TFr and BTFr using \wcf line widths as the velocity tracers and Eq. \ref{eq:mstar1} to derive baryonic masses, with both the slopes and zero points left free during the fitting. From the figure, it is immediately evident that the BUDHIES TFr parameters are strikingly different from the UMa TFrs, in particular, the BUDHIES "all" sample. Due to the limited range in line widths, we do not analyse these TFrs further, but proceed with the analysis based on Figs. \ref{fig:tfr} and \ref{fig:btfr}.


\begin{figure*}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/TF_z_20_B_fin.pdf}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/TF_z_50_B_fin.pdf}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/TF_z_20_R_fin.pdf}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/TF_z_50_R_fin.pdf}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/btfr_bo_uma_20.pdf}
\includegraphics[trim={0.5cm 0.5cm 1cm 1.7cm},clip, width=0.45\linewidth]{chapter3/img_update/btfr_bo_uma_50.pdf}

\caption{Top and middle: The luminosity-based TFrs for the \textit{Cluster} and \textit{Control} samples in B-band and R-bands respectively, using \wct\ (left) and \wcf\ (right). Bottom: BTFrs using the same velocity measures as the luminosity based TFrs but expressed as 2V$_{rot,20}$ (left) and 2V$_{rot,50}$ (right). The \textit{Control} sample and its corresponding TFr is shown by the pink circles and lines, while the \textit{Cluster} sample and TFr is shown by the black triangles and lines. The open and solid symbols as well as the dashed and solid lines represent the \textit{TFS} and \textit{HQS} respectively. The UMa galaxies and TFr are given in orange. The fit parameters are printed in the bottom-right of each panel.}
\label{fig:bo}
\end{figure*}

\subsection{The TFr from an environmental perspective}\label{bo}

The final versions of the TFr presented in this chapter investigate the effect of the environment on the TFr, taking advantage of the fact that the \b\ samples also include galaxies in a cluster environment. In particular, we are interested to study these environmental effects from a "Butcher-Oemler" (BO) perspective. The BO effect \citep{BO84} manifests itself as a higher fraction of blue galaxies in the cores of clusters at higher redshifts. The cluster Abell 963, part of the seminal BO paper, is a massive, lensing cluster hosting an unusual large fraction of blue galaxies in its core (f$_{\rm b}=$0.19), and is one of the nearest BO clusters. In contrast, Abell 2192, at a similar redshift as Abell 963, is a non-BO cluster with no blue galaxies associated with its core, weak in X-rays and still in the process of forming \citep[for more information on the two clusters, see][]{Yara0_12, Yara1_13,Yara2_15,Yara3_16}. Several studies of the BO effect using optical and other bands have been carried out, with varying results \citep[e.g.,][]{Couch94, Lavery86, Tran03, DePropris04,Andreon04,Andreon06,Urquhart10, Lerchester11}. While some confirmed the presence of this BO effect, others claimed it was a selection bias by preferential inclusion of brighter, bluer galaxies at higher redshifts. However, the BO effect in relation to the cold atomic gas content of galaxies has never been investigated, and this was the primary driver for the \b\ survey. Previous studies of the \b\ data have shown that none of the blue galaxies within the central 1 Mpc region of Abell 963 were detected in \H\ \citep[see][]{Verheijen07,Yara3_16}. However, we are interested to investigate whether the galaxies outside the cluster core of Abell 963 are responsible for the blueing and brightening of the TFr observed in Fig.\ref{fig:tfr}.  The advantage of having \H\ data from a BO cluster such as Abell 963 therefore allows us to study its effect on the TFr and BTFr.

For both the \textit{TFS} and \textit{HQS}, we constructed two sub-samples, distinguished by their environment. Galaxies belonging to the cluster Abell 963 alone, defined as the velocity range within 2.5$\mathrm{\sigma_{cl}}$ from the cluster recession velocity, with $\mathrm{\sigma_{cl}}$ = 933 \kms\ being the velocity dispersion of Abell 963, made up the \textit{Cluster} sub-sample, while the remainder of the galaxies in both survey volumes, consisting of those in the foreground and background of A963 as well as those in the entire A2192 survey volume, made up the \textit{Control} sub-sample. While Abell 2192 is also classified as a "cluster", we include it in the \textit{Control} sample since Abell 2192 has a much smaller velocity dispersion ($\mathrm{\sigma_{cl}}$ = 645 \kms) and a negligible intra-cluster medium (ICM) compared to Abell 963. Anyhow, only one direct \H\ detection exists within a projected distance of 1 Mpc from the cluster centre and this galaxy is not a member of the \textit{TFS}. A total of 19 galaxies from the \textit{TFS} belong to the \textit{Cluster} sub-sample, while 17 belong to the \textit{Control} sub-sample. From the \textit{HQS}, 7 and 12 galaxies belong to the \textit{Cluster} and \textit{Control} sub-samples respectively. The various environment-based TFrs and BTFrs are illustrated in Fig. \ref{fig:bo}. 

Compared to the \textit{TFS}, which consists of galaxies from all environments, the TFrs derived using the \textit{Control} sample show smaller offsets from the UMa sample in all cases. The \textit{Cluster} TFr is significantly brighter ($\Delta$R = 0.65 $\pm$ 0.09 mags) and bluer ($\Delta$(B-R) = 0.27 $\pm$ 0.12 mags) than UMa, using \wcf. The same trend, though milder, is also observed in the \textit{Control} sample, with galaxies being both brighter ($\Delta$R = 0.31 $\pm$ 0.08 mags) and bluer ($\Delta$(B-R) = 0.30 $\pm$ 0.11 mags) than UMa. The BTFrs, however, are still comparable to UMa even with the exclusion of cluster galaxies. This is discussed further in Sect. \ref{envir}.
%BO imprint on TFR, MHI/L ratios, CMD, stellar mass-HI mass plots



\subsection{Parameter table layout}\label{paramtab}
The fit results for the various TFrs in this chapter are given in Tables \ref{tab:fitparams} and \ref{tab:fitparamsbo}.
Table \ref{tab:fitparams} provides the fit parameters for the luminosity-based TFrs and BTFrs for the three samples in consideration: UMa, \textit{TFS} and \textit{HQS}. Table \ref{tab:fitparamsbo} is similar, but provides the fit parameters for the \textit{Cluster} and \textit{Control} samples (see Sect. \ref{bo}). In addition, the tables also provide the offset differences. 
Given below is a description of the columns. \\

\noindent
\textit{Column} (1) TFr: Describes which TFr has been fit. Given in bold are the headers, consisting of the TF categories, for instance, the $\mathrm{W_{20}}$-R band, $\mathrm{W_{20}}$-B band etc. The numbers given next to the headers for the  BTFrs indicate the stellar mass prescription used. $1$ represents Eq. \ref{eq:mstar1} while $2$ represents Eq. \ref{eq:mstar2}. \\
\textit{Column} (2) Count: The number of galaxies belonging to the specified sample. \\
\textit{Column} (3): The slopes with errors obtained at the time of fitting. This is true for the UMa sample. For the others, the slope is fixed to the UMa value.\\
\textit{Column} (4): The zero points with errors obtained at the time of fitting.\\
\textit{Column} (5) The reduced $\mathrm{\chi^2_{red}}$ signifying whether the observed scatter can be explained given the errors. \\
\textit{Column} (6) The total vertical rms scatter taking into account all the data points. \\
\textit{Columns} (7)  Offsets in zero points with UMa: Offsets in the zero points calculated from the re-fitted UMa line with the slope fixed to the UMa sample with all parameters left free. \\
\textit{Columns} (8)  Offset in zero point with other \b\ samples. \\


\section{Discussion}\label{discussion}

%The TFr provides a useful benchmark for gaining insight into how d As well as a goal to understand in its own right, the TFR is particularly useful as a benchmark with which to compare samples of galaxies, in order to examine the differences between them. Using this method, we can gain insight into the evolution of disc galaxies by considering the variation of the TFR with cosmic time %Bamford06
Several high redshift studies on the TFr exist (see Sect. \ref{redshiftevol}), though there are none that make use of \H\ as the choice of kinematic tracer. The only known \H\ study of the TFr beyond the Local Universe (z$>$0.1) by \citet{Catinella15} shows that an optically selected sample of extremely massive, gas rich and luminous galaxies also seems to follow the local BTFr from GASS \citep{Catinella12}; however, their work is not a dedicated TFr study and the limited range in their magnitudes and line widths does not allow further analysis.
TFr studies based on cosmological numerical simulations provide some insights into the \textit{expected} redshift evolution of the TFr, with a possibility to carefully construct a sample of suitable galaxies with accurate inclination measurements. Regardless, the number of such studies using the extended \H\ discs of galaxies to trace the evolution in the TFr is limited. Using semi-analytical models, \citet{Obreschkow09} concluded that their simulated TFrs in the Local Universe are in good agreement with the fiducial, observed TFr based on the HIPASS survey, but at higher redshifts, found an increase in the scatter and a shift in the zero points towards higher velocities for a given baryonic mass (their Fig. 14).  On the other hand, \citet{Glowacki20} studied the evolution of the BTFr using the SIMBA simulation, and found that the zero point of the BTFr at higher redshifts is shifted towards lower velocities (their Fig. 3) and only detectable for disc-like galaxies with V$_{\rm flat}$ as the kinematic measure. Thus, a proper morphological classification is abundantly important for an apt evaluation of the redshift evolution of the TFr. 

This section provides a discussion of our observational findings and presents caveats that the reader needs to keep in mind, to ensure that systematic differences in the comparison samples are not mistaken for an evolution in the TFr parameters. 




\subsection{Scatter}\label{scatter}

The differences in the scatter of the luminosity-based TFrs as presented in Fig. \ref{fig:tfr} can be the result of a number of factors, such as the choice of photometric band (B versus R), the velocity measure (\wct\ versus \wcf), the inclusion of different galaxy populations in the sample, inaccuracies in the measurement of inclinations, intrinsic differences in the kinematics and morphologies of galaxies at higher redshifts and the effect of environment on these galaxies. Interestingly, the BTFrs as presented in Fig. \ref{fig:btfr} show a notably smaller scatter, as also reported in the literature \citep[e.g.,][]{Lelli16}. In all cases, however, the z=0.2 TFrs show a larger vertical scatter compared to the z=0 TFr. Below, we explore some of the factors mentioned above in more detail.


\subsubsection{Sample selection} \label{sampseldiscussion}

Galaxies at higher redshifts are found to have larger kinematical and morphological anomalies than local galaxies \citep{Kannappan02, Flores06, Kassin07}.  In all these studies, inclusion of these galaxies with disturbed and complex morphologies introduced a large scatter in the TFr. \citet{Weiner06} and \citet{Kassin07} showed in their studies that the scatter in the stellar mass TFr was greatly reduced by adopting a kinematic estimator $S_{0.5}$, which adds a measure of disordered, non-circular motions to the rotational velocity, effectively accounting for pressure support. This empirical approach to reduce the scatter was also confirmed by simulations \citep[see, for instance, ][]{Covington09}.

In the extensive sample selection procedure adopted for this chapter (see Sect. \ref{sampsel}), our attempt was to filter out optically disturbed and interacting galaxies since our goal is to construct a robust TFr using galaxies with reliable photometry and \H\ line widths that reflect the rotational velocities as a tracer of total dynamical mass. Due to the limitations in the resolution and quality of both the \H\ and the optical data, however, it is likely that some kinematically disturbed systems may have been included in our sample selection process, despite our best efforts. 

It is noteworthy that there is almost no difference in the TFrs of the two \b\ sub-samples (\textit{HQS} and \textit{TFS}), implying that a stricter control over the \H\ properties of galaxies, in particular the symmetry of the \H\ global profile, does not significantly alter the TFr or reduce the scatter. The offsets in the zero points of the \textit{HQS} and the \textit{TFS} are given in Col. (9) of Table \ref{tab:fitparams}, and in all cases, the differences are less than 0.1 magnitude. For simplicity, we will limit the rest of the discussion to the larger \textit{TFS} alone.

%and he galaxies with the maximum dispersions belong to the "flagged samples", consisting of imperfect photometry or global profile anomalies. This does not necessarily imply the inclusion of obviously disturbed or interacting galaxies. However, due to the limited spatial resolution of our observations,  We do find that the galaxies from the BUDHIES MS (coloured points) have the least scatter. Another source of scatter could arise from the choice of velocity tracer, which is discussed separately in Sect. \ref{velmeasure}. %Another reason could be attributed to the variations in the total mass-to-light ratios of these galaxies (expand...).
%Some of the strongest outliers in all the TFrs belong to the flagged sample, which explains their larger dispersions.

\begin{figure*}
\includegraphics[trim={0cm 0.5cm 0cm 0cm },clip,width=\linewidth]{chapter3/img_update/mag_diff_t_tfq.pdf}

\caption{Difference in the absolute magnitudes based on two different internal extinction corrections for the two available photometric bands, B (left) and R (right). The magnitudes were corrected for galactic extinction, K-corrections and the internal extinction corrections were adopted from \citet{Tully98} and \citet{Tully85} respectively. The differences are plotted against the absolute magnitudes based on \citet{Tully98}, which is the standard correction used in this chapter. The colours and symbols are identical to fig. \ref{fig:cmd}. Average differences for each sample are printed to the top left of the figures.}
\label{fig:tfq_diff}
\end{figure*}



\subsubsection{Choice of corrections}\label{corrdisc}

In the previous sections, we have already stressed the importance of having homogeneous samples with consistently applied corrections to properly compare the parameters of different TFrs. Moreover, the corrections themselves affect the samples differently, depending on their underlying properties, and could play a significant role in altering the parameters of the TFr. To illustrate this, we made use of two different internal extinction correction methods. The first is from \citet[][referred to as T98]{Tully98}, which is the standard correction adopted for this chapter and described by Eq. \ref{eq:intext_tully98} in Sect. \ref{photcor}. The second is from \citet[][referred to as TFq]{Tully85} which is dependent on inclination only, and is given as follows:

%   \mathrm{ A_\mathrm{band}^{i,TFq} = -2.5 log [f(1 + e^{(-\tau_\mathrm{band} sec\; i))} + (1 - 2f)(\frac{1 - e^{(-\tau_\mathrm{band} sec \:i)}}{(\tau_\mathrm{band} sec \:i)})}]

\begin{equation}
   \mathrm{ A_\lambda^{i,TFq} = -2.5 log \left[f(1 + e^{-\tau_\lambda sec\; i}) + (1 - 2f)\left(\frac{1 - e^{-\tau_\lambda sec \:i}}{\tau_\lambda sec \:i}\right)\right]}
\end{equation}

\noindent
where, for a slab of dust containing a homogeneous mixture of stars of fraction (1 - 2f), f signifies the fraction of stars above and below this slab, while $\tau_\lambda$ gives the optical depth of the dust layer as a function of wavelength. We used f = 0.1, $\tau_B$ = 0.81 and $\tau_R$ = 0.40, taken from \citet{Verheijen97}. %, who in turn accessed these values through Tully et al (private communication).



\begin{figure*}

    \includegraphics[trim={4cm 0cm 4cm 1cm },clip,width=\linewidth]{chapter3/img_update/color_offsetcomp.pdf} 
    \includegraphics[trim={4cm 0cm 4cm 1cm },clip,width=\linewidth]{chapter3/img_update/dvsys_offsetcomp.pdf} 
    \includegraphics[trim={4cm 0cm 4cm 1cm },clip,width=\linewidth]{chapter3/img_update/w20_w50diff_offsetcomp.pdf} 
    \includegraphics[trim={4cm 0cm 4cm 1cm },clip,width=\linewidth]{chapter3/img_update/mhi_mbar_offsetcomp.pdf} 
    
    \caption{Scatter plot of the vertical offsets (difference in magnitudes) of the individual galaxies points from the luminosity-based TFr from UMa, as a function of (a) B-R colour, (b) quantified asymmetry, (c) quantified shallowness and (d) ratio of the \H\ to baryonic mass. Points lying above the dashed 'zero' line are brighter than the UMa TFr while those below are fainter. From first to the last columns are the TFrs from the two photometric bands and velocity measures: $\mathrm{W_{20}}$-M$_B$, $\mathrm{W_{20}}$-M$_R$, $\mathrm{W_{50}}$-M$_B$, $\mathrm{W_{50}}$-M$_R$. All colours and symbols are identical to Fig. \ref{fig:cmd}. }
    \label{fig:offset_col}
\end{figure*}



Shown in Fig. \ref{fig:tfq_diff} are the differences in the absolute magnitudes of the various samples, based on the two internal extinction corrections, for both photometric bands. From the figure, it can be noted that the differences are larger in the B-band than the R-band. Secondly, the corrections least affect the HIGHz sample because it consists of more face-on galaxies than \b\ and UMa. However, both UMa and \b\ show similar corrections in both the bands due to similarities in the distribution of inclinations and line widths (see Fig. \ref{fig:all_hist}) and hence these different corrections would not significantly impact the TFr results. The two extreme galaxies (no. 14 and 26 in Column (1) of Table \ref{tab:A963_HI_table_tf}) have the largest inclinations and hence the largest corrections in both bands. They were both assigned an inclination of 90$^\circ$ since the axis ratios returned by \textit{galfit} were less than 0.2, which is the assumed disc thickness. Also worth noting is that the choice of these internal extinction corrections would display different B-R colours, especially in the HIGHz sample, compared to the UMa or \b\ samples. 

Similarly, the choice of corrections applied to the line widths would also impact the TFr. For instance, the choice of turbulent motion corrections for this chapter are adopted from \citet{Verheijen&Sancisi01}, which were optimized for the UMa galaxies based on rotation curve measurements. For an unresolved sample like \b, however, there is no way of knowing if these corrections are adequate. It is important to highlight here that all the correction methods adopted for this work are applied consistently to all the comparison samples.


\subsubsection{Dependence on photometric band and colour}\label{coldisc}

Some studies such as \citet{Flores06} (z$\sim$0.6) claim to find a larger scatter in the B-band TFr compared to other bands. We find that both the K-corrections and internal extinction corrections are larger in the B-band than the R-band, and after applying these corrections the vertical scatters in the \b\ TFrs are not significantly different in the B and R bands (see Fig. \ref{fig:tfr} and Table \ref{tab:fitparams}). This implies that the choice of photometric band does not seem to affect the observed scatter in the \b\ TFrs. The applied corrections, however, do result in differences in the zero-points between the \b\ TFrs and the z=0 TFr from UMa, with the offsets being larger (brighter) in the B-band than in the R-band in all cases. This is most likely due to the B-band being significantly more sensitive to light from active star-forming regions than the R-band. Qualitatively, this is expected, since galaxies at higher redshifts are predicted to have younger stellar populations \citep[e.g.,][]{Dutton11}. The TFrs in the respective photometric bands are discussed more in detail in Sect. \ref{redshiftevol}. Furthermore, Fig. \ref{fig:offset_col} illustrates the vertical offsets (offset in magnitude) of each individual galaxy from the z=0 UMa TFr as a function of B-R colour for the two velocity tracers, \wct\ and \wcf. No significant trend is found in the scatter or offsets as a function of colour for the \b\ TFrs, although we do find a mild colour dependence for the UMa galaxies, particularly in the B-band, which the bluer \b\ galaxies seem to follow albeit with a larger scatter.


\subsubsection{Inclinations}

Improper inclination measurements are a dominant source of scatter in the TFr, and thus deserve special attention, since inclination corrections are applied not just to the kinematic measures but also to the magnitudes. Inclinations and their uncertainties are estimated in a number of ways, such as tilted ring fits to the \H\ velocity fields, \H\ disc ellipticities, and from optical axis ratios. For the \b\ data, the axis ratios were computed from Sersic models fit to the R-band images of the galaxies using \textit{galfit}. These axis ratios were converted to inclinations using a disc thickness (q$_0$) of 0.2, and the TFr zero point and scatter did not change notably with a different value of q$_0$. With limited resolution of the optical images and unresolved \H\ data, this is the only approach to a reasonable inclination measurement. Several other literature studies with unresolved data also commonly use a similar approach \citep[e.g.,][]{Tully_Fisher77, Topal18}.

For the comparison samples, namely UMa and HIGHz, inclinations were used from the respective papers. For the UMa sample, inclination measurements are robust due to the availability of resolved \H\ data. The HIGHz sample suffers from limitations in resolution similar to \b, and their inclinations were also derived from exponential fits to the SDSS r-band images.


\subsubsection{Choice of velocity measures}\label{velmeasure}

Conventional \H\ based TFr studies make use of several velocity definitions, depending on the type of data available. For global profiles, various width definitions have been employed while spatially resolved rotation curves allow measurements of the outer flat part, the inner peak velocity or the velocity at a radius of 2.2 scale lengths of the stellar disc. The choice of velocity measure can have significant effects on the statistical properties of the TFr. 

\begin{figure*}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/27_gp.pdf}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/48_gp.pdf}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/78_gp.pdf}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/101_gp.pdf}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/45_gp.pdf}
\includegraphics[trim={20 10 40 20},clip, width=0.31\linewidth]{chapter3/img_update/117_gp.pdf}

\caption{Some examples of asymmetric \H\ profiles that show the presence low-level \H\ which is responsible for broadening the observed $\mathrm{W_{20}}$ line widths. The velocity resolution of these profiles is 38 \kms.}
\label{fig:asym_ex}
\end{figure*}

For single dish and spatially unresolved \H\ studies, the classic approach for estimating 'the' rotational velocities of galaxies is based on the corrected widths of the global \H\ profiles \citep{Tully_Fisher77} at the 20\% and 50\% of the peak flux density (\wct\ and \wcf\ respectively), where inferred rotational velocities are roughly half of the corrected \H\ profile line widths. \citet{Lelli19} found significantly tighter TFrs using \H\ line-widths as proxies for rotational velocities, as compared to other velocity tracers such as the H$\alpha$ and CO emission lines, which probe velocities in the inner parts of galaxies. This implies that \H\ line widths, while indirect velocity measures, are better kinematic tracers of the dark matter potential than other tracers originating from the inner star-forming discs of galaxies. Rotational velocities measured along the flat part of \H\ rotation curves are found to provide the tightest TFrs \citep{Verheijen01,Ponomareva17,Lelli19}. However, such measurements require spatially resolved \H\ kinematics from interferometric observations, which are often not available. Additionally, \citet{Glowacki20} found, for their sample of galaxies from the SIMBA simulation, that $\mathrm{W_{20}}$ line widths were the best proxies for V$_{\mathrm{flat}}$, whereas $\mathrm{W_{50}}$ suggested smaller rotational velocities by definition. However, when considering only disc galaxies, both velocity measures traced V$_{\mathrm{flat}}$ quite well, except for dispersion-dominated low mass galaxies, which lay off the 1:1 relation between 2V$_{\mathrm{flat}}$ and $\mathrm{W_{50}}$. This also highlights the importance of proper sample selection.

Since the \b\ sample consists mostly of spatially unresolved \H\ sources, the corrected \H\ profile line widths \wct\ and \wcf\ were used as proxies for the rotational velocities. Interestingly, we found a striking difference in \wct\ and \wcf\ without any correlation with the average SNR of the \H\ profiles (see Fig. \ref{fig:fracdiff1}). We concluded that galaxies in our sample have intrinsically shallower \H\ profile wings compared to the Local Universe counterparts. Furthermore, the \H\ profiles of the \b\ galaxies also tend to be more asymmetric than the UMa galaxies.

Our sample selection procedure resulting in the \textit{HQS} (described in detail in Sect. \ref{sampsel}) involved further stringent quantitative constraints on the \H\ profile to ensure a more reliable estimate of the rotational velocity. The first criterion ensured a higher SNR in the \H\ profiles. The second imposed constraints on the symmetry in the profiles, while the third criterion assessed the steepness of the profile edges. Figure \ref{fig:steep} shows histograms of the steepness and symmetry of these profiles. From these histograms, it is clear that the galaxies in the \textit{HQS} still have more asymmetric profiles with shallow edges compared to the UMa galaxies. However, we find that these more stringent quantitative criteria do not significantly reduce the TFr scatter or zero point offset of the \textit{HQS} compared to the \textit{TFS}. % The first involved an automated profile classifier that only retained double-horned and boxy HI profiles.

The differences observed in the \wct\ and \wcf\ line widths pose the question about the correct choice of velocity measure, since they both result in two different TFrs (illustrated in Fig. \ref{fig:tfr}). Further analysis of galaxies with asymmetric \H\ profile shapes in the two \b\ samples suggests the presence of low-level unresolved \H\ which is likely not participating in the rotation of these galaxies but appears to broaden the \H\ profiles at low flux levels, thus affecting the \wct\ line widths. The \wcf\ line widths on the other hand, seem less affected by this broadening. Some of these asymmetric profiles are shown in Fig. \ref{fig:asym_ex}. Thus, smaller offsets with UMa seen in the \wct\ TFrs (Fig. \ref{fig:tfr}, top) are likely due to an overestimation of the \wct\ line widths, causing the \b\ sample to shift towards larger rotational velocities and hence closer to UMa. Plotting the vertical offsets of all individual galaxies from the UMa TFrs as a function of increasing asymmetry (|$\Delta$ V$_{sys}$|/\wot) and increasing shallowness ($\Delta$W$=$\wct-\wcf) in Fig. \ref{fig:offset_col}, we do not see any particular trend.



To explore a possible correlation between the environment and the occurrence of asymmetric and shallow \H\ profiles, the \b\ samples were categorised further into two sub-samples, the \textit{Cluster} and \textit{Control} samples (see Sect. \ref{bo}). Histograms similar to Fig. \ref{fig:steep} are shown for these sub-samples in Fig. \ref{fig:steep_bo}. Most of these asymmetric and shallow \H\ profiles originate from the \textit{Cluster} sample, though the \textit{Control} sample also exhibits some asymmetric and shallow profiles. \citet{Jaffe11b} also found similar disturbances in their optical emission-line profiles of cluster galaxies. Probing the nature of these differences in the context of evolutionary signatures as seen by studies such as \citet{Kannappan02, Kassin07} amongst others, would require further analysis of the \H\ profiles and a larger sample, which is beyond the scope of this chapter.  


%\begin{figure*}
%    \centering
%    \includegraphics[trim={3cm 0.5cm 3cm 0.2cm },clip,width=\linewidth]{A963_globpr_ex.pdf}
%    \includegraphics[trim={3cm 0cm 3cm 0.2cm },clip,width=\linewidth]{A2192_globpr_ex.pdf}
%    \caption{Some examples of the observed global HI profiles of galaxies in the BUDHIES sample. Top: A963, bottom: A2192. The numbers printed to the top-right indicate the catalogue number from Paper 1, also provided in Table \ref{tab:A963_HI_table}. Provided below these index numbers are the fractional differences between the W$\mathrm{_{20}}$ and W$\mathrm{_{50}}$ line widths. A fractional difference close to zero indicates that the profiles have steep wings, as expected for normal late-type galaxies }
%    \label{fig:globprof}
%\end{figure*}


%Figure 10 presents the TF relationship based on the MB magnitude for 32 intermediate redshift galaxies. As in Sect. 4.1, most of the dispersion is related to interlopers, i.e. to galaxies with velocity fields different to those of rotating discs. For the eleven rotating discs however we notice that the scatter is larger than what is found for local galaxies. We have verified whether this can be due to the uncertainty on the correction related to the inclination (which is much larger at B wavelength than that at K band), which could especially affect galaxies that have not been imaged by the HST. It seems that it is not the case because the three galaxies lying at 3σ above the local TF have HST images available (HDFS4020, 4180 and 5190). There are 3 to 5 spirals that show a higher B luminosity than that expected from the local TF, while none show the reverse effect (lower B luminosity than expected). It might be understood if we were directly viewing a highly active star formation event (such as a giant HII region) in some distant spirals.


\noindent\subsubsection{Choice of stellar mass estimator}

Similar to Sect. \ref{corrdisc}, we here discuss the systematics involved in the choice of stellar mass prescription used to estimate baryonic masses. For this purpose, two different stellar mass prescriptions, Eqs. \ref{eq:mstar1} and \ref{eq:mstar2} respectively, were used to derive stellar and baryonic masses. Shown in Fig. \ref{fig:mbarcomp} are the ratios of the two baryonic masses derived using Eq. \ref{eq:mstar1} and \ref{eq:mstar2} for both, \b\ and UMa. We find that the baryonic masses derived from both stellar mass prescriptions are consistent, with insignificant offsets from the line of equality of 1.008 and 1.003 for the \b\ \textit{TFS} and UMa samples respectively. The resulting BTFrs from the two stellar mass estimators are shown in Fig. \ref{fig:btfr} and their fit parameters are given in Table \ref{tab:fitparams}. They are both consistent with the Local BTFr within the errors (see Sect. \ref{disc_stel_bar}), indicating that our choice of stellar mass prescription does not seem to impact the BTFr.


\subsection{Evolution in the TFr with redshift}\label{redshiftevol}

There are no \H\ studies of similarly constructed TFrs at higher redshifts in the literature to compare our results to. Other works at higher redshifts make use of other kinematic tracers and are based on optical or CO measurements, which originate from the inner regions of galaxies. There are currently many conflicting results and ongoing debates regarding the evolution of the TFr parameters with redshift. The first investigations using long slit spectroscopy of high-z galaxies showed varied results \citep{Vogt97, Rix97, Simard98}, as did subsequent studies using long-slit or integral field unit (IFU) observations \citep[e.g.,][]{Ferreras01,Ziegler02,Bohm04,Ferreras04,Conselice05,Flores06,Bamford06,Weiner06, Kassin07,Puech08,DiTeodoro16,Tiley16}. More recent studies such as \citet{DiTeodoro16} who analysed H$\alpha$ velocity fields from IFU spectroscopy to derive the stellar mass TFr, reported no significant evolution out to z $\sim$ 1. \citet{Topal18} presented the first CO-based TFrs beyond the Local Universe (0.05 < z < 0.3) and also found no significant evolution of the zero-point as a function of redshift when compared with the local TFr \citep{Tiley16}.


\begin{figure*}

\includegraphics[trim={0cm 0cm 0cm 0cm },clip,width=\linewidth]{chapter3/img_update/steepness_bo.pdf} 
\includegraphics[trim={0cm 0cm 0cm 0cm },clip,width=\linewidth]{chapter3/img_update/asymmetry_bo.pdf} 
    
\caption{ Similar to Fig. \ref{fig:steep} but for the control (pink) and cluster (black) samples, respectively: Top: histograms showcasing the difference in the observed line widths (shallowness); Bottom: histograms showing the absolute fractional differences in the systemic velocities derived from the two line width measures (asymmetry). The orange histograms show the UMa sample. Open histograms correspond to the \textit{TFS}, while the hatched histograms show the \textit{HQS}. }
\label{fig:steep_bo}
\end{figure*}

Conflicting results in the literature are likely caused by differences in the construction of the comparison samples and inconsistencies in the applied corrections, which, as discussed previously, could introduce systematic offsets which may be mistaken for evolutionary signatures. In our analysis, we have chosen to compare our \b\ TFrs with the local UMa TFr from \citet{Verheijen01} instead of other literature samples because of the similarities in the available data: WSRT interferometry and B- and R-band photometry with corrections applied consistently and identically to both the \b\ and the UMa observables. Since the range in \H\ line widths is relatively small, our analysis is limited to investigating the offsets in the zero points while fixing the slope to the z=0 TFr from UMa. The fit results for the two \b\ sub-samples and the offsets with respect to each other as well as with UMa are listed in Table \ref{tab:fitparams}, in which offsets greater than 5$\sigma$ are highlighted. Since the differences between the \textit{TFS} and \textit{HQS} are minor, we will limit the remainder of this discussion to the larger \textit{TFS} only.

\subsubsection{Evolution in the luminosity-based TFr}

In Sect. \ref{velmeasure} we discussed in detail the differences observed in the \wct\ and \wcf\ line widths, and the possible reasons for the  asymmetries and the shallow edges seen in the \H\ profiles of the \b\ galaxies. The M$_{\rm R}$-\wct\ TFr shows an insignificant offset of 0.19 $\pm$ 0.06 magnitudes from UMa, whereas in the B-band, the offset is notably larger (0.47 $\pm$ 0.06). The \wcf\ based TFr on the other hand, shows larger offsets in both B (0.72 $\pm$ 0.06) and R (0.44 $\pm$ 0.06) bands.  Given that the \wct\ might tend to overestimate rotational velocities, the \b\ galaxies likely shift towards larger inferred rotational velocities, thus bringing them closer to the z=0 TFr. This can explain the differences observed in the TFrs from the two velocity measures (Fig. \ref{fig:tfr}). The offsets in the zero points from the \wcf\ TFrs however, imply that galaxies in the past were both brighter ($\Delta$ZP$_\mathrm{R}$ = 0.44 mags) and bluer ($\Delta$ZP$_{(\mathrm{B-R})}$ = 0.28 mags) than galaxies in the present epoch. One of the reasons for pronounced offsets in the B-band is the greater sensitivity to star-formation activity in galaxies (discussed in Sect. \ref{coldisc}). This is also found in the literature, for example, by \citet{Bohm16} who found a brightening in their B-band TFr of field galaxies at higher redshifts. 

\begin{figure}
\includegraphics[trim={20 10 40 20},clip, width=0.9\linewidth]{chapter3/img_update/diff_uma_zib.pdf}
\caption{Ratio of the baryonic masses derived from the two stellar mass prescriptions, Eq. \ref{eq:mstar1} (referred to as $\mathrm{M_{bar}^{mxd}}$) and Eq. \ref{eq:mstar2} (referred to as $\mathrm{M_{bar}^{zib}}$) as a function of $\mathrm{M_{bar}^{mxd}}$. The purple circles are the \b\ \textit{TFS} galaxies while the orange circles indicate the UMa galaxies. The solid purple and orange lines and the corresponding coloured numbers printed to the bottom-right indicate the mean ratios of the baryonic masses for the TFS and UMa samples, respectively. The dashed grey line indicates the line of equality.}
\label{fig:mbarcomp}
\end{figure}


%2011). Discussed in Sect. \ref{envir} is the effect of the environment on these differences in the zero points.

%sample, the R-band TFr using \wct as the kinematic tracer shows a slight brightening of 0.14 magnitudes ($\sim$2.3$\sigma$) from the UMa TFr. In the B-band, the offset in zero point is more pronounced ($\sim$7.6$\sigma$). In the \wcf TFr, however, the offsets are much more significant, with 0.76 ($\sim$12.6$\sigma$) and 0.45 magnitudes ($\sim$7.5$\sigma$) in the B and R-bands respectively. 

%Now considering the "main" sample only, we find more compelling offsets (5$\sigma$ or more), with $\sim$6$\sigma$ in the \wct-R TFr and $\sim$5$\sigma$ in the \wcf-R TFr. The B-band offsets are greater than  $\sim$9$\sigma$. Our speculations for this pronounced offset and larger scatter in the B-band are discussed in Sect. 7.1.2. No significant offsets are found between the two BUDHIES subsamples (all offsets < 4$\sigma$.)


\subsubsection{Evolution in the Baryonic TFr}\label{disc_stel_bar}

As shown in Fig. \ref{fig:mratios}, the higher \mhi/\mstel\ and \mhi/\mbar\ ratios of the \b\ galaxies compared to UMa. (see Sect. \ref{compprop}) implies that a larger fraction of the baryonic content in the \b\ galaxies is in the form of \H. The figure also shows a larger intrinsic spread in properties for the UMa sample, which is not reflected in a larger scatter in the TFr or BTFr.  In particular, the two UMa galaxies (NGC 3729 and NGC 4102) with the lowest \mhi/\mstel\ and \mhi/\mbar\ ratios in Fig. \ref{fig:mratios} (b) and (d) have the lowest \H\ masses and small \H\ discs, yet they follow the TFr and BTFr. Despite the spread in properties, none of the UMa galaxies are outliers in the z=0 TFr or the BTFr (Figs. \ref{fig:tfr} and \ref{fig:btfr}). This implies, firstly, that for the TFr and its mass range under consideration here, the \H\ is significant only as a robust tracer of the rotational velocities of the Dark Matter halos of galaxies. Secondly, in the velocity range probed in this study, the BTFr is neither affected by the radial distribution of the baryons in galaxies as found by \citet{Zwaan95,Verheijen01}, nor by the proportion of the \H\ or stellar components that make up the baryonic content.

Turning our attention to the \b\ BTFrs, we find that their zero points are comparable to the z=0 BTFrs, using either stellar mass estimators (Eqs. \ref{eq:mstar1} and \ref{eq:mstar2}). For the 2V$_{50}$ BTFrs constructed with the \textit{TFS}, the offsets in the zero points are as small as +0.08 $\pm$ 0.02 dex and -0.02 $\pm$ 0.03 dex, based on Eqs. \ref{eq:mstar1} and \ref{eq:mstar2} respectively. We therefore conclude that there is no evolution in the zero point of the BTFr with redshift up to z $\sim$ 0.2. This supports the finding by \citet{Dutton11}, who find that the scaling relations using baryonic masses show a weak evolution. Shown in the last panel of Fig. \ref{fig:offset_col} are the vertical offsets of the UMa and \b\ galaxies from the luminosity-based UMa TFrs as a function of the \mhi/\mbar\ ratio. No particular trend is seen for either sample.


%In both cases, it is clear that the stellar masses are underestimated from the prescriptions used. This is also visually evident from the HIGHz sample. Note the downward turn of galaxies with higher rotational velocities. From these results, it is evident that the choice of IMF plays a key role in the extent of offset observed, but by how much, and whether these offsets can be also attributed to one of the intrinsic properties of the BUDHIES galaxies is a speculation that is beyond the scope of this paper. However, we must exercise caution regarding the origin of such systematic effects,like the offsets based on Eq. \ref{eq:mstar2} which could very easily be mistaken for evolutionary trends instead.

%Looking at the conversion to baryonic masses based on Eq. \ref{eq:mbar}, we find a spectacular recovery of the BTFrs, almost identical to the Local BTFr, using both stellar mass prescriptions. From the BTFrs of the BUDHIES sample using both \wcf and \wct as the kinematic measures, we find no evolution of the BTFr at z$\sim$ 0.2 with a maximum offset of -0.11 magnitudes. Note the presence of a "bump" at lower rotational velocities, which seems to suggest that a handful of galaxies lie off the BTFr and are more massive for their rotational velocities. We identified these outliers, and none of them belong to the \textit{main} sample. These are galaxies 11, 31, 48, 54, 60, 98 and 110 in A963 and 21 and 39 in A2192. These numbers are based on Col (2) of Table \ref{tab:A963_HI_table}. \textcolor{cyan}{I will look at their properties in detail and then comment. Offhand analysis shows no particularly striking properties that are common in these galaxies.}%UDGs? (need to check which galaxies these are).


\subsection{Effect of cosmic environment on the TFr}\label{envir}

There are several literature studies linking scaling relations such as the TFr to the evolution of galaxies in different environments. In dense cluster environments, for instance, kinematically anomalous galaxies are expected to be more common than in the field due to mechanisms such as ram-pressure stripping, tidal interactions, mergers, harassment and strangulation \citep[e.g.,][]{Oosterloo05, Poggianti17, Jaffe18, Toomre72, White78, Smith10, Kawata08, Maier16}. Inclusion of such galaxies in a TFr analysis are expected to lead to a larger scatter and systematic offsets in the TFr parameters, as discussed in Sect. \ref{sampseldiscussion}. 

There are some environment- and morphology-specific studies of the TFr, both at low \citep[e.g.,][]{Vogt04,Mocz12} and high redshifts. At higher redshifts, several environment-based TFr studies reported no significant differences in the TFrs in cluster and field populations \citep{Ziegler03,Nakamura06,Jaffe11b,Perez21}, while other authors such as \citet{bamford05}, \citet{Milvang-Jensen03} and \citet[][for z$\sim$ 1.5]{Perez21} found an overall brightening of cluster galaxies at a fixed rotational velocity. Other morphology-specific studies such as \citet{Bedregal06,Yara14} reported fainter magnitudes at a given rotational velocity for lenticular and early-type galaxies compared to spiral galaxies.

Our thorough selection criteria were aimed at ensuring the selection of isolated, inclined systems with symmetric \H\ profiles with steep edges. However, it is still possible that the local environment around these galaxies may contribute to the scatter or offsets observed in Figs. \ref{fig:tfr} and \ref{fig:btfr}, since a significant fraction of the \b\ galaxies lie in the vicinity of the massive, lensing cluster Abell 963. It is of particular interest to investigate the offset and scatter in the TFr in the context of the so-called "Butcher-Oemler" (BO) effect \citep{BO84}. The core of Abell 963 contains an unusually large fraction (19\%) of blue galaxies although none of which were detected in \H\ within a projected distance of 1 Mpc from the cluster centre. This implies that these blue galaxies may not be gas-rich and actively star-forming systems but still have their light dominated by a young, post-starburst stellar population. In a series of papers, the substructure and nature of these blue galaxies were studied based on \H\ stacking in phase space \citep{Verheijen07, Yara1_13,Yara2_15, Yara3_16}, with the conclusion that the blue galaxies were stripped of their \H\ during their first passage through the Intra-Cluster Medium (ICM) which resulted in temporarily enhanced star formation, and that these blue galaxies could possibly have remaining \H\ with masses below our detection threshold. Other blue galaxies in the vicinity of the cluster could still be gas bearing and experiencing enhanced star formation activity.

To probe the effect of the environment on the TFr and BTFr parameters, the \textit{TFS} and \textit{HQS} were further classified into two categories: the \textit{"Control"} and the \textit{"Cluster"} sub-samples (see Sect. \ref{bo} for the sample construction). We have discussed the correlation between asymmetric and shallow \H\ profiles, and environment in Sect. \ref{velmeasure}. Here, we discuss the TFrs shown in Fig. \ref{fig:bo}. The fit results are tabulated in Table \ref{tab:fitparamsbo}. In the figure, the top four panels show the luminosity-based TFrs using the \wct\ and \wcf\ respectively (similar to Fig. \ref{fig:tfr}), for the \textit{Cluster} and \textit{Control} samples. Based on the \wcf\ velocity measures, it is observed that the \textit{Cluster} sample is significantly brighter (0.65 mags) and bluer (0.27 mags) than the Local TFr. Exclusion of the \textit{Cluster} galaxies from the TF sample (which we call the \textit{Control} sample) does impact the \textit{Control} TFr and the offset in zero point with UMa is smaller (0.31 $\pm$ 0.08 and 0.63 $\pm$ 0.07 in the B and R bands respectively) than the \textit{TFS}. However, the brightening and blueing of the \b\ (\textit{Control}) galaxies is still not insignificant. This finding indicates that environment does seem to play a role in shaping the TFr, especially at higher redshifts, where the scatter is larger \citep[e.g.,][]{Moran07}.

Focusing instead on the environment-based BTFrs (Fig. \ref{fig:bo}, bottom 2 panels), we find that the  V$_{50}$-BTFr of the \textit{Control} sample is consistent with UMa. Additionally, the \textit{Cluster} BTFr, while offset from both the \textit{Control} as well UMa TFrs, is still consistent within the errors (maximum offset is 0.2 mags). This implies that though the offsets in the luminosity-based TFrs cannot be ignored, much of the luminosity arises from the B-band which is sensitive to new star formation and does not contribute significantly to the stellar masses (which largely depend on the B-R colour) of these galaxies. This new star formation could occur prior to or during the first pericentric passage through the ICM when the galaxies still contain a detectable amount of \H\ gas \citep[e.g.,][]{Mahajan12,Yara3_16,vulcani18c}. Thus, our results imply that galaxies in the past and irrespective of their environment, while bluer and brighter, do not show a difference in their relative baryonic content with respect to the z=0 sample.

%The use of galaxy kinematics to study the evolution of starforming galaxies in clusters has been traditionally linked to scaling relations such as the Tully-Fisher relation (TFR, Tully &Fisher 1977), that can only be applied to regular rotating discs. While some authors claimed no difference between the cluster and field TFRs (Ziegler et al. 2003, Nakamura et al. 2006), others reported that spiral galaxies were slightly overluminous (Bamford et al. 2005) and display a larger TFR scatter (Moran et al. 2007) in the cluster environment at z<1. However, galaxies with irregular kinematics cannot be excluded from a comprehensive environmental study since they represent the majority of the population in clusters (Rubin et al. 1999, Vogt et al. 2004). Following this idea, Bösch et al. (2013a) were able to link RPS events with asymmetries in the gas velocity profile of cluster galaxies that do not show significant distortions in their stellar structure

\subsection{Comparison with HIGHz}

Lastly, for a cursory comparison, we also overlaid the HIGHz sample in the \wcf\ TFrs and BTFrs plots. The HIGHz sample consists of optically selected massive, luminous and red galaxies at redshifts similar to \b\ (see Sect. \ref{compprop} for more details). \citet{Catinella15} found that they lie on the local BTFr from GASS, though the galaxies had not been corrected for turbulent motion, inclination or internal extinction. In our work, corrections applied to the \b\ galaxies were identically applied to the HIGHz sample. It should be noted, however, that the magnitudes of these galaxies were extracted from SDSS and converted to Johnson-B and Cousins-R magnitudes following \citet{Cook14}, which could have a small impact on their position in these plots.

Compared to our luminosity-based TFrs (Fig. \ref{fig:tfr}), we find that, while the HIGHz sample is roughly consistent with the Local TFr, a nearly flat distribution is visually obvious and a correlation between luminosity and line width is nearly absent. In the case of the BTFr (Fig.\ref{fig:btfr}), we find that the HIGHz galaxies have significantly larger baryonic masses for their rotational velocities compared to both the Local TFr and \b. Unfortunately, the limited range in luminosity as well as line widths does not allow for further analysis of this sample. 

\section{Summary and Conclusions}\label{summary}

With this work, we present the first dedicated attempt to construct an \H-based TFr beyond the Local Universe using direct \H\ detections. We have studied the luminosity-based B- and R-band TFrs as well as the baryonic TFr at z $\sim$ 0.2 from a meticulously selected sample of galaxies detected in \H\ from the Blind Ultra-Deep \H\ Environmental Survey (\b). Deep B-band and R-band data was obtained from the INT (for more details, see Paper 1). The \b\ TF sample (\textit{TFS}) comprises 36 galaxies, of which 29 are in the survey volume containing Abell 963 and 7 in the volume containing Abell 2192. Of these, 11 and 7 galaxies together make up the \textit{High Quality} sub-sample (\textit{HQS}) based on stringent quantitative thresholds imposed on the shape of the \H\ global profile. Our results were compared with an identically constructed TFr from the Ursa Major association of galaxies in the Local Universe at a distance of 18.6 Mpc \citep[UMa,][]{Verheijen01}. Our main results are as follows: \\

\noindent
(1) The best fit inverse R-band and baryonic TFrs for the \b\ TF sample with all parameters left free are:  \\  \\
M$_R$ = (-8.4 $\pm$ 0.54) log (\wcf)]+ (-0.33 $\pm$ 1.41); \\
log(\mbar/M$_\odot$) = (3.4 $\pm$ 0.20) log (2V$\mathrm{_{50}^{R,t,i}}$) + (1.98 $\pm$ 0.61); \\

\noindent
These are based on the \wcf\ velocity measures and stellar masses are computed using Eq \ref{eq:mstar1}. Fits using other velocity measures and stellar mass estimators are given in Sects. \ref{tfr} and \ref{btfr} Due to the limited range and larger errors in line widths of the \b\ galaxies compared to UMa, further analysis was restricted to the TFr zero points only by fixing the slope to the UMa TFr. \\

\noindent
(2) The scatter in the \textit{TFS} and \textit{HQS} TFrs are very similar, suggesting that stricter quantitative selection criteria on the shapes of the \H\ profiles do not reduce the scatter.\\

\noindent
(3) Similarly, differences in the zero points of the \textit{TFS} and \textit{HQS} TFrs are always less than 0.05 magnitudes, implying that stricter selection criteria also do not affect the TFr zero points. These thresholds were chosen to improve the quality of the sample without compromising too much on the sample size. However, the \b\ galaxies in the \textit{HQS} still seem to have more asymmetric \H\ profiles with shallower wings than the UMa galaxies. Further inspection of these asymmetric profiles suggests the presence of low-level unresolved \H\ gas, possibly from optically unidentified nearby companions, that likely does not participate in the rotation of the galaxies but broadens the \wct\ in some cases. This leads to the intrinsic differences observed in the two line width measures. The majority of these disturbed \H\ profiles are from galaxies belonging to the cluster Abell 963. \\

\noindent
(4) Adopting \wcf\ as the velocity measure, the \b\ TFr is both bluer and brighter than the z=0 TFr (based on offsets in the zero points alone). The cluster Abell 963 has some influence on these offsets, but exclusion of these cluster galaxies (lying within 2.5$\mathrm{\sigma_{cl}}$, called the "\textit{Cluster}" sample) from the TF sample (which is referred to as the "\textit{Control}" sample) still shows a smaller yet significant brightening of 0.31 magnitudes in the R-band and 0.63 magnitudes in the B-band. \\

\noindent
(5) The zero point offsets depend on the choice of photometric band and velocity measure. Offsets in the B-band are always larger than the R-band. Due to an overestimation of rotational velocities using \wct, the \b\ sample shifts towards larger rotational velocities and hence closer to the UMa TFr, thus greatly reducing the offsets in the zero points.\\

\noindent
(6) Galaxies belonging to the \textit{Cluster} sample are significantly brighter (0.65 mags) and bluer (0.27 mags) than the Local TFr, as well as the \textit{Control} sample ($\sim$0.3 mags).\\

\noindent
(7) The Baryonic TFr at z$\sim$0.2, is strikingly close to the Local BTFr. Two different stellar-mass prescriptions were used, and the resulting BTFrs are found to be consistent with the Local BTFr, within the uncertainties. The exclusion of cluster galaxies does not affect the results. \\

\noindent
(8) A cursory comparison of the optically selected HIGHz galaxies with the UMa and \b\ samples show that they are largely consistent with the luminosity-based \b\ and local TFr but have higher baryonic masses for their rotational velocities. \\

\noindent
(9) Lastly, it is very important to ensure that the comparison samples trace similar galaxy populations for a proper and unbiased comparison, since the various corrections, even if consistently applied, may affect different galaxy populations differently.\\

\noindent
We conclude from the \textit{Control} sample that field galaxies in the past were brighter and bluer, but contain a similar baryonic content to galaxies in the Local Universe. The galaxies in our high redshift sample are more gas-rich than galaxies in the Local Universe. Galaxies belonging to the BO cluster Abell 963 seem to be more luminous and bluer than other galaxies at similar redshifts, as well as local galaxies. Finally, with this study, we reinforce the fact that \H\ as a kinematical tracer of the rotational velocities of galaxies is an important tool to further our knowledge of the evolution of such scaling relations. We aim to provide an important yardstick for future \H-based surveys at higher redshifts with more sensitive survey instruments such as MeerKAT and the Square Kilometre Array. 



\section*{Acknowledgements}

AG and MV would like to acknowledge the Netherlands Foundation for Scientific Research support through VICI grant 016.130.338 and the Leids Kerkhoven-Bosscha Fonds (LKBF) for travel support. AG thanks P. Bilimogga for useful discussions, for providing the \H\ profile widths for the Perseus-Pisces data and the systemic velocities for the Ursa Major sample. AG also thanks N. Choque. and J. Healy for useful discussions on galaxy modelling with \textit{galfit}. JMvdH acknowledges support from the European Research Council under the European Union's Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement nr. 291531. Y.J. acknowledges financial support from CONICYT PAI (Concurso Nacional de Insercion en la Academia 2017) No. 79170132 and FONDECYT Iniciacion 2018 No. 11180558. The WSRT is operated by the Netherlands Foundation for Research in Astronomy, supported by the Netherlands Foundation for Scientific Research. The full acknowledgement of the Sloan Digital Sky Survey Archive used in this chapter can be found at http://www.sdss.org.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%% REFERENCES %%%%%%%%%%%%%%%%%%

% The best way to enter references is to use BibTeX:
\section*{Data availability}
The data underlying this article will be shared on reasonable request to the corresponding author.


%\bibliographystyle{mnras}
%\bibliography{references2} 











%\begin{figure*}
%\includegraphics[width=\linewidth]{M_star_color.pdf}
%\caption{M$_{*}$-colour diagram for the BUDHIES and UMa samples.}

%\end{figure*}







%\begin{figure*}
%\includegraphics[trim={0 30cm 0 30cm},clip,width=0.15\linewidth]{A963_globprofs.pdf}
%\includegraphics[trim={0 30cm 0 30cm},clip,width=0.15\linewidth]{A2192_globprofs.pdf}
%\includegraphics[trim={0 30cm 0 30cm},clip,width=0.15\linewidth]{UMa_globprofs.pdf}
%\includegraphics[trim={0 30cm 0 30cm},clip,width=0.15\linewidth]{pp_globprofs.pdf}
%\caption{Comparison of the global HI profiles of the various samples}

%\end{figure*}


%\begin{figure*}
%\includegraphics[width=\linewidth]{CMD_sdss_all.pdf}
%\caption{The colour-magnitude diagram of the BUDHIES and HIGHz samples using galactic extinction corrected sdss g and r magnitudes. The horizontal panels show the distribution after each individual step, such as transformation to Johnson B and Cousins R filters, K-corrections and internal extinction corrections.}

%\end{figure*}




%\begin{figure*}

%    \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.21\linewidth]{W20B_mhi_offsetcomp.pdf} 
 %   \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.21\linewidth]{W20R_mhi_offsetcomp.pdf}
%    \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.21\linewidth]{W50B_mhi_offsetcomp.pdf}
 %   \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.21\linewidth]{W50R_mhi_offsetcomp.pdf}
    
%    \caption{Caption}
%    \label{fig:offset_mhi}
%\end{figure*}


%\begin{figure*}

%    \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.41\linewidth]{W20R_mbar_offsetcomp.pdf} 
%    \includegraphics[trim={0.3cm 2.5cm 1.2cm 1cm },clip,width=0.41\linewidth]{W50R_mbar_offsetcomp.pdf}
    
%    \caption{Caption}
%    \label{fig:offset_mbar}
%\end{figure*}


\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}


\input{chapter3/TF_tables_new.tex}

\onecolumn


\onecolumn
%\begin{landscape}
%{\setlength{\tabcolsep}{5pt}

\newgeometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=1.4cm}
%\setcounter{table}{0}
%\renewcommand{\thetable}{A\arabic{table}}


\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\fontsize{8}{11}\selectfont
{\setlength{\tabcolsep}{3.5pt}
%\begin{landscape}
\LTcapwidth=\textwidth
%\begin{center}
    


\begin{longtable}{c | c  c  c  c  c | c  c}

\caption{\label{tab:fitparams} Parameters and offsets of the various TFrs.} \\

\hline \hline

& & & \textit{Parameters} & &  &\multicolumn{2}{c}{ZP Offsets} \\ \cline{2-8}
TFr & Count & a  & b  & $\chi^2_{\mathrm{red}}$ & $\sigma$ & Offset UMa & Offset \textit{TFS} \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8)\\

\hline
\endfirsthead
\caption{continued} \\
\hline \hline


& & & \textit{Parameters} & &  & \multicolumn{2}{c}{ZP Offsets} \\ \cline{2-8}
TFr & Count & a  & b  & $\chi^2_{\mathrm{red}}$ & $\sigma$ & Offset UMa & Offset \textit{TFS} \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8)\\

\hline 
\endhead
\hline
\endfoot
\textit{\textbf{$\mathrm{W_{20}}$-R}} & & & & & & & \\ \cline{1-1}  
UMa (free)  &  22  &  -8.29  $\pm$ 0.28  &  -0.2  $\pm$  0.69  & 3.88  &  0.34  & - & - \\ 
UMa  &  22  &  -8.29  (fixed)  &  -0.20  $\pm$  0.04  & 3.69  &  0.34   & - & -\\ 
TFS  &  36  &  -8.29  (fixed)  &  -0.39  $\pm$  0.05  & 6.35  &  0.68  & 0.19 $\pm$ 0.06 & -\\ 
HQS  &  19  &  -8.29  (fixed)  &  -0.38  $\pm$  0.05  & 10.0  &  0.70  & 0.18 $\pm$ 0.06 & 0.01 $\pm$ 0.07\\ 
&&&&&&& \\
\textit{\textbf{$\mathrm{W_{50}}$-R}} & & & & & & &  \\ \cline{1-1} 
UMa (free)  &  22  &  -8.68  $\pm$ 0.31  &  0.74  $\pm$  0.73  & 3.50  &  0.34  & - & - \\ 
UMa  &  22  &  -8.68  (fixed)  &  0.74  $\pm$  0.04  & 3.33  &  0.34   & - & -\\ 
TFS  &  36  &  -8.68  (fixed)  &  0.30  $\pm$  0.05  & 3.40  &  0.56  & \textbf{0.44} $\pm$ \textbf{0.06} & -\\
HQS  &  19  &  -8.68  (fixed)  &  0.35  $\pm$  0.06  & 5.20  &  0.57  & \textbf{0.39} $\pm$ \textbf{0.07} & 0.05 $\pm$ 0.08\\
&&&&&&& \\
\textit{\textbf{$\mathrm{W_{20}}$-B}} & & & & & & & \\ \cline{1-1}  
UMa (free)  &  22  &  -7.94  $\pm$ 0.28  &  -0.02  $\pm$  0.69  & 7.62  &  0.45  & - & - \\ 
UMa  &  22  &  -7.94  (fixed)  &  -0.02  $\pm$  0.04  & 7.26  &  0.45   & - & -\\ 
TFS  &  36  &  -7.94  (fixed)  &  -0.49  $\pm$  0.04  & 7.02  &  0.69  & \textbf{0.47} $\pm$ \textbf{0.06} & -\\ 
HQS  &  19  &  -7.94  (fixed)  &  -0.48  $\pm$  0.05  & 10.23  &  0.68  & \textbf{0.46} $\pm$ \textbf{0.06} & 0.01 $\pm$ 0.06\\ 
&&&&&&& \\
\textit{\textbf{$\mathrm{W_{50}}$-B}} & & & & & & & \\ \cline{1-1} 
UMa (free)  &  22  &  -8.25  $\pm$ 0.3  &  0.72  $\pm$  0.72  & 6.56  &  0.44  & - & - \\ 
UMa  &  22  &  -8.25  (fixed)  &  0.72  $\pm$  0.04  & 6.25  &  0.44   & - & -\\ 
TFS  &  36  &  -8.25  (fixed)  &  -0.0  $\pm$  0.05  & 3.73  &  0.56  & \textbf{0.72} $\pm$ \textbf{0.06} & -\\ 
HQS  &  19  &  -8.25  (fixed)  &  0.04  $\pm$  0.06  & 5.55  &  0.56  & \textbf{0.68} $\pm$ \textbf{0.07} & 0.04 $\pm$ 0.08\\
&&&&&&&\\
\textit{\textbf{BTFr V$_{20}$: 1}} & & & & & & &  \\ \cline{1-1} 
UMa (free)  &  22  &  3.02  $\pm$ 0.1  &  2.8  $\pm$  0.36  & 3.64  &  0.12  & - & - \\ 
UMa  &  22  &  3.02  (fixed)  &  2.80  $\pm$  0.01  & 3.46  &  0.12   & - & -\\ 
TFS  &  36  &  3.02  (fixed)  &  2.79  $\pm$  0.02  & 5.28  &  0.23  & 0.01 $\pm$ 0.02 & -\\ 
HQS  &  19  &  3.02  (fixed)  &  2.79  $\pm$  0.02  & 8.85  &  0.24  & 0.01 $\pm$ 0.02 & 0.0 $\pm$ 0.03\\
&&&&&&& \\
\textit{\textbf{BTFr V$_{50}$: 1}} & & & & & & &  \\ \cline{1-1} 
UMa (free)  &  22  &  3.2  $\pm$ 0.11  &  2.36  $\pm$  0.37  & 3.79  &  0.13  & - & - \\ 
UMa  &  22  &  3.20  (fixed)  &  2.36  $\pm$  0.01  & 3.61  &  0.13   & - & -\\ 
TFS  &  36  &  3.20  (fixed)  &  2.44  $\pm$  0.02  & 3.38  &  0.21  & 0.08 $\pm$ 0.02 & -\\ 
HQS  &  19  &  3.20  (fixed)  &  2.42  $\pm$  0.02  & 5.35  &  0.21  & 0.06 $\pm$ 0.02 & 0.02 $\pm$ 0.03\\
&&&&&&& \\
\textit{\textbf{BTFr V$_{20}$: 2}} & & & & & & &  \\ \cline{1-1} 
UMa (free)  &  22  &  3.2  $\pm$ 0.11  &  2.31  $\pm$  0.35  & 3.52  &  0.12  & - & - \\ 
UMa  &  22  &  3.20  (fixed)  &  2.31  $\pm$  0.01  & 3.36  &  0.12   & - & -\\ 
TFS  &  36  &  3.20  (fixed)  &  2.23  $\pm$  0.02  & 5.27  &  0.24  & 0.08 $\pm$ 0.02 & -\\ 
HQS  &  19  &  3.20  (fixed)  &  2.22  $\pm$  0.02  & 8.46  &  0.25  & 0.09 $\pm$ 0.02 & 0.01 $\pm$ 0.03\\
&&&&&&& \\
\textit{\textbf{BTFr V$_{50}$: 2}} & & & & & & &  \\ \cline{1-1} 
UMa (free)  &  22  &  3.43  $\pm$ 0.12  &  1.75  $\pm$  0.37  & 4.35  &  0.15  & - & - \\ 
UMa  &  22  &  3.43  (fixed)  &  1.75  $\pm$  0.02  & 4.14  &  0.15   & - & -\\ 
TFS  &  36  &  3.43  (fixed)  &  1.73  $\pm$  0.02  & 3.83  &  0.24  & 0.02 $\pm$ 0.03 & -\\ 
HQS  &  19  &  3.43  (fixed)  &  1.71  $\pm$  0.02  & 6.15  &  0.25  & 0.04 $\pm$ 0.03 & 0.02 $\pm$ 0.03

 
\end{longtable}
}
\normalsize
%\end{longtable}
%\end{landscape}






\pagebreak


\newgeometry{left=2.25cm, right=2cm, top=2.5cm, bottom=2cm}
%\setcounter{table}{0}
%\renewcommand{\thetable}{A\arabic{table}}


\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\fontsize{8}{11}\selectfont
{\setlength{\tabcolsep}{3.5pt}
%\begin{landscape}

\LTcapwidth=\textwidth
\begin{longtable}{c  | c  c  c  c  c | c  c}
 
\caption{\label{tab:fitparamsbo} Fit parameters of the environment-based TFrs}\\

%\begin{tabular}{c  | c  c  c  c  c | c  c}
%& & \textit{Parameters} & & & & & \textit{Offset comparisons}& & \\ \cline{2-4} \cline{6-10}
\hline \hline
& & & \textit{Parameters} & & & \multicolumn{2}{c}{ZP Offsets}\\ \cline{2-8}
TFr & Count & a  & b  & Chisq & Scatter & UMa & Cluster sample \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8)\\
\hline

\hline
\endfirsthead
\caption{continued} \\
\hline \hline

& & & \textit{Parameters} & & & \multicolumn{2}{c}{ZP Offsets}\\ \cline{2-8}
TFr & Count & a  & b  & Chisq & Scatter & UMa & Cluster sample \\
(1)  & (2)  & (3) & (4) & (5)  & (6) & (7) & (8)\\
\hline
\hline 
\endhead
\hline
\endfoot

\textit{$\mathrm{W_{20}}$ R} & & & & & &\\ \cline{1-1} 
UMa  &  22  &  -8.29  (fixed)  &  -0.2  $\pm$  0.04  & 3.69  &  0.34  &  -  &  -    \\ 
TFS Cluster   &  19  &  -8.29  (fixed)  &  -0.47  $\pm$  0.06  & 5.78  &  0.68  &  0.27 $\pm$ 0.08  &  -     \\ 
TFS Control   &  17  &  -8.29  (fixed)  &  -0.31  $\pm$  0.07  & 7.20  &  0.70  &  0.11 $\pm$ 0.08  &  0.16 $\pm$ 0.09    \\ 
HQS Cluster   &  7  &  -8.29  (fixed)  &  -0.44  $\pm$  0.08  & 11.43  &  0.61  &  0.24 $\pm$ 0.09  &  -    \\ 
HQS Control   &  12  &  -8.29  (fixed)  &  -0.33  $\pm$  0.07  & 10.03  &  0.72  &  0.13 $\pm$ 0.08  &  0.11 $\pm$ 0.1   \\ 
& & & & & & \\
\textit{$\mathrm{W_{20}}$ B} & & & & & &\\ \cline{1-1} 
UMa  &  22  &  -7.94  (fixed)  &  -0.02  $\pm$  0.04  & 7.26  &  0.45  &  -  &  -    \\ 
TFS Cluster   &  19  &  -7.94  (fixed)  &  -0.56  $\pm$  0.06  & 6.58  &  0.68  &  \textbf{0.54} $\pm$ \textbf{0.07}  &  -     \\ 
TFS Control   &  17  &  -7.94  (fixed)  &  -0.42  $\pm$  0.06  & 7.80  &  0.70  &  \textbf{0.40} $\pm$ \textbf{0.07}  &  0.14 $\pm$ 0.09    \\ 
HQS Cluster   &  7  &  -7.94  (fixed)  &  -0.49  $\pm$  0.07  & 11.28  &  0.61  &  \textbf{0.47} $\pm$ \textbf{0.08}  &  -    \\ 
HQS Control   &  12  &  -7.94  (fixed)  &  -0.47  $\pm$  0.07  & 10.72  &  0.72  &  \textbf{0.45} $\pm$ \textbf{0.08}  &  0.02 $\pm$ 0.1   \\
& & & & & & \\
\textit{$\mathrm{W_{50}}$ R } & & & & & &\\ \cline{1-1} 
UMa  &  22  &  -8.68  (fixed)  &  0.74  $\pm$  0.04  & 3.33  &  0.34  &  -  &  -    \\ 
TFS Cluster &  19  &  -8.68  (fixed)  &  0.09  $\pm$  0.08  & 1.58  &  0.44  &  \textbf{0.65} $\pm$ \textbf{0.09}  &  -     \\ 
TFS Control &  17  &  -8.68  (fixed)  &  0.43  $\pm$  0.07  & 5.03  &  0.60  &  0.31 $\pm$ 0.08  &  0.34 $\pm$ 0.11    \\ 
HQS Cluster &  7  &  -8.68  (fixed)  &  0.18  $\pm$  0.11  & 2.21  &  0.39  &  0.56 $\pm$ 0.12  &  -    \\ 
HQS Control &  12  &  -8.68  (fixed)  &  0.41  $\pm$  0.07  & 7.02  &  0.61  &  0.33 $\pm$ 0.08  &  0.23 $\pm$ 0.13   \\ 
& & & & & & \\
\textit{$\mathrm{W_{50}}$ B } & & & & & &\\ \cline{1-1} 
UMa  &  22  &  -8.25  (fixed)  &  0.72  $\pm$  0.04  & 6.25  &  0.44  &  -  &  -    \\ 
TFS Cluster &  19  &  -8.25  (fixed)  &  -0.18  $\pm$  0.08  & 2.14  &  0.44  &  \textbf{0.90} $\pm$ \textbf{0.09}  &  -     \\ 
TFS Control &  17  &  -8.25  (fixed)  &  0.11  $\pm$  0.06  & 6.29  &  0.60  &  \textbf{0.61} $\pm$ \textbf{0.07}  &  0.29 $\pm$ 0.10    \\ 
HQS Cluster &  7  &  -8.25  (fixed)  &  -0.08  $\pm$  0.10  & 3.73  &  0.39  &  \textbf{0.80} $\pm$ \textbf{0.11}  &  -    \\ 
HQS Control &  12  &  -8.25  (fixed)  &  0.08  $\pm$  0.07  & 8.30  &  0.61  &  \textbf{0.64} $\pm$ \textbf{0.08}  &  0.16 $\pm$ 0.12   \\ 
& & & & & & \\
\textit{2V$_{20}$ BTFr} & & & & & &\\ \cline{1-1} 
UMa  &  22  &  3.02  (fixed)  &  2.8  $\pm$  0.01  & 3.46  &  0.12  &  -  &  -    \\ 
TFS Cluster &  19  &  3.02  (fixed)  &  2.83  $\pm$  0.07  & 5.03  &  0.22  &  0.03 $\pm$ 0.07  &  -     \\ 
TFS Control &  17  &  3.02  (fixed)  &  2.75  $\pm$  0.07  & 5.55  &  0.22  &  0.05 $\pm$ 0.07  &  0.08 $\pm$ 0.09    \\ 
HQS Cluster &  7  &  3.02  (fixed)  &  2.85  $\pm$  0.08  & 11.60  &  0.22  &  0.05 $\pm$ 0.08  &  -    \\ 
HQS Control &  12  &  3.02  (fixed)  &  2.75  $\pm$  0.07  & 7.51  &  0.23  &  0.05 $\pm$ 0.07  &  0.10 $\pm$ 0.11   \\ 
&&&&&& \\
\textit{2V$_{50}$ BTFr} & & & & & &\\ \cline{1-1} 
UMa  &  22  &  3.20  (fixed)  &  2.36  $\pm$  0.01  & 3.61  &  0.13  &  -  &  -    \\ 
TFS Cluster &  19  &  3.20  (fixed)  &  2.56  $\pm$  0.08  & 1.41  &  0.15  &  0.20 $\pm$ 0.08  &  -     \\ 
TFS Control &  17  &  3.20  (fixed)  &  2.36  $\pm$  0.06  & 4.20  &  0.20  &  0.00 $\pm$ 0.06  &  0.2 $\pm$ 0.10    \\ 
HQS Cluster &  7  &  3.20  (fixed)  &  2.57  $\pm$  0.10  & 1.98  &  0.15  &  0.21 $\pm$ 0.11  &  -    \\ 
HQS Control &  12  &  3.20  (fixed)  &  2.36  $\pm$  0.06  & 5.83  &  0.21  &  0.00 $\pm$ 0.06  &  0.22 $\pm$ 0.12   \\ 

\end{longtable}
}
%\end{landscape}
% Don't change these lines
%\bsp	% typesetting comment
\label{lastpage}

\newpage
%\textit{W20 R} & & & & & \\ \cline{1-1} 
%UMa  &  22  &  -8.15  $\pm$ 0.0  &  -0.49  $\pm$  0.04  & 4.31  &  0.37  &  -  &  -     \\ 
%BO sample  &  9  &  -8.15  (fixed)  &  -0.89  $\pm$  0.07  & 8.74  &  0.6  &  \textbf{0.4} $\pm$ \textbf{0.08}  &  $-$     \\ 
%Control sample  &  14  &  -8.15  (fixed)  &  -0.61  $\pm$  0.06  & 8.64  &  0.71  &  0.12 $\pm$ 0.08  &  0.28 $\pm$ 0.09     \\ 
%\textit{W20 B} & & & & & \\ \cline{1-1} 
%UMa  &  22  &  -7.79  $\pm$ 0.0  &  -0.34  $\pm$  0.04  & 8.04  &  0.48  &  -  &  -      \\ 
%BO sample  &  9  &  -7.79  (fixed)  &  -1.0  $\pm$  0.06  & 9.1  &  0.59  &  \textbf{0.66} $\pm$ \textbf{0.08}  &  -      \\ 
%Control sample  &  14  &  -7.79  (fixed)  &  -0.78  $\pm$  0.06  & 9.33  &  0.71  &  \textbf{0.44} $\pm$ \textbf{0.07}  &  0.22 $\pm$ 0.09    \\  \hline

%\caption{}
%\end{tabular}







    %\captionof{figure}{Images \number\numexpr 6 * \x + 1\relax\space to
      %\number\numexpr 6 * \x + 6\relax.}
  
%4.0, 13.0, 21.0, 24.0


%\begin{figure*}
 %   \centering
 %   \includegraphics[trim={4.5cm 1cm 3.5cm 1cm},clip,width=1.2\textwidth]{galfit_2_atlas.pdf}
%    \includegraphics[angle =270,trim={6cm 2.5cm 10cm 3.5cm},clip,width=1.2\textwidth]{HIatlas2.pdf}
 %   \caption{Test atlas}
%    \label{fig:testatlas}
%\end{figure*}


%\end{landscape}
%%%%%%%%%%%%%%%%% APPENDICES %%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newgeometry{left=2cm, right=2cm, top=2.5cm, bottom=2cm}
%\setcounter{table}{0}
%\renewcommand{\thetable}{A\arabic{table}}


\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\fontsize{8}{11}\selectfont
{\setlength{\tabcolsep}{3.5pt}
\begin{landscape}
\LTcapwidth=\textwidth


\begin{longtable}{l |  c  c | c  c | c }

    
 \captionsetup{width=16cm}
\caption{\label{tab:assessment} Detailed break-down of the galaxies rejected at each step of the sample selection process}\\

\hline \hline
& \multicolumn{2}{c|}{A963}  & \multicolumn{2}{c|}{A2192} & \\
%\multicolumn{2}{c}{}  \\
%\cline{2-9}
\multicolumn{1}{c|}{Criteria} & Rejected cat no.  & \multicolumn{1}{c|}{Final sample size} & Rejected cat no. & \multicolumn{1}{c|}{Final sample size} & \multicolumn{1}{c}{Final sample size}  \\
\multicolumn{1}{c|}{(1)}   & (2) & \multicolumn{1}{c|}{(3)}  & (4) & \multicolumn{1}{c|}{(5)} & (6)  \\
\hline

\endfirsthead
\caption{continued} \\
\hline \hline

& \multicolumn{2}{c|}{A963}  & \multicolumn{2}{c|}{A2192} & \\
%\multicolumn{2}{c}{}  \\
%\cline{2-9}
\multicolumn{1}{c|}{Criteria} & Rejected cat no.  & \multicolumn{1}{c|}{Final sample size} & Rejected cat no. & \multicolumn{1}{c|}{Final sample size} & \multicolumn{1}{c}{Final sample size}  \\
\multicolumn{1}{c|}{(1)}   & (2) & \multicolumn{1}{c|}{(3)}  & (4) & \multicolumn{1}{c|}{(5)} & (6)  \\
\hline

 
\endhead
\hline
\endfoot


%\hline \hline
%& \multicolumn{2}{c|}{A963}  & \multicolumn{2}{c|}{A2192} & \\
%\multicolumn{2}{c}{}  \\
%\cline{2-9}
%\multicolumn{1}{c|}{Criteria} & Rejected cat no.  & \multicolumn{1}{c|}{Final sample size} & Rejected cat no. & \multicolumn{1}{c|}{Final sample size} & \multicolumn{1}{c}{Final sample size}  \\
%\multicolumn{1}{c|}{(1)}   & (2) & \multicolumn{1}{c|}{(3)}  & (4) & \multicolumn{1}{c|}{(5)} & (6)  \\
%\hline



\multicolumn{1}{c|}{\textbf{Parent Sample}} & \textbf{127} & \multicolumn{1}{c|}{-} & \textbf{39} & - &  \\\hline



\multicolumn{1}{c|}{\textbf{\textit{Observational criteria}}}  & & & & &  \\ 

Galaxies cut off at band edges   & 28, 38 & 125   & 20, 22 & 37 & 162  \\
& & & & & \\
Galaxies without INT photometry  & 12, 16, 125, 126, 127   & 120  & 7, 37 & 35  & 155  \\ 

& & & & & \\
Galaxies with unreliable INT   & 41, 44, 83  & 117  & 5, 16, 34 & 32  & 149  \\
photometry due to nearby & & & & &  \\
stars or other galaxies & & & & &  \\  
& & & & & \\


\multicolumn{1}{c|}{\textbf{\textit{Qualitative criteria}}}  & & & & &  \\

Nearby optical companions (UV   & 4, 8, 15, 19, 23, 24, 25, 26, 29, 32, & 99  & 2, 27, 33, 35 & 28  & 127 \\
bright) might lead to \H\ profile  &    35, 52, 64, 73, 80, 97, 107, 120 &  & & & \\

 disturbances, kinematical   &      & & & & \\
disturbances in main galaxy &   &   & & &  \\ 

& & & & & \\

Obvious disturbance in optical    & 34, 47, 59, 60, 66, 69, 77, 84, & 89   &6, 11, 12, & 22 & 111  \\
 
image   &    98, 123 &   & 28, 32, 38 & & \\
& & & & &  \\
\H\ profile shape (reject type 2,5) & 1, 3, 5, 6, 11, 13, 14, 17, 18, 21, & 40 & 1, 3, 9, 10,   & 11 & 51 \\
&   22, 30, 31, 33, 39, 42, 46, 49, 51, & & 15, 17, 19, 21, & & \\
&   55, 56, 57, 62, 65, 68, 70, 72, 75, & & 23, 26, 36 & & \\
&   76, 79, 81, 87, 90, 91, 92, 94, 95, & & & & \\
&  96, 100, 103, 105, 111, 112, 114, & & & & \\
&    115, 116, 119,  122, 124   & & & &  \\


& & & & & \\

Inclinations < 45 degrees & 4, 36, 43, 53, 85, 89, 104, 106, 108,   & 29 & 8, 14, 25, 29 & 7 & 36\\
&  113, 121 & & & & \\
& & & & & \\
\multicolumn{1}{c|}{\textbf{\textit{Quantitative criteria}}} & & & & &   \\
 Error on \wot and \wof < 10 \%   & 7, 37, 50, 54, 99, 102, 110, 118 &  21  & - & 7   & 28   \\


& & & & &\\

 
0.05 < |$\Delta$V$_{\mathrm{sys}}$/\wot| < 0.05    & 27, 78, 101  & 18 & - & 7 & 25 \\

  & & & & & \\

\wot - \wof < 50 \kms  & 10, 45, 58, 67, 93, 117 & 12 & - & 7   & 19  \\

  & & &  & &\\

\hline


\end{longtable}

\end{landscape}
}
\normalsize

\restoregeometry


%\appendix
\onecolumn

\foreach \x/\y in {7/1,10/2,27/3,37/4,45/5,50/6,54/7,58/8,67/9,78/10,93/11,99/12,101/13,102/14,110/15,117/16,118/17}{
   
    \begin{figure}
        \begin{center}
            \includegraphics[trim={4.5cm 1cm 3.5cm 0cm},clip,width=\textwidth]{chapter3/img/galf_A963/galfit_\x_atlas.pdf}
            \includegraphics[angle =270,trim={6cm 1.5cm 10cm 3.5cm},clip,width=1\textwidth]{chapter3/img/HI_A963/HIatlas\x.pdf}
            \captionsetup{labelformat=empty}
            \caption{A963 TFS cat no. \x}
        \end{center}
        
   
    \end{figure}}


\foreach \x in {2,9,20,40,48,61,63,71,82,86,88,109}{
\begin{figure}
  \begin{center}
   \includegraphics[trim={4.5cm 1cm 3.5cm 0cm},clip,width=\textwidth]{chapter3/img/galf_A963/galfit_\x_atlas.pdf}
   \includegraphics[angle =270,trim={6cm 1.5cm 10cm 3.5cm},clip,width=1\textwidth]{chapter3/img/HI_A963/HIatlas\x.pdf}
   \captionsetup{labelformat=empty}
   \caption{A963 TFS/HQS catno. \x}
   \end{center}
\end{figure}}


 

\foreach \y in {4,13,18,24,30,31,39}{
   \begin{figure}
  \begin{center}
   \includegraphics[trim={4.5cm 1cm 3.5cm 0cm},clip,width=\textwidth]{chapter3/img/galf_A2192/galfit_\y_atlas_A2192.pdf}
   \includegraphics[angle =270,trim={6cm 1.5cm 10cm 3.5cm},clip,width=1\textwidth]{chapter3/img/HI_A2192/HIatlas\y.pdf}
   \captionsetup{labelformat=empty}
   \caption{A2192 TFS/HQS cat no. \y}
   \end{center}
\end{figure}}











%\end{document}


